History-Matching of Imbibition Flow in Multiscale Fractured Porous Media Using Physics-Informed Neural Networks (PINNs)

We propose a workflow based on physics-informed neural networks (PINNs) to model multiphase fluid flow in fractured porous media. After validating the workflow in forward and inverse modeling of a synthetic problem of flow in fractured porous media, we applied it to a real experimental dataset in which brine is injected at a constant pressure drop into a CO2 saturated naturally fractured shale core plug. The exact spatial positions of natural fractures and the dynamic in-situ distribution of fluids were imaged using a CT-scan setup. To model the targeted system, we followed a domain decomposition approach for matrix and fractures and a multi-network architecture for the separate calculation of water saturation and pressure. The flow equations in the matrix, fractures and interplay between them were solved during training. Prior to fully-coupled simulations, we proposed pre-training the model. This aided in a more efficient and successful training of the coupled system. Both for the synthetic and experimental inverse problems, we determined flow parameters within the matrix and the fractures. Multiple random initializations of network and system parameters were performed to assess the uncertainty and uniqueness of the results. The results confirmed the precision of the inverse calculated parameters in retrieving the main flow characteristics of the system. The consideration of multiscale matrix-fracture impacts is commonly overlooked in existing workflows. Accounting for them led to several orders of magnitude variations in the calculated flow properties compared to not accounting for them. To the best of our knowledge, the proposed PINNs-based workflow is the first to offer a reliable and computationally efficient solution for inverse modeling of multiphase flow in fractured porous media, achieved through history-matching noisy and multi-fidelity experimental measurements.

==> changes/main0.tex <==
% \documentclass[12pt]{article}
% \usepackage{graphicx}
% \usepackage{titlesec}
% \usepackage[hyperfootnotes=true]{hyperref}
% \hypersetup{colorlinks, citecolor=blue, linkcolor=blue, urlcolor=blue}
% \usepackage{makecell}
% \renewcommand{\cellalign}{vh}
% \usepackage{hyperref}%
% \usepackage{color,soul}
% \usepackage{amsmath}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{changes}
% \providecommand{\keywords}[1]
% {\small	
% \textbf{\textit{Keywords---}} #1}
% \usepackage{geometry}
% \geometry{ a4paper, total={170mm,257mm}, left=30mm, right=30mm, top=25mm, bottom=25mm, }
% \graphicspath{{figs/}}
% \usepackage{caption}
% % \ucharacterisationinputenc
% \usepackage{authblk}
% \renewcommand\Authfont{\small}
% \renewcommand\Affilfont{\small}

% \usepackage[numbers]{natbib}

% % \usepackage{natbib} 
% % \bibliographystyle{apalike}
% % \bibliographystyle{naturemag} % Nature bibliography style
% % \bibliographystyle{nature} % Nature bibliography style
% \bibliographystyle{IEEEtranN} % Nature bibliography style

% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{eqns}  % Use the equations
% % \captionsetup{font=small}
% \usepackage{xcolor}




% \title{\textbf{History-Matching of Mixed Imbibition Flow in Multiscale Fractured Porous Media Using Physics-Informed Neural Networks (PINNs)}}
% % \title{\textbf{Physics-Informed Neural Networks (PINNs) Solver for History Matching of Multiphase Flow in Multiscale Fractured Porous Media}}


% \author[1]{Jassem Abbasi\thanks{Corresponding author: Jassem Abbasi (jassem.abbasi@uis.no)}}
% \author[2]{Ben Moseley}
% \author[3]{Takeshi Kurotori}
% \author[4]{Ameya D. Jagtap}
% \author[3]{Anthony R. Kovscek}
% % \author[2]{Siddhartha Mishra}
% \author[1]{Aksel Hiorth}
% \author[1]{Pål Østebø Andersen}

% \affil[1]{\textit{Department of Energy Resources, University of Stavanger, Stavanger, Norway}}
% \affil[2]{\textit{Seminar for Applied Mathematics, ETH Zürich, Zürich, Switzerland}}
% \affil[3]{\textit{Department of Energy Science and Engineering, Stanford University, Stanford, USA}}
% \affil[4]{\textit{Aerospace Engineering Department, Worcester Polytechnic Institute, Worcester, MA 01609, USA}}

% \begin{document}
% \maketitle

% \begin{abstract}
% In this work, we propose a workflow based on physics-informed neural networks (PINNs) to model, and history-match multiphase flow in fractured porous media experiments. After validating the workflow in forward and inverse modeling of a synthetic problem of flow in fractured porous media, we applied it to a real experimental imbibition dataset in which water is injected at a constant pressure drop into a CO$_2$ saturated shale core plug. The core plug was naturally fractured. The exact spatial position of fractures and dynamic in-situ distribution of fluids were imaged using a CT-scan setup. 
% To model the targeted system, we followed a domain decomposition approach for matrix and fractures; and a multi-network architecture for the separate calculation of water saturation and pressure. The flow equations in matrix, fractures, and interplay between them were solved during the training. Prior to fully-coupled simulations, we suggested pre-training the model to aid in the capturing of physical attributes more effectively.
% Both for the synthetic and experimental problems, we determined flow parameters within the matrix and the fractures. Multiple random initializations were performed to assess the uncertainty and uniqueness of the calculations, and the results confirmed the reliability of the solutions. The consideration of multiscale impacts, while commonly overlooked in existing workflows due to computational inefficiencies, has led to several orders of magnitude variation in the calculated flow properties. The proposed workflow demonstrated reliable  and computationally efficient solutions for inverse evaluation of problems corresponding to multiphase flow in multiscale porous media with noisy and multifidelity datasets. 




% \end{abstract}


% \keywords{keywords: Physics-Informed Neural Networks (PINNs), \and multiphase flow, \and inverse calculations, \and multiscale fractured porous media}



% \section{Introduction}


% Interpretation of multiphase flow phenomena in fractured porous media is challenging, because of their intrinsic multiscale nature \cite{Fung1991SimulationReservoirs}. In such systems, the behavior of fluids are variational across scale, where the processes at each scale influence the overall behavior of the system \citep{Geers2017HomogenizationProblems}. Almost all natural porous media are to some degree fractured; however, an inaccurate representation of their influence on flow phenomena can lead to substantial errors. These errors can propagate from microscale force balance estimations to macroscale predictions of porous media behavior. For applications such as geological carbon storage, fluid flow in aquifers, and recovery of hydrocarbons \citep{Rangel-German2006Multiphase-flowMedia} this can lead to incorrect predictions and suboptimal decisions. However, most common approaches for estimating multiphase flow properties in porous media are developed for homogeneous systems with simplified frontal behavior. These limitations make them inapplicable to complex multiscale problems, such as flow in naturally fractured rocks. The characterization of multiphase flow in porous media commonly is performed via inverse calculation of the model parameters through history matching of the experimental measurements. In practical procedures, the problem is bypassed by avoiding analyzing rocks with multiscale behavior, or making different simplifying assumptions \citep{Berre2019FlowApproaches}. However, these simplifications can be unreliable, particularly for formations like shale, where complex fracture networks significantly influence fluid flow behavior \citep{Salem2022ImpactShale}.

% The coupled matrix and fracture multiphase flow systems requires specialized techniques and approaches to model and simulate \citep{Odster2019AMedia}. Fractures introduce discontinuities in the flow field, which can lead to numerical instabilities and reduced accuracy in traditional numerical methods. Additionally, the need for fine discretization of the domain to capture these discontinuities results in high computational costs \citep{Bastian2000NumericalMedia}.
% In recent years, various numerical methods based on finite-element and finite-volume approaches have been recommended to solve the problem more efficiently \citep{Komijani2023AnCoupling, Myner2016AGrids}. However, the implementation of the algorithms is complex, and the numerical scheme typically faces challenges such as high computational requirements and low convergence reliability \citep{Yang2021RecentMedia}, making them impractical for inverse calculation purposes. Furthermore, recent advancements in measurement and imaging technologies have revolutionized our ability to characterize complex flow patterns in porous media. These improvements, while challenging to investigate, offer unprecedented accuracy and resolution, significantly enhancing our capacity to investigate multiphase flow dynamics \citep{Tekseth20244DTomography}. Given these limitations and opportunities, there is a persistent demand for the development of more precise and computationally reliable mathematical tools, especially for the inverse interpretation of multi-fidelity datasets.  

% In the recent years, Physics-Informed Neural Networks (PINNs) have emerged as a data-driven technique, seamlessly integrating both high-fidelity and noisy datasets and domain expertise to solve differential equations governing various engineering and scientific problems \citep{Raissi2019Physics-informedEquations}. More specifically, it has shown potential to solve problems of multiphase flow in porous media in forward or inverse modes \citep{Latrach2024ASystems}, e.g., modelling of countercurrent spontaneous imbibition \citep{Abbasi2023SimulationNetworks}, solving multiphysics coupled flow problems\citep{Amini2023InverseNetworks} and modelling density-driven flow in porous media for CO$_2$ storage \citep{Du2023ModelingSequestration}. However, studies are primarily focused on systems with homogeneous properties, often overlooking systems with multiscale features. The application of PINNs to multiscale problems is an emerging area of research, with some studies proposing various techniques in recent years \citep{Alber2019IntegratingSciences}. 
% For instance, \citet{Wang2021OnNetworks}, for problems such as wave propagation and Poisson equation, proposed using Fourier feature embedding to capture the behavior of the system at various spatial scales and avoid the potential spectral biases in the PINNs predictions. Spectral bias is defined as the tendency of networks to learn solutions with the lowest possible frequencies. \citet{Weng2022MultiscaleKinetics}  proposed multiscale PINNs for modeling of stiff chemical kinetics. They utilized different NNs with similar architectures for the different scales of magnitudes of reaction rates. \citet{Riganti2023AuxiliaryProblems} applied multi-output PINNs with multiple auxiliary variables associated and the Legendre terms to solve the Boltzmann equation efficiently. \citet{Moseley2023FiniteEquations} introduced Finite-Basis PINNs, by decomposing the domains of the problems, e.g., (2+1)-dimensional (D) wave propagation equations, using a finite set of basis functions, inspired by finite element methods. However, the literature shows significant gaps in applying PINNs for solving the multiphase flow in naturally fractured porous media, as a strategy for forward modeling and inverse parameter identification. 

% In this work, we have implemented a data-driven workflow based on multi-scale PINNs architecture for (3+1)D simulation of multiphase flow in fractured porous media and inverse calculation of flow parameters by history matching experimental-scale datasets with multi-fidelity attributes. The proposed workflow utilizes a multi-network architecture combined with various regularization techniques, such as data resampling during training, along with a step-wise training strategy to efficiently achieve the desired solutions. The robustness of the computational framework was first demonstrated through validation using a synthetic benchmark problem, and the performance compared against a common approach in the community. Then we investigated a complex experimental scenario of water flooding in CO$_2$ saturated fractured shale rock \citep{Kurotori2023MixedMedia}. We incorporated a large multi-fidelity observational dataset, including 3D in-situ saturation data measured using a high-resolution computed tomography (CT) scan setup, in the process of inverse calculations. Our work showcases the potential of PINNs to bridge the gap between complex physical models and experimental datasets, inverse analysis of the multi-fidelity experimental datasets corresponding to the multi-phase flow in fractured porous media. Furthermore, this work offers new insights into the multi-scale characterises of multiphase flow in complex fractured geological settings. 


% % {\color{red}Ameya: To enhance clarity and highlight the novelty of this manuscript, it is a good idea to integrate a point-wise discussion on the contributions alongside the discussion on the experimental dataset. This approach will distinctly showcase the unique aspects and innovations of the study.}



% \section{Results}

% We investigate a (3+1)D problem of two-phase flow in fractured porous media. It is assumed the flow is controlled by Darcy's law in both fracture (Ω$_F$ ) and matrix (Ω$_M$ ) domains, where we refer to the low-permeable non-fractured zone as matrix, and the high-permeable fractured zone as fracture. The matrix domain occupies the majority of the pore volume while the fracture domain has a much higher permeability than the matrix. A schematic of the geometry of the core and the fractures is visualized in Fig. \ref{fig:2}a. The Darcy velocity (\(u_i\)) of each phase is determined by Darcy's law \citep{Das2005UpscalingBeyond}:

% \begin{equation}
% u_i =-\lambda_i \nabla p_i,\ \ \lambda_i=\frac{Kk_{ri}}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy}
% \end{equation}

% where \(\lambda_i\) is mobility, \(p_i\) is the phase pressure, \(K\) and \(k_{ri}\) are absolute permeability and relative permeability, respectively, and \(\mu_i\) is the phase viscosity. The index \(i\) determines wetting \((w)\), and non-wetting \((nw)\) phases. The effects of gravity have been ignored. The capillary pressure, \(p_c = p_{nw}-p_{w}\), relates the phase pressures.  The conservation law for the spatiotemporal mass transport of phases in a matrix zone is defined as:

% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right)+q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_frac_cont}
% \end{align}

% A similar mass conservation equation can be defined in the fracture domain: 

% \begin{align}
% \phi^F\partial_t\left(\rho_is_{i}^{F}\right)=-\nabla^\parallel\left(\rho_iu_i^\parallel\right)\ -q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_F \label{eq:massbalF}
% \end{align}

% where \(q_i^\bot\) is matrix-fracture mass flux term and is a function of the local pressure difference between two mediums, and the matrix flow properties \citep{Berre2019FlowApproaches}. To solve above coupled equations, we defined a set of multi-scale neural networks architecture, and trained it based on concept of PINNs. See  \hyperref[sec:methods]{Methods} for detailed information on the mathematics of the problem, the NNs architecture, the collocation points applied, the observational data used, and the training procedure.



% \begin{figure}[htbp]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=.999\textwidth]%
%     {graphics/Fig2.jpg}% picture filename
% \end{center}
% \caption{\textbf{A schematic of the problem under study and the proposed PINNs-based computational workflow.} \textbf{a)} The simplified geometry of the matrix-fracture system and the impacting boundary conditions, \textbf{b)} The spatial distribution of the matrix and fracture collocation points, \textbf{c)} Separate networks for the state variables of matrix and fracture systems, \textbf{d)} The architecture of each NN, and \textbf{e)} the cross-sectional view of the porosity distribution in the experimental data, \textbf{f)} the proposed step-wise learning strategy.}
% \label{fig:2}
% \end{figure}



% \subsection{Synthetic Benchmark Problem}
% \label{sec:benchmarksection}
% This section focuses on validating the proposed workflow against a fully-characterized synthetic problem. We introduce a coupled matrix-fracture flow problem to validate the solutions obtained using PINNs and to compare different strategies. Fig. \ref{fig:benchprof}a1 provides a 3D visualization of the matrix-fracture system. Specifically, we define a cylindrical core featuring a significant vertical fracture (located at \(x=12.5\) mm) in the flow direction (\(y\)). The properties of both the matrix and the fracture are detailed in Table \ref{tab:benchprops}. Additionally, Fig. \ref{fig:benchprof}a2 illustrates the static geometry of the matrix and fracture system, along with a 3D visualization of the discretized model used for Finite-Difference (FD) simulation. We have utilized an in-house FD simulator \citep{Lohne2017ARegimes}, to provide with the solution of the defined benchmark problem. The advantage of the used simulator compared to other available simulators was its ability to seamlessly solve experimental boundary conditions. The specifications of the utilized PINNs model is provided in Table \ref{tab:benchPINNsprops}. In this section, the same network architecture as in Fig. \ref{fig:2} has been used. Also, the pre-training strategy was applied in both forward and inverse problems.


% \input{tables/t_bl}


% \subparagraph*{Forward simulation. } The flow saturation profile within the matrix, after forward solution of the problem based on the true parameter values, is visualized in Fig. ~\ref{fig:benchprof}. The visualisation of 3D profile of \(s_w\) and \(p_{w}\) as well as cross-sectional lateral invasion of water demonstrate the ability of the PINNs model to capture key 3D flow characteristics. The small errors in the predictions - i.e., the mean absolute error (MAE) of 0.028 for \(s_w\) and 0.42 bar for \(p_w\) - is accumulated mainly around the imbibition fronts. It is worth mentioning that, since the multiscale modeling strategies of the two approaches differ, we do not expect to achieve exactly identical solutions. The computational times for the numerical solver and the PINNs solver were comparable for this specific forward problem. Time-efficient and accurate solutions have been achieved via utilising a variety of techniques, such as pre-training of the PINNs model using simplified assumptions, separate network architecture, resampling of the points during the training, and Fourier transformations in the networks, as described in \hyperref[sec:methods]{Methods}. Resampling of the collocation points at suitable intervals helped the model to reach more accurate and unique solutions within an ensemble of simulations. Figure~\ref{fig:benchprof} clearly shows a sharp change in saturation at the flow fronts. This observation is primarily due to the low viscosity of CO$_2$ compared to the water phase (viscosity ratio of \(\mu_{\text{CO}_2}/\mu_{\text{water}} = 0.017\)). This difference in mobility of fluids creates a shock front in the system which is normally reported challenging for many mathematical methods to solve, including PINNs \cite{Fuks2020LIMITATIONSMEDIA}. In the matrix system, the problem is manageable as the frontal shock is mainly cancelled-out by capillary diffusion effects. However, in the fracture domain, the flow is primarily governed by viscous forces, necessitating specialized techniques. In this work, we assumed a small value of capillary diffusion in the fracture domain to mitigate the described issue without compromising the accuracy and speed of the computations.
 

% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.95\textwidth]%
%     {graphics/fdbench.jpg}
% \end{center}
% \caption{\textbf{The geometry, and a comparative analysis of the frontal behavior of fluids as simulated by PINNs and FD for the benchmark problem’s forward simulation.} \textbf{a)} The map of the fracture in the synthetic matrix-fracture problem: 1) the geometry, 2) the equivalent static model for the FD simulations, \textbf{b)} a 3D visualization of  \(s_w\), and \(p_w\) profiles, and their point-wise absolute errors at t=57.7 hrs. \textbf{c)} the 2D cross-sectional view of \(s_w\) at y=29 mm for various time points: t=33.2, 57.7, and 81.2 hrs.}
% \label{fig:benchprof}
% \end{figure}


% \subparagraph{Inverse Calculations Based on History Matching of Recovery Factor.}
%  Here, we try to utilise PINNs for the purpose of inverse calculating the flow parameters of the system, i.e., \(k_r\), \(p_c\) and \(\Lambda\) of matrix, by history matching of the observational data. Here, \(\Lambda\) refers to a normalized Capillary Diffusion Coefficient (CDC), which controls the rate of capillary flow within porous media and is a function of the \(k_r\) and \(p_c\) curves. At this stage, we consider only the RF curve as the observation data - which represents the volumetric fraction of the CO$_2$ phase expelled from the porous media over time. In this benchmark example, the porosity and permeability of the matrix, as well as all the properties of the fracture, are assumed to be known prior to calculations. After random sampling of the inverse parameters, the calculations continued for 22000 epochs, until the error in RF was minimized (Fig. \ref{fig:benchinvres}a), the loss terms are stabilized (Fig. \ref{fig:benchinvres}f1), and the trend of changes in inverse parameters reached to plateau (Fig. \ref{fig:benchinvres}f2). The matching of the matrix RF curve (Fig. \ref{fig:benchinvres}b) could lead to the accurate estimation of the \(\Lambda\) curve with normalized mean absolute error (NMAE) of 0.098, as observable in Fig. \ref{fig:benchinvres}b. PINNs calculations could also accurately predict the volumetric rate of the injected water, as shown in Fig. \ref{fig:benchinvres}c. The main determining factor on the total injected rate is $K_F$, as the fracture shows orders of magnitude higher permeability compared to the matrix. 

% However, as expected, the model did not accurately retrieve the \(k_r\) and \(p_c\) curves (Figs. \ref{fig:benchinvres}c and \ref{fig:benchinvres}d) due to the system's high degrees of freedom and the insufficient information on the wetting phase pressure. We expect that there are infinite sets of \(k_r\) and \(p_c\) curves that can lead to the observed dataset, as reported by \citet{Abbasi2024ApplicationTests}. This limitation is evident in Fig. \ref{fig:benchinvres}e, where the network could predict the saturation profile in the system but failed to accurately predict the pressure distributions. The error is higher in zones with lower \(s_w\) values, due to the significance of \(p_c\). All possible combinations of \(k_r\) and \(p_c\) curves (that lead to similar \(\Lambda\) curves) are expected to lead to similar imbibition trend and frontal behavior. 

% Fig. \ref{fig:MFflow} provides a comparison of the matrix-fracture exchanges. Positive values indicate flow out of the fracture (into the matrix). In contrast, negative values indicate flow into the fracture (from the matrix). Initially, we observe a strong wetting phase flow from the fracture to the matrix, which stabilizes over time. This behavior results in an almost straight cumulative flow line versus \(\sqrt{t}\) at the beginning of the flow (\(t<20\) hrs), highlighting the significant influence of capillary forces. The trend of cumulative imbibed volume then stabilizes at \(t>20\) hrs, as also reported in \citet{Zahasky2019SpatialImbibition}. However, the non-wetting phase experienced a matrix to fracture flow at the early times of the simulation, and which then stopped after \(t\approx 4\) hrs. This behavior is anticipated in combined co-current/counter-current spontaneous imbibition processes, as also reported by \citet{Haugen2014CapillaryTest}. Fig. \ref{fig:MFflow}c compares vector field of velocity for both phases. Although the wetting phase continuously imbibes into the matrix, the non-wetting phase follows viscous forces within the matrix towards the outlet of the system, indicating \textit{the governance of the co-current spontaneous imbibition mechanism in the matrix in a large fraction of the injection period}. 





% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/benchres.jpg}
% \end{center}
% \caption{\textbf{The results of inverse calculation for the synthetic benchmark model, based on history matching of the RF curve vs. time.} \textbf{a)} The trend of minimizing error compared to the RF data, \textbf{b)} The RF curve, \textbf{c)} The estimated flow curves compared to the true and the randomly initialized values: \(\Lambda\), \( p_c\) and \(k_r\) curves, respectively, \textbf{d)} The comparison of water injection rate for FD and PINNs models,  \textbf{e)} The flow profile along the injection direction for (1) \(s_w\)  and (2) \(p_w\), at t= 23.22, 57.7, 98.2, 167.9 hrs, \textbf{f)} the training trend, 1) The total loss term, ${\mathcal{L}}_{t}$, and loss terms corresponding to the PDE residuals for matrix, i.e.,  ${\mathcal{L}}_{PI}^{M}$, ${\mathcal{L}}_{PIw}^{M}$, and ${\mathcal{L}}_{PInw}^{M}$ , 2) the trend of changes in $\bar{\Lambda}$, \textbf{g)} A comparison of the run-time and accuracy of two history-matching approaches in the estimation of the \(\Lambda\) curve: PINNs, and FD + Nelder-Mead (NM) optimizer. }
% \label{fig:benchinvres}
% \end{figure}




% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/MFflow.jpg}
% \end{center}
% \caption{ \textbf{The matrix-fracture interaction rates for the benchmark problem.} In all the figures the right axis show the cumulative values. The scatter points represent values at various spatiotemporal collocation points; \textbf{a1,2)} The mass rate of flow between two media for both phases; the right axis shows the cumulative mass flow (equation (\ref{eq:massratecum})). \textbf{b1,2)} the volumetric rate of flow; the right axis show the cumulative fraction of pore-volume (equation (\ref{eq:dimenlessPVMF})), \textbf{c)} 2D vector field plot at z=0.0125 m. Here, \( u_w \) and \( u_{nw} \) are not directly comparable, as they are scaled to the same range for visualization purposes.}
% \label{fig:MFflow}
% \end{figure}



% \subparagraph{Uncertainty Quantification.} To validate the reported results, we employed an ensemble-based uncertainty quantification approach, performing multiple iterations with random initializations of the inverse parameters (refer to Appendix \ref{sec:PINNsComputationalstrat} for detailed methodology). As demonstrated in Fig. \ref{fig:benchinvens}a, the \(\Lambda\) curves consistently converged to similar values in different cases, all with low errors compared to the true \(\Lambda\) curve. It shows that \textit{ the system is well defined in relation to the \(\Lambda\) curve}, which means that there is only one set of \(\Lambda\) that can produce the observed measurements. In contrast, the \(k_r \) and \(p_c\) curves converged to distinct values, exhibiting the high degree of freedom in the system of equations. Similar results have been discussed in \citet{Abbasi2024ApplicationTests} for a 1D spontaneous imbibition system. Accurate estimation of the \( p_c \) curve requires measuring the pressure of both phases, which is often challenging in practical scenarios. Consequently, the uncertainty in the \( p_c \) curve propagates to the \( k_r \) curves. The results show the challenges in calculating \( k_r \) and \(p_c\) in problems dominated by capillary forces. Additionally, we observe low discrepancies between different solutions of \(k_{rnw}\). This is due to the low viscosity of the CO\(_2\) phase, which results in a high sensitivity of phase velocity to \(k_{rnw}\) values, makes their range of variation much lower than \(k_{rw}\).


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.991\textwidth]%
%     {graphics/bench_ens.jpg}
% \end{center}
% \caption{ \textbf{The inverse calculation results for an ensemble with different initialization of the inverse parameters.} The initialization has been performed randomly.  \textbf{a)} the initial guess \textcolor{gray}{(gray)} and the final estimations after inverse calculations have been compared for \textcolor{magenta}{(magenta)} of \( \Lambda\), \( p_c\), \( k_{rw}\) and \( k_{rnw}\)  curves, respectively. The \textcolor{blue}{blue} curves show the true values. The shaded areas represent the mean $\pm$ standard deviations (STD).  \textbf{b)} the optimization landscape of different terms during optimization during the training: \( \mathcal{L}_t\), RF (MAE), and \( \bar{\Lambda}\), respectively.}
% \label{fig:benchinvens}
% \end{figure}



% \subparagraph{Computational Cost.} The PINNs calculations were performed on a single A2000 GPU, which took around 1.5-2.5 hours depending on the size of the network and collocation points. The computational time was in the same range for both the forward and inverse problems, and regardless of the different sets of observational data used during history-matching, such as the in-situ $s_w$ dataset. For comparison, we also attempted to history-match the problem using a coupled FD and Nelder-Mead (NM) optimizer (see Appendices \ref{sec:compres} and \ref{sec:historymatching} for more info). Individual forward simulations for a 27,000 cell FD model ranged from 40 minutes to 2 hours, depending on the complexity of effective parameters (e.g., flow parameter shapes and matrix-fracture property contrasts). In the case of history matching the RF curve, the computational time of FD-NM optimisation was around 20 hours, with the NMAE of 0.81 (compared to the NMAE of 0.098 for PINN) in the estimated $\Lambda$ curve (see Fig. \ref{fig:benchinvres}g). When we added the in-situ $s_w$ dataset, the FD-NM optimizer failed to operate efficiently. The results highlights\textit{the significant advantage of proposed PINNs-based workflow compared to FD-based history-matching approach for inverse evaluation of experiments of multiphase flow in fractured porous media.}.






% \subsection{Experimental Problem}
% This section employs PINNs for the interpretation and parameter identification of a real experiment of multiphase water-CO$_2$ flow in a naturally fractured shale rock sample, presented in \ref{sec:experimentaldata}. The known properties of the system is shown in Table \ref{table:shalerockprops}. As an initial estimation, \(K\) and \(K_F\)  are assumed as 0.01 and 100 multipliers of the experimentally measured mean permeability of the rock  (\( K = 0.01 K_{exp} \) and \( K_F = 100 K_{exp} \)). The impact of \( K \) can be indirectly adjusted based on the calculated \(\Lambda\) curve, and \( K_F \) can be accurately calculated through history-matching the total injection rate of water. Among all properties of the system, \(k_r(s_w)\), \(p_c(s_w)\), and their combined alternative, \(\Lambda(s_w)\), as well as \(K_F\) are unknown and are required to be estimated based on the experimental observations.



% \input{tables/table_experimental_props}



% \subparagraph{History Matching of the recovery curve and the total injection rate.} 
% The volume of recovered fluids, the volume of the injected fluids, and the pressure drop along the core, all over time, are the most commonly utilized observational data for studying multiphase flow processes in porous media. We calculated the RF curve by averaging the in-situ water saturation data obtained from CT-scan measurements. In addition to the matrix multi-phase flow parameters,  $K_F$ was assumed unknown, and allowed to be estimated during the inverse calculations. Inverse computations were started by randomly generated initial guess values for each parameter. To perform history matching of the RF curve, we employed the step-wise calculation process, as introduced in section \ref{sec:SolutionMethod}. The training process was stopped after 17000 epochs, when the trainable parameters reached a plateau. The validity of the inverse-calculated parameters then was validated by running a fine-grid FD numerical simulation based on these parameters, and comparing the obtained results with the experimental data. The results of inverse computation of matrix flow parameters, i.e., \(k_r\), \(p_c\), \(\Lambda\) curves  are shown in Fig. \ref{fig:expres1}a. The validation of these curves by the forward FD simulations showed a reasonable match to the RF of the experimental data (Fig. \ref{fig:expres1}c). Simultaneously, we matched the total injected fluids versus time, as shown in Fig. \ref{fig:expres1}d. The total volume of injected fluids is predominantly influenced by \(K_F\), as a significant portion $(>99\%)$ of the injected fluid enters the core through the fracture system and then flows toward the outlet face by bypassing the matrix. A small fraction of the fluid imbibes into the matrix, enabling the depletion of the non-wetting phase. The high injection rate at the beginning of the flow is due to the low resistance of the CO$_2$ phase, which initially saturated the fracture domain. The rate quickly drops to the level of $\approx$ 1.0 $mm/hr$ after breakthrough of the water phase at the outlet. A comparison of the RF curve, and the breakthrough time of water shows the injection rate of water is much higher than the critical rate of water advance. The critical rate is defined as the rate of water advance at which the positions of the water fronts in both the matrix and the fracture are equal \citep{Mattax1962ImbibitionReservoir}. It is concluded that \textit{the frontal behavior of fluids in matrix is not significantly influenced by the total injection rate in the system}, due to the permeability dominance of fracture domain \cite{Berkowitz2002CharacterizingReview}.


% \subparagraph{ The calculated $k_r$ and $p_c$ curves are not unique.} 
% As it is also previously discussed in \ref{sec:benchmarksection}, \textit{the \(k_r\) and \(p_c\) curves exhibit non-uniqueness due to the degrees of freedom within the system} (unlike the \(\Lambda\) curve that can be uniquely estimated). 
% This conclusion is further supported by the results of ensemble-based uncertainty quantification shown in Figure \ref{fig:expres1}e. The accurate estimation of \(k_r\) is easier when the effects of viscous forces dominate the matrix flow. However, in this system, the matrix is primarily influenced by capillary forces.



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.999\textwidth]%
%     {graphics/expres1.jpg}
% \end{center}
% \caption{ \textbf{The results for inverse calculation of matrix flow parameters by history matching of the RF experimental data.} \textbf{a)} The initial guess and final inverse calculated flow curves, i.e., \(k_r\), \(p_c\) and \( \Lambda\) curves, respectively. \textbf{b)} The trend of converging to the final values vs. epoch for different inverse parameters, \textbf{c)} The matched \( \bar{s_w}\) curve by PINNs (1) and the validation results from FD simulations (2), \textbf{d)} Matching the fracture permeability (\(K_f\)) and the history matching of volumetric injection rate: 1) the trend of changes in \(K_f\) versus the matrix permeability and experimentally measured permeability, \(K_{exp}\), 2) The contribution of matrix and fracture in the inlet face, 3) The total velocity of fluids compared to the experimental observational data. \textbf{e)} The results of inverse calculations for an ensemble of models with different initialization values. e1 and e2 show the convergence trends, and later show the saturation function curves. The grey curves are the initial guesses. }
% \label{fig:expres1}
% \end{figure}




% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/profile3dexp.jpg}
% \end{center}
% \caption{ \textbf{A visualization compares water saturation ($s_w$) and wetting phase pressure ($p_w$) distributions in the porous media (matrix) at different times}. The figure compares the PINNs solution after inverse computations, FD solution after forward validation simulation, and experimental CT-scan images. It is important to note that the local saturation data was not utilized during the inverse calculations for the PINNs. Also, the FD simulation shows the forward analysis using the PINNS-based inverse calculated flow parameters. }
% \label{fig:3DprofileExp}
% \end{figure}

% \subparagraph{The Importance of Multiscale Simulations.} We investigate the significance of multiscale simulations in understanding multiphase flow in porous media in complex geometries, and their impacts on parameter identification calculations. In two separate cases, we conducted inverse calculations using PINNs while ignoring fractures and their interaction with the matrix: 1) matching only RF data, 2) matching RF data as well as total injection rate (Q$_{inj}$). Then, we compared the results to the cases with included fractures (see Fig.~\ref{fig:fracimpact}). The results clearly show the differences between the inverse calculated flow parameters (Fig.~\ref{fig:fracimpact}a). In the case of matching only RF data, ignoring the impacts of fractures could lead to about two orders of magnitude difference in the magnitude of the capillary forces in matrix ( \( \bar{\Lambda}= 8e-3 \) for the non-fractured scenario, compared to \( \bar{\Lambda}= 9e-5 \) for the fractured scenario). When Q$_{inj}$ was used as observational data, the results, specifically the relative importance of viscous and capillary forces, significantly changed. This led to high relative permeability and low capillary pressure values, which can be unexpected for shale rock. It resulted in the misidentification of viscous flow as the dominant mechanism, underestimating the influence of capillary forces. 
% The obtained results highlights the \textit{critical need for multiscale matrix-fracture simulations when dealing with porous media exhibiting multiscale features like fractures}. However, these multiscale impacts are normally bypassed or overlooked in existing workflows due to computational inefficiencies and instability issues in numerical methods .


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/fracimpact.jpg}
% \end{center}
% \caption{ \textbf{The impact of multiscale simulations on the inverse calculated flow parameters of porous media.} \textbf{a)} The calculated flow parameters, i.e.,  \( \Lambda\) ,\( p_c\), and \( k_r\) vs. saturation, respectively. \textbf{b)} The validation of the obtained results with FD simulations, in matching with the experimental RF data, \textbf{c)} The trend of changes in \( \mathcal{L}_t\), \( \bar{\Lambda}\), \({k}_{rw}^{max}\), and MAE in RF  vs. epochs, respectively. }
% \label{fig:fracimpact}
% \end{figure}




% \subparagraph{History matching of in-situ water saturation data.}

% History matching of high-fidelity datasets, in this case (3+1)D in-situ water saturation data from CT scans, presents a significant challenge but also offers exciting opportunities to gain deeper insights into porous media properties. In Fig. \ref{fig:insitusat}, rather than relying on RF data for the inverse calculations, we utilized the local spatiotemporal values of \(s_w\) directly as observational data for both history matching and the estimation of flow parameters. Additionally, we employ an adaptive fracture importance determination strategy to understand local variations in matrix-fracture interactions, serving as indicators of changes in fracture properties within the rock. A comparison of cases the history matching of the datasets with and without denoised observational data show no meaningful differences in both saturation distributions as well as the inverse calculated \(\Lambda\) curves. Denoising have been performed via a 3D convolutional kriging approach, as explained in Appendix \ref{sec:PINNsComputationalstrat}. These results exhibit \textit{the capabilities of PINNs in extracting the governing physical properties of systems even in the presence of noisy observations} \citep{Chen2021Physics-informedData}. 

% In Fig. \ref{fig:insitusat}c, an approach is utilized to automatically detect the inconsistencies between the PINNs predictions (based on the homogeneous fracture properties assumption), and the CT-scan images, in the fractured zone. The approach is explained in Appendix \ref{sec:PINNsimplementation}. In the points with gray color, the PDE solution closely matches the CT images, indicating high certainty in the defined fracture system. In the blue zones, the CT images show less imbibition than expected values by the PINNs solution, suggesting lower matrix-fracture interactions. Conversely, in the red regions, the saturation trends in the CT images differ significantly from the PINNs expectations, highlighting discrepancies that were successfully detected in both the original and denoised datasets. The results successfully showed the differences between the fracture properties, as well as uncertainties in the zones considered as the fractured areas. The results demonstrate that while we assumed a connected fracture network with uniform properties, the observations may not confirm these assumptions.



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/insituepinns.jpg}
% \end{center}
% \caption{\textbf{ The PINNs solution for inverse calculations when the in-situ water saturation data have been used as the observations.} A comparison has been made between two cases in which the observations have been pre-processed using a convolutional kriging algorithm. \textbf{a)} A comparison of the inverse calculated flow curves (\(k_r\), \( p_c\) and \(\Lambda\), respectively) for different scenarios of using observational data, \textbf{b)} A comparison of the 3D water saturation ($s_w$) profiles at $t=23.4$ hrs, \textbf{c)} The results of fracture uncertainty quantification (\textcolor{gray}{gray} indicates minimal uncertainty, \textcolor{blue}{blue} represents medium uncertainty, and \textcolor{red}{red} represents high uncertainty) }
% \label{fig:insitusat}
% \end{figure}






% \section{Discussion}

% In this study, we have proposed a computational workflow based on Physics-Informed Neural Networks (PINNs) as a solver for the simulation and parameter identification of (3+1)D two-phase flow processes in naturally fractured porous materials. The workflow can be applied as a tool for interpretation of experimental datasets of multiphase flow in porous media with complex geometries. After validation of the model against a synthetic scenario, we applied the framework to interpret and analyse a multi-fidelity experimental dataset for water injection in a CO$_2$ saturated fractured shale rock. The studied experimental problem is characterized by a confluence of complexities: significant permeability contrasts, unpatterned distribution of fractures, highly unfavorable mobility ratios, and the presence of shock fronts in the fractures. 

% The results demonstrated the effectiveness of the workflow in capturing the multiscale flow dynamics, as well as the phase and pressure distributions in the system. In the case of inverse calculations, the workflow could perform the calculations orders of magnitude faster and more accurate than FD simulation methods. The implemented uncertainty quantification analysis yielded valuable insights into the unique and non-unique characteristics of the obtained solutions. The problem could be uniquely characterized with a unique \(\Lambda\) curve, in which is a combination of different flow properties of the system, confirming the relative dominance of capillarity forces as the flow mechanism in the matrix. However, reaching reliable information on individual \(k_r\) or \(p_c\) curves was not possible, as demonstrated by the applied uncertainty quantification analysis. Additionally, as the fractures served as primary flow conduits, we could reach to the unique values for the fracture permeability by matching the injected volume of the water phase. 

% Our comparison of inverse calculations with and without fractures demonstrates the pivotal role of multi-scale phenomena in interpreting the experiments of multi-phase flow in fractured porous media, as the presence of fractures introduces a hierarchy of scales in the system. These multi-scale effects, while commonly overlooked in practical procedures, can significantly change the overall system behavior, influencing the inverse calculated parameters such as effective permeability, capillary pressure, and relative permeability relationships, as well as the interplay between different flow mechanisms in the system. For instance, the role of capillary forces may be significantly mischaracterized, as the harmony between capillary forces in the matrix and viscous forces in the fractures creates a complex, scale-dependent flow regime. This oversight can result in misleading parameter estimations, misattribution of flow behaviors, and ultimately, the development of incorrect conceptual or large-scale geological models, potentially leading to poor predictions and decision-making in practical applications. The proposed model also performed well in evaluating the (3+1)D noisy observations of water saturation, and achieved results comparable to the denoised dataset. However, while PINNs offer promising solutions, further development is necessary to achieve fully reliable models for a wide range of multiphase flow scenarios. Increasingly complex fracture distributions likely require even more complex neural network architectures. This highlights the need for developing more flexible network architectures capable of handling the significant non-linearities exist in such complex systems.


% % {\color{red} Ameya: We should emphasize the detailed discussion of the in-situ experimental data set, as this is a key expectation of top journals like NMI. Without this, the paper may be perceived as another application-based PINN study.}




% \section{Methods}
% \label{sec:methods}


% \subsection{Mathematics of Flow in Fractured Porous Media}
% \label{sec:mathematicsofphysics}

% We approach a problem of 3D multiphase flow in a fractured porous media at core scale. 
% Our focus is specifically on interpreting data from a cylindrical core-plug experiment (rock taken from the Wolfcamp formation) \citep{Kurotori2023MixedMedia}. We refer to the low-permeable non-fractured zone as a matrix, and the high-permeable fractured zone as a fracture. The model is inferred from the definition that the matrix domain \((\Omega_M)\) occupies the majority of the pore volume and that fractures domain \((\Omega_F)\) have a much higher permeability than the matrix. A schematic of the geometry of the core and the fractures is visualized in Fig. \ref{fig:2}a. 
% The core is placed horizontally, and the fractures are distributed in the core with different orientations. The radial surface of the core at \(r_c\) is closed (no-flow boundary). The inlet and outlet faces are at \(y=0\)  and \(y=L\), respectively.  Water and CO\textsubscript{2} are considered to be the wetting \((w)\) and non-wetting \((nw)\) phases, respectively. In line with the experimental conditions, we neglected both the compressibility and the solubility of the phases. The system is initially saturated with the \(nw\) phase. The definition of the system implies that the flow phenomena are governed by mixed-imbibition mechanisms, where the fracture flow is driven by forced imbibition, and the matrix flow is governed by spontaneous imbibition between the fracture(s) and the matrix. Forced imbibition happens when an external force drives the wetting phase fluid through the porous media, overcoming any resistance from the medium and the non-wetting phase. Spontaneous imbibition, on the other hand, is the process in which the wetting phase fluid flows into a porous media via capillary forces without the need for external pressure \citep{Anderson1987WettabilityPressure}. In the following, the mathematics of flow in matrix and fracture domains are discussed.

% \subparagraph{Matrix Flow. }
% The Darcy flow velocity (\(u_i\)) of each phase in the matrix is determined by Darcy's law:

% \begin{equation}
% u_i =-\lambda_i \nabla p_i,\ \ \lambda_i=\frac{Kk_{ri}}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy}
% \end{equation}

% where \(\lambda_i\) is mobility, \(p_i\) is the phase pressure, \(K\) and \(k_{ri}\) are absolute permeability and relative permeability, respectively, and \(\mu_i\) is the phase viscosity. The index \(i\) determines\((w)\), and \((nw)\) phases. The effects of gravity have been ignored. The conservation law for the spatiotemporal mass transportation of phases in a matrix zone is defined as:

% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right),\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_cont}
% \end{align}


% Given that \({s}_{wc}=0\), we define the initial conditions as:

% \begin{align}
% \left\{\begin{array}{left} {s}_{w}(x,y,z,t = 0) = 0\\ {p}_{nw}(x,y,z,t = 0) = {p}_{i} \\  \end{array}\right \ \ \ {, \in\Omega}_M
% \label{eq:eqICmatrix}
% \end{align}

% At the inlet face ($y=0$), the wetting phase is injected under a constant pressure ${p}_{in}$ over time. At this face, it is assumed the wetting phase takes the highest possible mobility:

% \begin{align}
% \left\{\begin{array}{left} {s}_{w}(x,y = 0,z,t) = 1 - {s}_{nwr} \\ {p}_{w}(x,y = 0,z,t) = {p}_{in} \\  \end{array} 
% \label{eq:eqBC0matrix}
% \end{align}

% The production from the outlet face \((y=l)\) occurs at a constant pressure, \({p}_{out}\):
% \begin{align}
% {p}_{nw}(x,y = L,z,t) = {p}_{out} 
% \label{eq:eqBC1matrix}
% \end{align}
% At the outlet face of the core, no explicit constraints are imposed on the saturation of the fluid phases. The radial faces \((r = r_c)\) are sealed from flow in radial directions:

% \begin{align}
%  \frac{\partial p}{\partial r} |_{r = r_c} \approx |\frac{\partial p}{\partial x} |_{r = r_c} + |\frac{\partial p}{\partial z} |_{r = r_c} |= 0 
% \label{eq:eqBC1matrix}
% \end{align}

%  The assumed matrix properties state that the flow in the matrix is governed by viscous and capillary forces (gravity effects are assumed to be negligible). 


% \subparagraph{Fracture Flow. }
%  A fracture is typically characterized as a narrow, and high permeable zone enclosed by a less permeable matrix zone. This contrast in properties leads to highly heterogeneous flow behavior across the scales. The aperture between the fracture surfaces is generally small and is normally occupied by filling materials, which affects its effective porosity and permeability values \citep{Wu2016MultiphaseMedia}. 

% Although fractures are discontinuities in the porous medium, they can be considered as a separate porous medium domain \((\Omega_F)\). This assumption enables us to apply Darcy's law. 
% Consequently, we assume fractures to be high permeable porous zones. This makes the equations in the two media consistent, eliminating the need for unnecessary complexities in the calculations \citep{Martin2005ModelingMedia}. So, the average flux of each flowing phase in a fracture is written by modification of Darcy's law in equation (\ref{eq:darcy}):
  
 
% \begin{equation}
% v_i^{\parallel}=-\lambda_i^{\parallel} \nabla^\parallel p_i ,\ \ \lambda_i^\parallel=\frac{K^F k_{ri}^\parallel}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy_frac}
% \end{equation}

% In this equation, \(K_F\) is the fracture permeability, and \(k_{ri}^\parallel\) is the relative permeability of the fluids in the fracture. The value of the \(K_F\) is dependant on the fracture aperture, and also the extent of the filling materials in the fracture. 


% \subparagraph{Matrix-Fracture Interactions. }

% The accurate treatment of multiphase flow in a fractured porous media depends on the modeling of the dynamic matrix-fracture coupled interactions. Utilizing Darcy's law, the matrix-fracture flux is approximated by \cite{Berre2019FlowApproaches}:

% \begin{align}
% v_i^\bot=-2K^\bot\lambda_i^\bot\left[\frac{ p_{M,i}-p_{F,i} }{e_V}\right],\ \ \lambda_i^\bot \simeq \frac{k_{ri}}{\mu_i},\ \ \left(i=w,nw\right), \label{eq:e8}
% \end{align}

% Where \(K^\bot\) refers to the matrix-fracture permeability normal to the fracture surface, and \(e_V\) is the fracture average aperture. As an ideal case, if one assumes fracture as an open space between two parallel surfaces, then the aperture is called hydraulic aperture, \(e_h\). In practice, the value of \(e_v\) is much larger than  \(e_h\), i.e., \(e_v>>e_h\), as the fractures are normally filled with materials. The value of \(K_F\) is theoretically correlated to \(e_v\). In this study, the fracture aperture, \(e_v\), is assumed to be 0.001 m for all the fractures, and kept constant in all the evaluations. The cumulative value \( V_i^\bot(t)  \) of a rate \( v_i^\bot(t)  \) over time is given by the integral:

% \begin{align}
% V_i^\bot(t) = \int_0^t v_i^\bot(\tau) \, d\tau
%  ,\ \ \left(i=w,nw\right), \label{eq:cumv}
% \end{align}

% We can rewrite equation (\ref{eq:e8}) to obtain the mass transfer rate [kg/m\(^3\)/s] between the two media:

% \begin{align}
% q_i^\bot=\frac{2\rho_i}{e_V} v_i^\bot ,\ \ \left(i=w,nw\right), \label{eq:massrate}
% \end{align}
% The factor 2 denotes the flow across both sides of fracture to matrix, assuming the equal flow characteristics across the two surfaces of the fracture. Then, the cumulative mass rate [kg/m\(^3\)] is:
% \begin{align}
% Q_i^\bot(t) = \int_0^t q_i^\bot(\tau) \, d\tau
%  ,\ \ \left(i=w,nw\right), \label{eq:massratecum}
% \end{align}




% The equation of mass conservation in the fracture is the same as in the matrix, with an additional term representing the mass from the fracture to the matrix \( q_i^\bot \). So, by modifying the matrix mass balance equation (equation (\ref{eq:matrix_cont})), we define the mass balance in the fracture system:

% \begin{align}
% \phi^F\partial_t\left(\rho_is_{i}^{F}\right)=-\nabla^\parallel\left(\rho_iu_i^\parallel\right)\ -q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_F \label{eq:massbalF}
% \end{align}

  
% At the contact point of the matrix and fractures, the continuity equation should also be solved in the matrix domain. So, we may rewrite equation (\ref{eq:matrix_cont}) as: 


% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right)+q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_frac_cont}
% \end{align}


% The fraction of the pore volume of the matrix [dimensionless] that has been transferred between the matrix and fracture can also be calculated using the following equation:

% \begin{align}
% V_i^\bot(t) = \frac{Q_i^\bot(t)}{\phi \rho_i},\ \ \left(i=w,nw\right), \label{eq:dimenlessPVMF}
% \end{align}




% \subparagraph{Closure Equations. }
% Capillary pressure and relative permeability curves are crucial input to model multiphase flow in porous media, e.g., in equations (\ref{eq:matrix_cont}), (\ref{eq:massbalF}) and (\ref{eq:matrix_frac_cont}). These curves are normally defined using theoretical correlations, with a few matching parameters. In this work, we apply an extended version of the Corey function \citep{Corey1954ThePermeabilities} to model relative permeability curves:


% \begin{align}
% {k}_{rw}({S}_{w}) = {k}_{rw}^{max}({S}_{w})^{{n}_{w}};\ \ \ \ \ \ {n}_{w} = {n}_{w1}{S}_{w} + {n}_{w2}(1 - {S}_{w}) \label{eq:krw_eq}
% \end{align}
% \begin{align}
% {k}_{rnw}({S}_{w}) = {k}_{rnw}^{max}(1 - {S}_{w})^{{n}_{nw}};\ \ \ \ \ \ {n}_{nw} = {n}_{nw1}{S}_{w} + {n}_{nw2}(1 - {S}_{w})
% \label{eq:krnw_eq}
% \end{align}

% In the extended version, \(n_w\) and \(n_{nw}\) are defined as saturation exponents that are weighted linearly with saturation \(S_w\). \(S_w\) is the normalized water saturation and is calculated as:

% \begin{align}
% {S}_{w} = \frac{{s}_{w} - {s}_{wc}}{1 - {s}_{nwr} - {s}_{wc}};
% \label{eq:Sweq}
% \end{align}

% The capillary pressure curve \(P_c(S_w)\) [pa] is calculated via Leverett scaling \citep{Leverett1942Dimensional-modelBehavior}:

% \begin{align}
% P_c = \sigma \sqrt{\frac{\phi}{K}} J
% \label{eq:pceq}
% \end{align}

% In this context, J(S$_w$) represents the Leverett J-function, a dimensionless function that describes the shape of the capillary pressure curve. We define J-function via the modified \citet{Bentsen1977UsingCurve} correlation:

% \begin{align}
% J(S_w) =  - {J}_{1}\mathrm{\ln}(\frac{{S}_{w}}{{S}_{eq}}) + {J}_{2}\mathrm{\ln}(\frac{1 - {S}_{w}}{1 - {S}_{eq}})
% \label{eq:Jeq}
% \end{align}

% The equation is hard constrained in a way that that \(J(S_{eq})=0\) and that \(dJ/dS_w\)   becomes infinite at endpoints. 

% However, previous research by \cite{Andersen2023Early-andCoefficient} demonstrated that capillary-dominated two-phase flow in porous media (spontaneous imbibition) can be uniquely characterized by the capillary diffusion coefficient (CDC) curve. This curve represents a mixed combination of flow properties of both phases:

% \begin{align}
% \Lambda = \mu_m \lambda_{nw} f_w \left( -\frac{dJ}{dS_w} \right)
% \label{eq:Lambda}
% \end{align}
% In this equation, \(\mu_m\) is the geometric mean of the phase viscosities \((\sqrt{\mu_w \mu_{nw}}\)). The CDC curve, as well as the dynamics of multiphase flow in porous media is mainly controlled by the relative permeability of the phases and the capillary pressure curves. Measurement of these curves is challenging and typically requires indirect methods, such as history matching using numerical simulations \citep{Krause2015AccurateCurves}. However, history matching in complex geometries, such as fractured porous media, is a challenging task that involves significant computational complexities. The challenge becomes more serious when high-fidelity datasets, such as CT-scan images, must be matched. In this work, we propose the application of PINNs as a reliable framework for history matching and characterisation of such problems. 


% \subparagraph{Known and Unknown Parameters. }
% To fully characterize the discussed system of equations, it is crucial to determine and understand the properties of both the matrix and the fractures. The determination of the some properties such as fluids properties, or average porosity and permeability of rock can be done using simpler methods. However, determination of the multiphase flow properties of the system - i.e., the relative permeability (\( k_r\)) and capillary pressure (\( p_c\)) of the matrix - is essential for accurately understanding the governing mechanisms, and this primarily requires multiphase experimental core flooding tests, in which the cylindrical rock is first saturated by a phase, then injected by the second phase at controlled pressures and flow rates. 
% The \( k_r\) curve can be fully addressed via six parameters related to the Corey model (equations (\ref{eq:krw_eq}) and (\ref{eq:krnw_eq})): \({k}_{rw}^{max}\), \({k}_{rnw}^{max}\), \(n_{w1}\) and \(n_{w2}\), \(n_{nw1}\) and \(n_{nw2}\). Also, the \( p_c\) curve can be characterized via \(J_{1}\) and \(J_{2}\) parameters, based on equation (\ref{eq:Jeq}). 

% Due to the small pore volume of the fractures, we can reasonably assume a constant fracture porosity. The fracture permeability (\(K_{F}\)), which significantly impacts the overall flow rate during the experiments, needs to be calculated. Additionally, for simplicity, we assumed linear relative permeability curves for fractures \citep{DeLaPorte2005TheReservoirs}. 




% \subsection{Methodology}

% Physics-Informed Neural Networks (PINNs) were introduced by \citet{Raissi2019Physics-informedEquations} as an efficient method for solving differential equations by combining neural networks with physics-based principles. In this study, we defined neural networks (separately for matrix (\( \mathcal{N}_m \)) and fracture (\( \mathcal{N}_f \)) domains), to emulate the functional dependency between the independent and dependent variables:

% \begin{align}
% {s}_{w},{p}_{nw} = \mathcal{N}^{M}(x,y,z,t,\theta,\eta)
% \label{eq:pceq}
% \end{align}
% \begin{align}
% {s}_{w}^{f},{p}_{nw}^{f} = \mathcal{N}^{F}(x_{f},y_{f},z_{f},t,\theta_{f},\eta)
% \label{eq:p1}
% \end{align}

% where, [\(x, y, z\)] and [\(x_f, y_f, z_f\)]   are the spatial coordinates corresponding to the collocation points of matrix and fracture, respectively. Also, \( \theta\) and \( \theta_f\) are the network trainable parameters.
% The goal is to solve an optimization problem where:
% \begin{align}
% \theta^{m,f},\eta = \arg\min(\mathcal{L}_{t})
% \label{eq:p2}
% \end{align}

% Here, \( \eta\) is the set of inverse parameters calculated during the inverse calculations. Also, \( \mathcal{L}_{t} \) is the total loss term, defined to minimize the errors in both the physical flow equations in the matrix and fracture, as well as the available observation data. The outlet of networks are the state variables of the system, which are the \(s_w\), and \(p_{nw}\). The total loss term is a weighted combination of matrix and fracture losses, as well as losses corresponding to observational data:


% \begin{align}
% \mathcal{L}_{t} = \mathcal{L}_{t}^{M} + \mathcal{L}_{t}^{F} + \mathcal{L}_{t}^{D} 
% \label{eq:p2}
% \end{align}

% where \(\mathcal{L}_{t}^{M}\) and \(\mathcal{L}_{t}^{F}\) are the total loss terms corresponding to the initial/boundary conditions, as well as the PDE residuals for matrix and fracture domains, respectively. Minimizing these terms ensures the PINNs solution respects the physical constraints within their domain.
% Furthermore, \(\mathcal{L}_{t}^{D}\) represents the total loss term corresponding to the errors in the predictions of PINNs compared to the observational data. The complete explanation of the PINNs implementation and the underlying loss terms is provided in Appendix \ref{sec:PINNsimplementation}.

% To address the inverse problem, we adopted an ansatz approach for representing the relative permeability and capillary pressure curves. This means a trainable vector was defined, where each element corresponded to a parameter within the chosen correlations for these curves (equations (\ref{eq:krw_eq}), (\ref{eq:krnw_eq}) and (\ref{eq:pceq})). More information regarding the initialization and definition of the inverse variables is provided in Appendix \ref{sec:PINNsComputationalstrat}. 



% \subsection{Model Architecture}
% The architecture of the applied PINNs model is shown in Fig. \ref{fig:2}.
% Due to the complexities in the geometry, and non-linearities in flow profiles, we considered the matrix and fracture systems as decomposed domains. Then, separate networks were allocated to each domain, to increase the flexibility of the networks in capturing the high-frequency trends in the solution of equations. Also, for each domain, the system state variables, i.e., pressure (\(p_{nw}\))  and water saturation (\(s_w\)) had separate networks (Fig. \ref{fig:2}b). Before passing the data to the network, the input data was normalised to the approximate range of (-1,1). The (de)normalization technique is discussed in Appendix \ref{sec:PINNsComputationalstrat}. 
% In the NNs corresponding to the \(S_w\) values (for both matrix and fracture), we used the following sequence of operators: an encoder, a Fourier transformer, a latent multilayer perceptron (MLP) network, an inverse Fourier transformer, and a decoder network (as shown in Fig. \ref{fig:2}c). The outlet of the NNs is then denormalized to the range of actual values. The Fourier transformers were used to make the networks able to capture the high-frequency or multi-scale behavior \citep{Wang2021OnNetworks} in the frontal regions of the saturation profiles. The NNs for the calculation of \(p_{nw}\) were similar, except that the Fourier and inverse Fourier transformations were not applied. The MLP network, which had a depth of five and a width of 80 neurons, was activated by an adaptive \(tanh\) activation function. 
% The model was initialized using the Glorot initialization scheme \citep{Glorot2010UnderstandingNetworks}. Separate MLP networks were used to address the self-adaptive local weighting of the errors in PDE residuals for matrix and fracture domains. See Appendices \ref{sec:PINNsimplementation} and \ref{sec:PINNsComputationalstrat} for more details.

% \subparagraph{Training:} 
% The network was trained utilizing an Adam optimizer employing a full-batch approach and incorporating a gradually decreasing learning rate, from 0.0003, to 0.0001. We have applied a weight decay value of 0.0001. The number of gradient descent training steps (epochs) depended on the problem's complexity. Typically, 15,000 to 25,000 epochs were needed for stable error values. 



% \input{tables/table_app2}


% \subsection{The Solution Approach} 
% \label{sec:SolutionMethod}
% The investigated system of equations governing the matrix and fracture domains exhibits a complex interdependency.  In this context, training the model using a fully-coupled approach generates chaotic computational behavior as the interaction terms between the matrix and fracture domains are highly sensitive to the accuracy of the calculations performed in each domain individually. In the other hand, the invasion of fluids from the fracture into the matrix domain is a strong function of the values of the interaction terms. Crucially, the differing loss landscapes of the matrix and fracture PINNs models result in distinct convergence behaviors. To mitigate these issues, alternative preconditioning techniques are necessary \citep{Krishnapriyan2021CharacterizingNetworks}. In this work, we suggested to apply a sequence of pre-training training steps before performing the fully-coupled simulations. The details of the applied approach is visualized in Fig. \ref{fig:2}e. In this process, at first, the matrix and fracture networks are trained individually, without utilizing any coupled inter dependencies. Then, we shift to the fully-coupled training technique. 

% However, the utilisation of the pre-training technique, although considers many of the possible flow mechanisms, however, neglects the impact of mechanisms such as viscous flow interactions between the matrix and fracture. The difference gets more critical when the permeability and capillary variation in matrix and fracture media is less significant. The mentioned mechanisms are naturally considered in the fully coupled approach. So, after pre-training of the networks, and reaching an equilibrium in the training process, we switch to the fully coupled technique. The mathematics behind coulping the matrix and fracture is previously explained in section \ref{sec:mathematicsofphysics}. 


% \subparagraph{Pre-training:} This stage leverages the model reduction technique \citep{Chung2017CouplingApproaches} as a means to tackle multiscale problems. To do so, we applied an independent training strategy for matrix and fracture at the beginning of training, before shifting to the fully-coupled training strategy. In this approach, instead of defining the matrix-fracture transfer to modify the PDEs of flow, we explicitly applied their impacts as the boundary conditions in the matrix. In this case: 

% \begin{itemize}
% \item Matrix: The multiphase flow in the matrix is analyzed by assuming that the \(s_w\)  and the \(p_{nw}\) in the matrix at points of intersection with fractures are equal to the corresponding values in the fractures.
% \begin{align}
% s_w = s_{w}^{F,BL},\ \ \ \ {\in\Omega}_{MF} \label{eq:pretrsw}
% \end{align}
% \begin{align}
% p_{nw} = p_{nw}^{F,BL},\ \ \ \ {\in\Omega}_{MF} \label{eq:pretrpnw}
% \end{align}

% \(s_{w}^{F,BL}\) is calculated using the 1D Buckley-Leverett (BL) theory, and \(p_{nw}^{F,BL}\)  is calculated using linear pressure distribution assumption. The Buckley-Leverett theory offers a fundamental analytical approach for forecasting the saturation profile and front velocity of the displacing fluid in two-phase flow in porous media. The BL theory is explained in Appendix  \ref{sec:BLequation}. 
% \item Fracture: The PINNs model corresponding to the PDE of multiphase flow in fractures is solved by ignoring the interactions with matrix. 
% \end{itemize}

% In the case of inverse calculations, before starting the optimization of inverse variables, it is essential to partially train the networks so that they can learn the main characteristics of the problem. This approach has been successfully applied in previous studies, such as those by \citet{Zhang2022AnalysesNetworks} and \citet{Abbasi2024ApplicationTests}. At this step, the trainable inverse parameters are kept frozen for some limited apochs. 


% \input{tables/table_dlnetwork}






% \subsection{Experimental Data}
% \label{sec:experimentaldata}
% The study evaluated experimental data from injecting water into a  CO\textsubscript{2}-saturated fractured shale rock core, as detailed in \cite{Kurotori2023MixedMedia}. The cylindrical Wolfcamp shale core had a length of 5.8 cm, diameters of 2.5 cm, an average permeability of \(1.97e-17\) m$^2$ (0.020 mD) and porosity of 0.102. The core was initially saturated with CO\textsubscript{2}, then water was injected at 530 psi injection pressure and 460 psi backpressure for 311 hours while confined at 700 psi. Dynamic CT images were captured at intervals, recording in-situ saturation, phase recovery, and injected fluid volume over time. Different fractures were identified from the CT scan images. History matching and inverse calculations in this study relied on several key experimental measurements (also see Fig. \ref{fig:colls}e):

% \begin{itemize}
% \item\textbf{Recovery Factor (RF)}: the volume fraction of the pore space displaced by the injected fluid over time. We calculated the RF curve by averaging the saturation of the wetting phase fluid obtained from CT scan images.
% \item\textbf{Boundary Conditions}: The constant pressure at the inlet and outlet boundaries were known based on the experimental setup.
% \item\textbf{Injection Volume}: The total volume of water injected into the system as a function of time was directly measured.
% \item\textbf{Spatial Saturation Data}: Spatial distribution of fluid saturation within the sample at different times, obtained through CT scans.
% \end{itemize}

% More details on the data sets used in this study and their use within the PINNs framework can be found in Appendix \ref{sec:PINNsimplementation}2.



% \subsection{Collocation Points}
% As it is visualized in Fig. \ref{fig:colls}, collocation points were extracted separately for the matrix and fracture domains based on the CT/micro-CT scan coordinates. 23500 matrix spatial collocation points were used in the core cylinder domain at specified x, y, z resolutions, excluding points in superposition with fractures. Boundary collocation points were collected for the cylinder ends and radius. Fracture collocation points were manually extracted from micro-CT scans. Temporal collocation points were randomly selected based on the \(\sqrt{t}\) distribution intervals, as it is expected that the system is mainly controlled by spontaneous imbibition mechanism. \cite{Abbasi2023SimulationNetworks} have shown how the selection of temporal points based on \(\sqrt{t}\) distribution intervals helps in improving PINNs solutions. More detailed information about the experimental data and the collocation points are provided in Appendix \ref{sec:PINNsCollocation Points}.





% \begin{figure}[htbp]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=.99\textwidth]%
%     {graphics/colls.jpg}% picture filename
% \end{center}
% \caption{ \textbf{The collocation points have been used for solving the problem under study.} The color of the points demonstrate the corresponding time for each point in the range \(t=1-10^6 \) sec. \textbf{a)} The collocation points at the boundary conditions of inlet (y=0) and outlet (y=L) faces (940 spatial points), \textbf{b)} The collocation points corresponding to the non-flowing boundary condition at \(r=r_{c}\) (8630 spatial points), \textbf{c)} The collocation points corresponding to the fracture (4103 spatial points), \textbf{d)} The collocation points corresponding to the matrix (23500 spatial points). The matrix collocation points with distance less than 0.0006 m from the fracture collocation points have been removed. \textbf{e)} the observational data points used in the data loss: 1) RF points, 2) points with the measured injected volume, and 3) spatiotemporal points of the in-situ \( s_w\) measured using CT-scan. }
% \label{fig:colls}
% \end{figure}






% \section*{Acknowledgments}
% Abbasi, Andersen, and Hiorth acknowledge the Research Council of Norway and the industry partners of NCS2030 – RCN project number 331644 – for their support.


% \bibliography{mendeley} 
% \printbibliography

% \input{suppl}

% \end{document}

% % \section*{Appendix: Numerical simulations }
% % We have utilized a finite-difference simulation approach to simulate the 








==> changes/main1.tex <==
% \documentclass[12pt]{article}
% \usepackage{graphicx}
% \usepackage{titlesec}
% \usepackage[hyperfootnotes=true]{hyperref}
% \hypersetup{colorlinks, citecolor=blue, linkcolor=blue, urlcolor=blue}
% \usepackage{makecell}
% \renewcommand{\cellalign}{vh}
% \usepackage{hyperref}%
% \usepackage{color,soul}
% \usepackage{amsmath}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \newcommand{\CO}{\text{CO\textsubscript{2}}
% \usepackage{changes}

% \providecommand{\keywords}[1]
% {\small	
% \textbf{\textit{Keywords---}} #1}
% \usepackage{geometry}
% \geometry{ a4paper, total={170mm,257mm}, left=25mm, right=25mm, top=25mm, bottom=25mm, }
% \graphicspath{{figs/}}
% \usepackage{caption}
% \ucharacterisationinputenc}

% \usepackage{natbib} 
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{eqns}  % Use the equations
% % \captionsetup{font=small}
% \usepackage{xcolor}




% \title{Physics-Informed Neural Networks (PINNs) Solver for History Matching of Multi-Phase Flow in Multi-Scale Fractured Porous Media}

% % \title{History Matching of Multi-Phase Flow in Fractured Porous Media using Physics-Informed Neural Networks (PINNs)}
% \author{ ...}
% \date{June 2024}


% \begin{document}
% \maketitle




% \begin{abstract}
% In this work, we utilize physics-informed neural networks (PINNs) to model, and  history-match multiphase flow in fractured porous media experiments. First, we apply PINNS to a  numerical benchmark problem, thereafter we apply PINNs to a real experimental dataset where water is injected at constant pressure drop into a CO$_2$ saturated shale core plug. The core plug was naturally fractured in different directions. The exact spatial position of fractures and dynamic in-situ distribution of fluids were imaged using a CT-scan setup. 

% To model the heterogenous porous media we have followed a domain decomposition approach for matrix and fractures; and a multi-network architecture for the separate calculation of water saturation and  pressure. Loss terms are defined for the flow equations in both the matrix and fractures. These equations also account for their corresponding boundary and initial conditions, as well as mass transfer between the matrix and fractures. To enable the PINNs model to accurately capture the physical properties of the system, we proposed a pre-training strategy, before fully-coupled simulations.

% Both for the benchmark and experimental system, by simultaneous matching of recovery and volumetric injection data, we determined flow parameters within the matrix and the fractures. Multiple random initialization were performed to assess the uncertainty and uniqueness of the calculations, showed the reliability of the solutions. The PINNs model successfully captured the essential physical mechanisms, including viscous and imbibition flow in both domains, as well as counter-current and co-current imbibition phase transfer between the matrix and fracture. 
% Our results demonstrate that PINNs are  capable to simulate and identifying parameters (history match) complex, multi-scale multi phase flow systems. 


% Furthermore, applying PINNs to solve the mathematical model it is possible to develop a solver that is orders of magnitude faster for inverse problems, more flexible in handling multi-fidelity datasets, and involves fewer implementation difficulties compared to classical finite volume or finite difference methods.



% \end{abstract}


% \keywords{ keywords: Physics-Informed Neural Networks (PINNs), \and multiphase flow, \and inverse calculations, \and multiscale fractured porous media}



% \section{Introduction}


% Simulating multi-phase flow phenomena in fractured porous media, as a highly multiscale coupled problem, is challenging because flow in the matrix and fractures behave significantly different in realistic scenarios \citep{Fung1991SimulationReservoirs}. A multiscale process refers to a system that exhibits a variational behavior across scales, where the processes at each scale influence the overall behavior of the system \citep{Geers2017HomogenizationProblems}. The characterization of multiphase flow in porous media commonly is performed via inverse calculation of the model parameters through history matching of the experimental data. 

% Almost all natural porous media are to some degree fractured, however, an inaccurate representation of fracture influence on multiphase flow phenomena can lead to substantial errors. These errors can propagate from microscale force balance estimations to macroscale predictions of porous media behavior, significantly impacting applications such as geological carbon storage, fluid flow in aquifers, and recovery of hydrocarbons \citep{Rangel-German2006Multiphase-flowMedia}. However, most common approaches for estimating multiphase flow properties in porous media are developed for homogeneous systems with 1D frontal behavior, making them unsuitable for multiscale problems.

% The modeling of coupled matrix and fracture multiphase flow systems requires specialized techniques and approaches to model and simulate \citep{Odster2019AMedia}. Fractures introduce discontinuities in the flow field, which can lead to numerical instabilities and reduced accuracy in traditional numerical methods. Additionally, the need for fine discretization of the domain to capture these discontinuities results in high computational costs \citep{Bastian2000NumericalMedia}.
% In the last years, various numerical methods based on finite-element and finite-volume approaches have been recommended to solve the problem more efficiently \citep{Komijani2023AnCoupling, Myner2016AGrids}. However, the implementation of the algorithms is complex, and the numerical scheme typically face challenges such as high computational requirements and low convergence reliability \citep{Yang2021RecentMedia}. In the practical applications, the influence of fractures is often neglected or modeled using simplified assumptions, e.g., by defining the matrix as the high permeable and heterogeneous zone \citep{Berre2019FlowApproaches}. However, in many cases, such as shale rocks, neglecting or simplifying the influence of fractures becomes impractical due to their significant impact on fluid flow behavior. Given these limitations, there is a persistent demand for the development of more precise and computationally efficient prediction tools. Furthermore, the advancements in imaging technologies over recent years have made it possible to visualize fluid dynamics within porous media at an experimental scale \citep{Tekseth20244DTomography}. High-resolution data, while valuable, often presents a significant challenge for history matching. This, combined with the inherent complexity of multi-scale and coupled interactions in fractured porous media, can leave traditional history matching of core-flooding experiments practically infeasible. So, the development of more reliable mathematical solvers in this area are particularly valuable for improving the efficiency of inverse calculations, which typically take orders of magnitude longer to solve than forward problems using classic numerical methods. 

% PINNs have emerged as a data-driven technique, seamlessly integrating both high-fidelity and noisy datasets and domain expertise to solve the differential equations governing various engineering and scientific problems \citep{Raissi2019Physics-informedEquations}. More specifically, it has shown potential to solve problems of multiphase flow in porous media in forward or inverse modes \citep{Latrach2024ASystems}, e.g., modeling of counter-current spontaneous imbibition \citep{Abbasi2023SimulationNetworks}, solving multiphysics coupled flow problems\citep{Amini2023InverseNetworks} and modeling of density driven flow in porous media for CO$_2$ storage \citep{Du2023ModelingSequestration}. However, studies are primarily focused on systems with homogeneous propertiess, often overlooking systems with multiscale features. The application of PINNs to multiscale problems is actively researched across various disciplines, with a variety of recommended techniques emerging in recent years \citep{Alber2019IntegratingSciences}. 
% For instance, \citet{Wang2021OnNetworks}, for the problems such as wave propagation and Poisson equation, proposed using Fourier feature embedding to capture the behavior of system at both various spatial scales, and avoiding the potential spectral biases in the PINNs predictions. Spectral bias is defined as the tendency of networks to learn the solutions with the lowest possible frequencies. \citet{Weng2022MultiscaleKinetics}  proposed multiscale PINNs for modeling of stiff chemical kinetics. They utilized different NNs with similar architectures for the different scales of magnitudes of reaction rate. \citet{Riganti2023AuxiliaryProblems} applied a multi-output PINNs with multiple auxiliary variables associated and the Legendre terms to solve the Boltzmann equation efficiently. \citet{Moseley2023FiniteEquations} introduced Finite-Basis PINNs, by decomposing the domains of the problems, e.g., (2+1)D wave propagation equations, using a finite-set of basis functions, inspired by finite-element methods. However, despite existing efforts, the literature shows significant gaps in applying PINNs for solving the multiphase flow in naturally fractured porous media, as a strategy for forward modeling and inverse parameter identification. 

% In this work, we have implemented a multi-scale PINNs architecture for 3D simulation of multiphase flow in fractured porous media and inverse calculation of flow parameters by history matching experimental-scale observed datasets. After validation of the model using a synthetic dataset, we have investigated an experimental problem of water flooding in a CO$_2$ saturated fractured shale rock \citep{Kurotori2023MixedMedia}. We have also incorporated in-situ saturation data measured using a 3D high-resolution CT-scan setup in the calculations. The results presented here for the first time demonstrates the application of PINNs as a reliable and optimal tool for the purpose of inverse analysis of the multi-fidelity experimental datasets corresponding to the multi-phase flow in fractured porous media.

% This work continues by outlining the mathematical concepts governing multiphase flow in fractured porous media. Subsequently, we elaborate on the specifics of the implemented PINNs framework. To assess the PINNs' capabilities before tackling the main experimental problem, we employed a synthetic benchmark model. This benchmark serves as a well-defined system of two-phase flow within a fractured porous media matrix. Finally, we evaluated the PINNs' performance across various scenarios of utilizing the experimental dataset, and analyzed the importance of multi-scale simulation of the problem under-study.





% \section{Mathematics of Flow in Fractured Porous Media}
% \label{sec:mathematicsofphysics}

% We approach a problem of 3D multiphase flow in a fractured porous media at core-scale. 
% Our focus is specifically on interpreting data from a cylindrical core-plug experiment (rock taken from the Wolfcamp formation) \citep{Kurotori2023MixedMedia}. We refer to the low-permeable non-fractured zone as matrix, and the high-permeable fractured zone as a fracture. The model is infered from the definition that the matrix domain \((\Omega_M)\) occupies the majority of the pore volume and that fractures domain \((\Omega_F)\) have a much higher permeability than the matrix. A schematic of the geometry of the core and the fractures is visualized in Fig. \ref{fig:coreschematic}. 
% The core is placed horizontally, and the fractures are distributed in the core with different orientations. The radial surface of the core at \(r_c\) is closed (no-flow boundary). The inlet and outlet faces are at \(y=0\)  and \(y=L\), respectively.  Water and CO\textsubscript{2} are considered to be the wetting \((w)\) and non-wetting \((nw)\) phases, respectively. In line with the experimental conditions, we neglected both the compressibility and the solubility of the phases. The system is initially saturated with the \(nw\) phase. The definition of the system implies that the flow phenomena are governed by mixed-imbibition mechanisms, where the fracture flow is driven by forced imbibition and the matrix flow is governed by spontaneous imbibition between the fracture(s) and the matrix. Forced imbibition happens when an external force drives the wetting phase fluid through the porous media, overcoming any resistance from the medium and the non-wetting phase. Spontaneous imbibition, on the other hand, is the process in which the wetting phase fluid flows into a porous media via capillary forces without the need of external pressure \citep{Anderson1987WettabilityPressure}. In the following, the mathematics of flow in matrix and fracture domains are discussed.

% \subparagraph{Matrix Flow: }
% The Darcy flow velocity (\(u_i\)) of each phase in matrix is determined by Darcy's law:

% \begin{equation}
% u_i=-\lambda_i\left \nabla p_i\right,\ \ \lambda_i=\frac{Kk_{ri}}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy}
% \end{equation}

% where \(\lambda_i\) is mobility, \(p_i\) is the phase pressure, \(K\) and \(k_{ri}\) are absolute permeability and relative permeability, respectively, and \(\mu_i\) is the phase viscosity. The index \(i\) determines\((w)\), and \((nw)\) phases. The effects of gravity have been ignored. The conservation law for the spatiotemporal mass transportation of phases in matrix  zone, is defined as:

% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right),\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_cont}
% \end{align}


% Given that \({s}_{wc}=0\), we define the initial conditions as:

% \begin{align}
% \left\{\begin{array}{left} {s}_{w}(x,y,z,t = 0) = 0\\ {p}_{nw}(x,y,z,t = 0) = {p}_{i} \\  \end{array}\right \ \ \ {, \in\Omega}_M
% \label{eq:eqICmatrix}
% \end{align}

% At the inlet face ($y=0$), the wetting phase is injected under a constant pressure ${p}_{in}$ over time. At this face, it is assumed the wetting phase takes the highest possible mobility:

% \begin{align}
% \left\{\begin{array}{left} {s}_{w}(x,y = 0,z,t) = 1 - {s}_{nwr} \\ {p}_{w}(x,y = 0,z,t) = {p}_{in} \\  \end{array}\right 
% \label{eq:eqBC0matrix}
% \end{align}

% The production from the outlet face \((y=l)\) occurs at a constant pressure, \({p}_{out}\):
% \begin{align}
% {p}_{nw}(x,y = L,z,t) = {p}_{out} 
% \label{eq:eqBC1matrix}
% \end{align}
% At the outlet face of the core, no explicit constraints are imposed on the saturation of the fluid phases. The radial faces \((r = r_c)\) are sealed from flow in radial directions:

% \begin{align}
% \left. \frac{\partial p}{\partial r} |_{r = r_c} \approx \frac{\partial p}{\partial x} |_{r = r_c} + \frac{\partial p}{\partial z} |_{r = r_c} = 0 \right
% \label{eq:eqBC1matrix}
% \end{align}

%  The assumed matrix properties state that the flow in the matrix is governed by viscous and capillary forces (gravity effects are assumed to be negligible). 


% \subparagraph{Fracture Flow: }
%  A fracture is typically characterized as a narrow, and high permeable zone enclosed by a less permeable matrix zone. This contrast in properties leads to highly heterogeneous flow behavior across the scales. The aperture between the fracture surfaces is generally small and is normally occupied by filling materials, which affects its effective porosity and permeability values \citep{Wu2016MultiphaseMedia}. 

% Although fractures are discontinuities in the porous medium, they can be considered as a separate porous medium domain \((\Omega_F)\). This assumption enables us to apply Darcy's law. 
% Consequently, we assume fractures to be high permeable porous zones. This makes the equations in the two media consistent, eliminating the need for unnecessary complexities in the calculations \citep{Martin2005ModelingMedia}. So, the average flux of each flowing phase in a fracture is written by modification of Darcy's law in eq. \ref{eq:darcy}:
  
 
% \begin{equation}
% v_i^{\parallel}=-\lambda_i^{\parallel} \nabla^\parallel p_i ,\ \ \lambda_i^\parallel=\frac{K^F k_{ri}^\parallel}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy_frac}
% \end{equation}

% In this equation, \(K_F\) is the fracture permeability, and \(k_{ri}^\parallel\) is the relative permeability of the fluids in the fracture. The value of the \(K_F\) is dependant on the fracture aperture, and also the extent of the filling materials in the fracture. 


% \subparagraph{Matrix-Fracture Interactions: }

% The accurate treatment of multiphase flow in a fractured porous media depends on the modeling of the dynamic matrix-fracture coupled interactions. Utilizing Darcy's law, the matrix-fracture flux is approximated by \cite{Berre2019FlowApproaches}:

% \begin{align}
% v_i^\bot=-2K^\bot\lambda_i^\bot\left[\frac{ p_{M,i}-p_{F,i} }{e_V}\right],\ \ \lambda_i^\bot \simeq \frac{k_{ri}}{\mu_i},\ \ \left(i=w,nw\right), \label{eq:e8}
% \end{align}

% Where \(K^\bot\) is the matrix-fracture permeability normal to the fracture surface, and \(e_V\) is the fracture average aperture. As an ideal case, if one assumes fracture as an open space between two parallel surfaces, then the aperture is called hydraulic aperture, \(e_h\). In practice, the value of \(e_v\) is much larger than  \(e_h\), i.e., \(e_v>>e_h\), as the fractures are normally filled with materials. The value of \(K_F\) is theoretically correlated to \(e_v\). In this study, the fracture aperture, \(e_v\), is assumed to be 0.001 m for all the fractures, and kept constant in all the evaluations. The cumulative value \( V_i^\bot(t)  \) of a rate \( v_i^\bot(t)  \) over time is given by the integral:

% \begin{align}
% V_i^\bot(t) = \int_0^t v_i^\bot(\tau) \, d\tau
%  ,\ \ \left(i=w,nw\right), \label{eq:cumv}
% \end{align}

% We can rewrite Eq. \ref{eq:e8} to obtain the mass transfer rate [kg/m\(^3\)/s] between the two media:

% \begin{align}
% q_i^\bot=\frac{2\rho_i}{e_V} v_i^\bot ,\ \ \left(i=w,nw\right), \label{eq:massrate}
% \end{align}
% The factor 2 denotes the flow across both sides of fracture to matrix, assuming the equal flow characteristics across the two surfaces of the fracture. Then, the cumulative mass rate [kg/m\(^3\)] is:
% \begin{align}
% Q_i^\bot(t) = \int_0^t q_i^\bot(\tau) \, d\tau
%  ,\ \ \left(i=w,nw\right), \label{eq:massratecum}
% \end{align}




% The equation of mass conservation in the fracture is the same as in the matrix, with an additional term representing the mass from the fracture to the matrix \( q_i^\bot \). So, by modifying the matrix mass balance equation (Eq. \ref{eq:matrix_cont}), we define the mass balance in the fracture system:

% \begin{align}
% \phi^F\partial_t\left(\rho_is_{i}^{F}\right)=-\nabla^\parallel\left(\rho_iu_i^\parallel\right)\ -q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_F \label{eq:massbalF}
% \end{align}

  
% At the contact point of the matrix and fractures, the continuity equation should also be solved in the matrix domain. So, we may rewrite eq. \ref{eq:matrix_cont} as: 


% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right)+q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_frac_cont}
% \end{align}


% The fraction of the pore volume of the matrix [dimensionless] that has been transferred between the matrix and fracture can also be calculated using the following equation:

% \begin{align}
% V_i^\bot(t) = \frac{Q_i^\bot(t)}{\phi \rho_i},\ \ \left(i=w,nw\right), \label{eq:dimenlessPVMF}
% \end{align}




% \subparagraph{Closure Equations: }
% Capillary pressure and relative permeability curves are crucial input to model multiphase flow in porous media, e.g., in eqs. \ref{eq:matrix_cont}, \ref{eq:massbalF} and \ref{eq:matrix_frac_cont}. These curves are normally defined using theoretical correlations, with a few matching parameters. In this work, we apply an extended version of the Corey function \citep{Corey1954ThePermeabilities} to model relative permeability curves:


% \begin{align}
% {k}_{rw}({S}_{w}) = {k}_{rw}^{max}({S}_{w})^{{n}_{w}};\ \ \ \ \ \ {n}_{w} = {n}_{w1}{S}_{w} + {n}_{w2}(1 - {S}_{w}) \label{eq:krw_eq}
% \end{align}
% \begin{align}
% {k}_{rnw}({S}_{w}) = {k}_{rnw}^{max}(1 - {S}_{w})^{{n}_{nw}};\ \ \ \ \ \ {n}_{nw} = {n}_{nw1}{S}_{w} + {n}_{nw2}(1 - {S}_{w})
% \label{eq:krnw_eq}
% \end{align}

% In the extended version, \(n_w\) and \(n_{nw}\) are defined as saturation exponents that are weighted linearly with saturation \(S_w\). \(S_w\) is the normalized water saturation and is calculated as:

% \begin{align}
% {S}_{w} = \frac{{s}_{w} - {s}_{wc}}{1 - {s}_{nwr} - {s}_{wc}};
% \label{eq:Sweq}
% \end{align}

% The capillary pressure curve \(P_c(S_w)\) [pa] is calculated via Leverett scaling \citep{Leverett1942Dimensional-modelBehavior}:

% \begin{align}
% P_c = \sigma \sqrt{\frac{\phi}{K}} J
% \label{eq:pceq}
% \end{align}

% In this context, J(S$_w$) represents the Leverett J-function, a dimensionless function that describes the shape of the capillary pressure curve. We define J-function via the modified \citet{Bentsen1977UsingCurve} correlation:

% \begin{align}
% J(S_w) =  - {J}_{1}\mathrm{\ln}(\frac{{S}_{w}}{{S}_{eq}}) + {J}_{2}\mathrm{\ln}(\frac{1 - {S}_{w}}{1 - {S}_{eq}})
% \label{eq:Jeq}
% \end{align}

% The equation is hard constrained in a way that that \(J(S_{eq})=0\) and that \(dJ/dS_w\)   becomes infinite at endpoints. 

% However, previous research by \cite{Andersen2023Early-andCoefficient} demonstrated that capillary-dominated two-phase flow in porous media (spontaneous imbibition) can be uniquely characterized by the capillary diffusion coefficient (CDC) curve. This curve represents a mixed combination of flow properties of both phases:

% \begin{align}
% \Lambda = \mu_m \lambda_{nw} f_w \left( -\frac{dJ}{dS_w} \right)
% \label{eq:Lambda}
% \end{align}
% In this equation, \(\mu_m\) is the geometric mean of the phase viscosities \((\sqrt{\mu_w \mu_{nw}}\)). The CDC curve, as well as the dynamics of multiphase flow in porous media is mainly controlled by the relative permeability of the phases and the capillary pressure curves. Measurement of these curves is challenging and typically requires indirect methods, such as history matching using numerical simulations \citep{Krause2015AccurateCurves}. However, history matching in complex geometries, such as fractured porous media, is a challenging task that involves significant computational complexities. The challenge becomes more serious when high-fidelity datasets, such as CT-scan images, must be matched. In this work, we propose the application of PINNs as a reliable framework for history matching and characterisation of such problems. 


% \subparagraph{Known and Unknown Parameters: }
% To fully characterize the discussed system of equations, it is crucial to determine and understand the properties of both the matrix and the fractures. The determination of the some properties such as fluids properties, or average porosity and permeability of rock can be done using simpler methods. However, determination of the multiphase flow properties of the system - i.e., the relative permeability (\( k_r\)) and capillary pressure (\( p_c\)) of the matrix - is essential for accurately understanding the governing mechanisms, and this primarily requires multiphase experimental core flooding tests. in which the cylindrical rock is first saturated by a phase, then injected by the second phase at controlled pressures and flow rates. 
% The \( k_r\) curve can be fully addressed via six parameters related to the Corey model (eqs. \ref{eq:krw_eq} and \ref{eq:krnw_eq}): \({k}_{rw}^{max}\), \({k}_{rnw}^{max}\), \(n_{w1}\) and \(n_{w2}\), \(n_{nw1}\) and \(n_{nw2}\). Also, the \( p_c\) curve can be characterized via \(J_{1}\) and \(J_{2}\) parameters, based on eq. \ref{eq:Jeq}. 

% Due to the small pore volume of the fractures, we can reasonably assume a constant fracture porosity. The fracture permeability (\(K_{F}\)), which significantly impacts the overall flow rate during the experiments, needs to be calculated. Additionally, for simplicity, we assumed linear relative permeability curves for the fractures \citep{DeLaPorte2005TheReservoirs}. 



% \begin{figure}[ht]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=1\textwidth]%
%     {graphics/Fig1.jpg}% picture filename
% \end{center}
% \caption{ a) The simplified geometry of the matrix-fracture system and the impacting boundary conditions. b) the spatial distribution of the detected fractures in the core.  }
% \label{fig:coreschematic}
% \end{figure}



% \section{Methodology}

% Physics-Informed Neural Networks (PINNs) were introduced by \cite{Raissi2019Physics-informedEquations} as an efficient method for solving differential equations by combining neural networks with physics-based principles. In this study, we defined neural networks (separately for matrix (\( \mathcal{N}_m \)) and fracture (\( \mathcal{N}_f \)) domains), to emulate the functional dependency between the independent and dependent variables:

% \begin{align}
% {s}_{w},{p}_{nw} = \mathcal{N}^{M}(x,y,z,t,\theta,\eta)
% \label{eq:pceq}
% \end{align}
% \begin{align}
% {s}_{w}^{f},{p}_{nw}^{f} = \mathcal{N}^{F}(x_{f},y_{f},z_{f},t,\theta_{f},\eta)
% \label{eq:p1}
% \end{align}

% where, [\(x, y, z\)] and [\(x_f, y_f, z_f\)]   are the spatial coordinates corresponding to the collocation points of matrix and fracture, respectively. Also, \( \theta\) and \( \theta_f\) are the network trainable parameters.
% The goal is to solve an optimization problem where:
% \begin{align}
% \theta^{m,f},\eta = \arg\min(\mathcal{L}_{t})
% \label{eq:p2}
% \end{align}

% Here, \( \eta\) is the set of inverse parameters calculated during the inverse calculations. Also, \( \mathcal{L}_{t} \) is the total loss term, defined to minimize the errors in both the physical flow equations in the matrix and fracture, as well as the available observation data. The outlet of networks are the state variables of the system, which are the \(s_w\), and \(p_{nw}\). The total loss term is a weighted combination of matrix and fracture losses, as well as losses corresponding to observational data:


% \begin{align}
% \mathcal{L}_{t} = \mathcal{L}_{t}^{M} + \mathcal{L}_{t}^{F} + \mathcal{L}_{t}^{D} 
% \label{eq:p2}
% \end{align}

% where \(\mathcal{L}_{t}^{M}\) and \(\mathcal{L}_{t}^{F}\) are the total loss terms corresponding to the initial/boundary conditions, as well as the PDE residuals for matrix and fracture domains, respectively. Minimizing these terms ensures the PINNs solution respects the physical constraints within their domain.
% Furthermore, \(\mathcal{L}_{t}^{D}\) represents the total loss term corresponding to the errors in the predictions of PINNs compared to the observational data. The complete explanation of the PINNs implementation and the underlying loss terms is provided in Appendix \ref{sec:PINNsimplementation}.

% To address the inverse problem, we adopted an ansatz approach for representing the relative permeability and capillary pressure curves. This means a trainable vector was defined, where each element corresponded to a parameter within the chosen correlations for these curves (eqs.  \ref{eq:krw_eq}, \ref{eq:krnw_eq} and \ref{eq:pceq}). More information regarding the initialization and definition of the inverse variables is provided in Appendix \ref{sec:PINNsComputationalstrat}. 



% \subsection{Model Architecture}
% The architecture of the applied PINNs model is shown in Fig. \ref{fig:2}.
% Due to the complexities in the geometry, and non-linearities in flow profiles, we considered the matrix and fracture systems as decomposed domains. Then, separate networks were allocated to each domain, to increase the flexibility of the networks in capturing the high-frequency trends in the solution of equations. Also, for each domain, the system state variables, i.e., pressure (\(p_{nw}\))  and water saturation (\(s_w\)) had separate networks (Fig. \ref{fig:2}b). Before passing the data to the network, the input data were normalized to the approximate range of (-1,1). The (de)normalization technique is discussed in Appendix \ref{sec:PINNsComputationalstrat}. 
% In the NNs corresponding to the \(S_w\) values (for both matrix and fracture), we used the following sequence of operators: an encoder, a Fourier transformer, a latent multilayer perceptron (MLP) network, an inverse Fourier transformer, and a decoder network (as shown in Fig. \ref{fig:2}c). The outlet of the NNs is then denormalized to the range of actual values. The Fourier transformers were used to make the networks able to capture the high-frequency or multi-scale behavior \citep{Wang2021OnNetworks} in the frontal regions of the saturation profiles. The NNs for the calculation of \(p_{nw}\) were similar, except that the Fourier and inverse Fourier transformations were not applied. The MLP network, which had a depth of five and a width of 80 neurons, was activated by an adaptive \(tanh\) activation function. 
% The model was initialized using the Glorot initialization scheme \citep{Glorot2010UnderstandingNetworks}. Separate MLP networks were used to address the self-adaptive local weighting of the errors in PDE residuals for matrix and fracture domains. See Appendices \ref{sec:PINNsimplementation} and \ref{sec:PINNsComputationalstrat} for more details.

% \subparagraph{Training:} 
% The network was trained utilizing an Adam optimizer employing a full-batch approach and incorporating a gradually decreasing learning rate, from 0.0003, to 0.0001. We have applied a weight decay value of 0.0001. The number of gradient descent training steps (epochs) depended on the problem's complexity. Typically, 15,000 to 25,000 epochs were needed for stable error values. 

% \subsection{The Solution Approach} 
% \label{sec:SolutionMethod}
% The investigated system of equations governing the matrix and fracture domains exhibits a complex interdependency.  In this context, training the model using a fully-coupled approach generates chaotic computational behavior as the interaction terms between the matrix and fracture domains are highly sensitive to the accuracy of the calculations performed in each domain individually. In the other hand, the invasion of fluids from the fracture into the matrix domain is a strong function of the values of the interaction terms. Crucially, the differing loss landscapes of the matrix and fracture PINNs models result in distinct convergence behaviors. To mitigate these issues, alternative preconditioning techniques is necessary \citep{Krishnapriyan2021CharacterizingNetworks}. In this work, we suggested to apply a sequence of pre-training training steps before performing the fully-coupled simulations. The details of the applied approach is visualized in Fig. \ref{fig:solmethod}. In this process, at first, the matrix and fracture networks are trained individually, without utilizing any coupled interdependencies. Then, we shift to the fully-coupled training technique. 

% However, the utilisation of the pre-training technique, although considers many of the possible flow mechanisms, however, neglects the impact of mechanisms such as viscous flow interactions between the matrix and fracture. The difference gets more critical when the permeability and capillary variation in matrix and fracture media is less significant. The mentioned mechanisms are naturally considered in the fully coupled approach. So, after pre-training of the networks, and reaching an equilibrium in the training process, we switch to the fully coupled technique. The mathematics behind coulping the matrix and fracture is previously explained in section \ref{sec:mathematicsofphysics}. 


% \subparagraph{Pre-training:} This stage leverages the model reduction technique \citep{Chung2017CouplingApproaches} as a means to tackle multiscale problems. To do so, we applied an independent training strategy for matrix and fracture at the beginning of training, before shifting to the fully-coupled training strategy. In this approach, instead of defining the matrix-fracture transfer to modify the PDEs of flow, we explicitly applied their impacts as the boundary conditions in the matrix. In this case: 

% \begin{itemize}
% \item Matrix: The multiphase flow in the matrix is analyzed by assuming that the \(s_w\)  and the \(p_{nw}\) in the matrix at points of intersection with fractures are equal to the corresponding values in the fractures.
% \begin{align}
% s_w = s_{w}^{F,BL},\ \ \ \ {\in\Omega}_{MF} \label{eq:pretrsw}
% \end{align}
% \begin{align}
% p_{nw} = p_{nw}^{F,BL},\ \ \ \ {\in\Omega}_{MF} \label{eq:pretrpnw}
% \end{align}

% \(s_{w}^{F,BL}\) is calculated using the 1D Buckley-Leverett (BL) theory, and \(p_{nw}^{F,BL}\)  is calculated using linear pressure distribution assumption. The Buckley-Leverett theory offers a fundamental analytical approach for forecasting the saturation profile and front velocity of the displacing fluid in two-phase flow in porous media. The BL theory is explained in Appendix  \ref{sec:BLequation}. 
% \item Fracture: The PINNs model corresponding to the PDE of multiphase flow in fractures is solved by ignoring the interactions with matrix. 
% \end{itemize}

% In the case of inverse calculations, before starting the optimization of inverse variables, it is essential to partially train the networks so that they can learn the main characteristics of the problem. This approach has been successfully applied in previous studies, such as those by \citet{Zhang2022AnalysesNetworks} and \citet{Abbasi2024ApplicationTests}. At this step, the trainable inverse parameters are kept frozen for some limited apochs. 


% \input{tables/table_dlnetwork}


% \begin{figure}[htbp]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=.999\textwidth]%
%     {graphics/Fig2.jpg}% picture filename
% \end{center}
% \caption{The architecture of the PINNs model: a)  The spatial distribution of the matrix and fracture collocation points, b) Separate networks for the state variables of matrix and fracture systems, c) The architecture of each NN, and d) the cross-sectional view of the porosity distribution in the experimental data.}
% \label{fig:2}
% \end{figure}



% \begin{figure}[htbp]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=.99\textwidth]%
%     {graphics/solution_approach.jpg}% picture filename
% \end{center}
% \caption{The solution approach for forward and inverse problems. The curriculum regularization is the process of training the Matrix PINNs model based on BL-type fracture model, at same time as training the Fracture PINNs (without source terms between two networks).}
% \label{fig:solmethod}
% \end{figure}


% \subsection{Experimental Data}
% \label{sec:experimentaldata}
% The study evaluated experimental data from injecting water into a  CO\textsubscript{2}-saturated fractured shale rock core, as detailed in \cite{Kurotori2023MixedMedia}. The cylindrical Wolfcamp shale core had a length of 5.8 cm, diameters of 2.5 cm, an average permeability of \(1.97e-17\) m$^2$ (0.020 mD) and porosity of 0.102. The core was initially saturated with CO\textsubscript{2}, then water was injected at 530 psi injection pressure and 460 psi backpressure for 311 hours while confined at 700 psi. Dynamic CT images were captured at intervals, recording in-situ saturation, phase recovery, and injected fluid volume over time. Different fractures were identified from the CT scan images. History matching and inverse calculations in this study relied on several key experimental measurements (also see Fig. \ref{fig:colls}e):

% \begin{itemize}
% \item\textbf{Recovery Factor (RF)}: the volume fraction of the pore space displaced by the injected fluid over time. We calculated the RF curve by averaging the saturation of the wetting phase fluid obtained from CT scan images.
% \item\textbf{Boundary Conditions}: The constant pressure at the inlet and outlet boundaries were known based on the experimental setup.
% \item\textbf{Injection Volume}: The total volume of water injected into the system as a function of time was directly measured.
% \item\textbf{Spatial Saturation Data}: Spatial distribution of fluid saturation within the sample at different times, obtained through CT scans.
% \end{itemize}

% More details on the data sets used in this study and their use within the PINNs framework can be found in Appendix \ref{sec:PINNsimplementation}2.



% \subsection{Collocation Points}
% As it is visualized in Fig. \ref{fig:colls}, collocation points were extracted separately for the matrix and fracture domains based on the CT/micro-CT scan coordinates. 23500 matrix spatial collocation points were used in the core cylinder domain at specified x, y, z resolutions, excluding points in superposition with fractures. Boundary collocation points were collected for the cylinder ends and radius. Fracture collocation points were manually extracted from micro-CT scans. Temporal collocation points were randomly selected based on the \(\sqrt{t}\) distribution intervals, as it is expected that the system is mainly controlled by spontaneous imbibition mechanism. \cite{Abbasi2023SimulationNetworks} have shown how the selection of temporal points based on \(\sqrt{t}\) distribution intervals helps in improving PINNs solutions. More detailed information about the experimental data and the collocation points are provided in Appendix \ref{sec:PINNsCollocation Points}.





% \begin{figure}[htbp]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=.99\textwidth]%
%     {graphics/colls.jpg}% picture filename
% \end{center}
% \caption{ The collocation points have been used for solving the problem under study. The color of the points demonstrate the corresponding time for each point in the range \(t=1-10^6 \) sec. a) The collocation points at the boundary conditions of inlet (y=0) and outlet (y=L) faces (940 spatial points), b) The collocation points corresponding to the non-flowing boundary condition at \(r=r_{c}\) (8630 spatial points), c) The collocation points corresponding to the fracture (4103 spatial points), d) The collocation points corresponding to the matrix (23500 spatial points). The matrix collocation points with distance less than 0.0006 m from the fracture collocation points have been removed. e) the observational data points used in the data loss: 1) RF points, 2) points with the measured injected volume, and 3) spatiotemporal points of the in-situ \( s_w\) measured using CT-scan. }
% \label{fig:colls}
% \end{figure}




% \section{Results and Discussion}

% \subsection{Benchmark Modeling}
% \label{sec:benchmarksection}
% The validation and comparison of applied approaches for addressing multiphase flow in fractured porous media are crucial. This section focuses on validating the proposed methodology against a fully-characterized synthetic problem. We introduce a coupled matrix-fracture flow problem to validate the solutions obtained using PINNs and to compare different strategies. Fig. \ref{fig:BenchFrac}a provides a 3D visualization of the matrix-fracture system. Specifically, we define a cylindrical core featuring a significant vertical fracture (located at \(x=12.5\) mm) in the flow direction (\(y\)). The properties of both the matrix and fracture are detailed in Table \ref{tab:benchprops}. 


% Additionally, Fig. \ref{fig:BenchFrac}b illustrates the static geometry of the matrix and fracture system, along with a 3D visualization of the discretized model. We have utilized an in-house finite-difference (FD) simulator - IORCoreSim (ICS) - \citep{Lohne2017ARegimes}, to provide with the solution of the defined benachmark problem. The advantage of ICS compared to other available simulators was its ability to simulate experimental boundary conditions through a developed module.
% The specifications of the utilized PINNs model is shown in Table \ref{tab:benchPINNsprops}. In this section, the same network architecture as in Fig. \ref{fig:2} has been used. Also, the pre-training strategy - explained in Fig. \ref{fig:solmethod} -  was applied.


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.89\textwidth]%
%     {graphics/BenchFracMap.jpg}
% \end{center}
% \caption{The map of the fracture in the benchmark matrix-fracture model. a) the geometry, b) the equivalent static model for the FD simulations}
% \label{fig:BenchFrac}
% \end{figure}


% \input{tables/t_bl}

% \input{tables/table_app2}



% \subparagraph*{Forward simulation. }
% To validate the PINNs model, we first simulated the benchmark problem in forward mode. The resulting flow saturation profile within the matrix is visualized in Figure~\ref{fig:benchprof}. Figure~\ref{fig:benchprof}a presents a 3D view, highlighting the similarity of the phase distribution across different spatial coordinates at a specific time (t = 57.7 hrs). Figure~\ref{fig:benchprof}b focuses on the lateral invasion of the wetting phase perpendicular to the fracture surface (at y = 29 mm) at various times. These visualizations demonstrate the PINNs model's ability to accurately capture the key three-dimensional flow characteristics.


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.95\textwidth]%
%     {graphics/fdbench.jpg}
% \end{center}
% \caption{A comparative analysis of the frontal behavior of fluids as simulated by PINNs and FD for the benchmark problem’s forward simulation. a) a 3D visualization of  \(s_w\), and \(p_w\) profiles, and their point-wise absolute errors at t=57.7 hrs. b) the 2D cross-sectional view of \(s_w\) at y=29 mm for various time points: t=33.2, 57.7, and 81.2 hrs.}
% \label{fig:benchprof}
% \end{figure}

% \subparagraph*{The importance of pre-conditioning. }


% \subparagraph{Inverse Calculations Based on History Matching of Recovery Factor.}
% This work's primary objective is to use PINNs to interpret 3D flow processes in porous media and then compute the system's unknown parameters via inverse interpretation of experimental/numerical observations. Therefore, here, we try to utilise PINNs for the purpose of calculating the flow parameters of the system, i.e., \(k_r\) and \(p_c\) of matrix, by history matching of the
% observational data. At this stage, we only consider the RF curve vs. time as the observation data. The analysis is based on the assumed characterization of matrix porosity and permeability, as well as assumed knowledge of fracture properties. 

% Fig. \ref{fig:benchinvres} shows the details of the results obtained after inverse calculations. The calculations continued for 12000 epochs, until the error in RF was minimized (Fig. \ref{fig:benchinvres}a) and the trend of changes in inverse parameters reached to a plateau. The matching of the matrix RF curve (Fig. \ref{fig:benchinvres}b) could lead to the inverse calculation of the CDC curve, as observable in Fig. \ref{fig:benchinvres}b. The PINNs calculations could also accurately predict the volumetric rate of the injected water, as it is shown in Fig. \ref{fig:benchinvres}c. The main determining factor on the total injected rate is the fracture permeability.

% However, we do not expect to accurately retrieve the \(k_r\) and \(p_c\) curves (Figs. \ref{fig:benchinvres}c and \ref{fig:benchinvres}d) due to the high degrees of freedom in the system and the lack of enough information about the pressure of the wetting phase. It means that there are infinite sets of \(k_r\) and \(p_c\) curves that can lead to the observed dataset. This limitation is evident in Fig. \ref{fig:benchinvres}e, where the network could predict the saturation profile in the system but failed to accurately predict the pressure distributions. 

% Fig. \ref{fig:MFflow} provides a comparison of the matrix-fracture exchanges. Positive values indicate flow out of the fracture (into the matrix). Conversely, negative values indicate flow into the fracture (from the matrix). Initially, we observe a strong wetting phase flow from the fracture to the matrix, which stabilizes over time. This behavior results in an almost straight cumulative flow line versus \(\sqrt{t}\), highlighting the significant influence of capillary forces. Fig. \ref{fig:MFflow}c compares vector field of velocity for both phases. Although the wetting phase continuously imbibes into the matrix, the non-wetting phase follows viscous forces within the matrix, indicating the presence of a co-current spontaneous imbibition mechanism in the system. 





% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/benchres.jpg}
% \end{center}
% \caption{The results of inverse calculation for the synthetic benchmark model, based on history matching of the recovery curve vs. time. a) The trend of minimizing error compared to the RF data, b) The RF curve, c) The estimated flow curves compared to the true and the randomly initialized values: \(\Lambda\), \( p_c\) and \(k_r\) curves, respectively, d) The comparison of water injection rate for FD and PINNs models,  e) The flow profile along the injection direction for (1) \(s_w\)  and (2) \(p_w\), at t= 23.22, 57.7, 98.2, 167.9 hrs, f) the trend of changing the different inverse variables vs. epochs during the inverse calculations. }
% \label{fig:benchinvres}
% \end{figure}





% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/MFflow.jpg}
% \end{center}
% \caption{ The matrix-fracture interaction rates for the benchmark problem. In all the figures the right axis show the cumulative values. The scatter points represent values at various spatiotemporal collocation points; a1,2) The mass rate of flow between two media for both phases; the right axis shows the cumulative mass flow (eq. \ref{eq:massratecum}). b1,2) the volumetric rate of flow; the right axis show the cumulative fraction of pore-volume (eq. \ref{eq:dimenlessPVMF}), c) 2D vector field plot at z=0.0125 m. Here, \( u_w \) and \( u_{nw} \) are not directly comparable, as they are scaled to the same range for visualization purposes.}
% \label{fig:MFflow}
% \end{figure}



% \subparagraph{Uncertainty Quantification.} To validate the results, we repeated the calculations multiple times - using an ensemble-based uncertainty quantification - each with random initialization of the inverse parameters (see Appendix \ref{sec:PINNsComputationalstrat} for more details). As demonstrated in Fig. \ref{fig:benchinvens}, the CDC curves consistently converge to similar values across different cases. It illustrates the system's well-defined nature in relation to the CDC curve. In contrast, the \(k_r \) and \(p_c\) curves converged to distinct values. A similar results have been discussed in \cite{Abbasi2024ApplicationTests} for a 1D spontaneous imbibition system. Accurate estimation of the \( p_c \) curve requires measuring the pressure of both phases, which is often challenging in practical scenarios. Consequently, the uncertainty in the \( p_c \) curve propagates to the \( k_r \) curves.  


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.991\textwidth]%
%     {graphics/bench_ens.jpg}
% \end{center}
% \caption{ The inverse calculation results for an ensemble with different initialization of the inverse parameters. The initialization have been performed randomly.  a) the initial guess \textcolor{gray}{(gray)} and the final estimations after inverse calculations have been compared for \textcolor{magenta}{(magenta)} of \( \Lambda\), \( p_c\), \( k_{rw}\) and \( k_{rnw}\)  curves, respectively. The \textcolor{blue}{blue} curves show the true values. The shaded areas represent the mean $\pm$ standard deviations (STD).  b) the optimization landscape of different terms during optimization during the training: \( \mathcal{L}_t\), RF (MAE), and \( \bar{\Lambda}\), respectively.}
% \label{fig:benchinvens}
% \end{figure}




% \subsection{Experimental Problem}
% This section employs PINNs for the interpretation and parameter identification of the real multiphase flow in the shale rock system, presented in \ref{sec:experimentaldata}. The known properties of the system is shown in Table \ref{table:shalerockprops}. The \(K\) and \(K_F\)  are assumed as 0.01 and 100 multipliers of the mean permeability of the rock.
% The matrix permeability is determined by \( K_F = 0.01 K_{exp} \), while the fracture permeability is determined by \( K = 100 K_{exp} \). The value of \( K \) can be adjusted based on the calculated CDC curve, and \( K_F \) can be accurately determined through history matching the total injection rate of water.



% \input{tables/table_experimental_props}



% \subparagraph{History Matching of the recovery curve and the total injection rate.} 
% The volume of recovered fluids, the volume of the injected fluids, and the pressure drop along the core, all over time are the most commonly utilized observational data for studying multiphase flow processes in porous media. In this study, we calculated the \( \bar{s_w}\) curve by averaging the in-situ water saturation data obtained from CT-scan measurements, representing the changes in the volume of the fluids saturated the rock. In addition to the matrix multi-phase flow parameters, the fracture permeability was assumed unknown, initialized to be  higher than the average permeability measured experimentally, reflecting the high conductivity of the fracture network. To perform history matching of the \( \bar{s_w}\) curve, we employed a three-step calculation process, as introduced in section \ref{sec:SolutionMethod}. Subsequently, we utilized the calculated properties to validate their accuracy by comparing the results against those obtained from a finite difference (FD) numerical simulation. The results of inverse computations for both matrix and fracture properties are shown in Fig. \ref{fig:expres1}. The inverse computations were started by randomly generated initial guess values for each parameter.

% Fig. \ref{fig:expres1} shows the estimated flow properties of matrix could effectively recover the RF curve. Also, the water injection rate could be matched effectively compared to the experimental data (Fig. \ref{fig:expres1}d). The results indicate that the fracture plays a crucial role in transferring fluids due to its high permeability.
% However, as it is also previously discussed in \ref{sec:benchmarksection}, the \(k_r\) and \(p_c\) curves exhibit non-uniqueness due to the degrees of freedom within the system (unlike the \(\Lambda\) curve that can be uniquely estimated). 
% This conclusion is further supported by the results of ensemble-based uncertainty quantification shown in Figure \ref{fig:expres1}e.




% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.999\textwidth]%
%     {graphics/expres1.jpg}
% \end{center}
% \caption{ The results for inverse calculation of matrix flow parameters by history matching of the \( \bar{s_w}\) experimental data. a) The initial guess and final inverse calculated flow curves, i.e., \(k_r\), \(p_c\) and \( \lambda\) curves, respectively. b) The trend of converging to the final values vs. epoch for different inverse parameters, c) The matched \( \bar{s_w}\) curve by PINNs (1) and the validation results from FD simulations (2), d) Matching the fracture permeability (\(K_f\)) and the history matching of volumetric injection rate: 1) the trend of changes in \(K_f\) versus the matrix permeability and experimentally measured permeability (\(K_{exp}\), 2) The contribution of matrix and fracture in the inlet face, 3) The total velocity of fluids compared to the experimental observational data. e) The results of inverse calculations for an ensemble of models with different initialization values. e1 and e2 show the convergence trends, and later show the saturation function curves. The grey curves are the initial guesses. }
% \label{fig:expres1}
% \end{figure}




% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/profile3dexp.jpg}
% \end{center}
% \caption{ A 3D cross-sectional visualization compares water saturation ($s_w$) and wetting phase pressure ($p_w$) distributions in the porous media (matrix) at different times. The figure compares the PINNs solution after inverse computations, FD solution after forward validation simulation, and experimental CT-scan images. It is important to note that the local saturation data was not utilized during the inverse calculations for the PINNs. Also, the FD simulation shows the forward analysis using the PINNS-based inverse calculated flow parameters. }
% \label{fig:3DprofileExp}
% \end{figure}

% \subparagraph{The Importance of Multiscale Simulations.} We investigate the significance of multiscale simulations in understanding flow in porous media and parameter identification calculations. In two separate cases, We conducted inverse calculations using PINNs while ignoring fractures and their interaction with the matrix: 1) matching RF data, 2) matching RF data as well as total injection rate (Q$_{inj}$). Then, we compared the results (see Fig.~\ref{fig:fracimpact}). The results clearly show the differences between the inverse calculated flow parameters (Fig.~\ref{fig:fracimpact}a). Ignoring the impacts of fractures could lead to about two orders of magnitude difference in the CDC magnitude of the matrix ( \( \bar{\Lambda}= 8e-3 \) for the fractured case, compared to \( \bar{\Lambda}= 9e-5 \) for the non-fractured case). When Q$_{inj}$ was used as observational data, the results, including the relative importance of viscous and capillary forces, significantly changed. This led to high relative permeability and low capillary pressure values, which can be unexpected for shale rock.
% This highlights the critical need for multiscale matrix-fracture simulations when dealing with porous media exhibiting multiscale features like fractures. 


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/fracimpact.jpg}
% \end{center}
% \caption{ The impact of multiscale simulations on the inverse calculated flow parameters of porous media. a) The calculated flow parameters, i.e.,  \( \Lambda\) ,\( p_c\), and \( k_r\) vs. saturation, respectively. b) The validation of the obtained results with FD simulations, in matching with the experimental RF data, c) The trend of changes in \( \mathcal{L}_t\), \( \bar{\Lambda}\), \({k}_{rw}^{max}\), and MAE in RF  vs. epochs, respectively. }
% \label{fig:fracimpact}
% \end{figure}




% \subparagraph{History matching of in-situ water saturation data.}

% The history matching of high-fidelity datasets, particularly (3+1)D in situ water saturation data obtained from in-situ CT images, represents a significant challenge and introduces opportunities in understanding porous media properties more insightfully. In Fig. \ref{fig:insitusat}, rather than relying on RF data for the inverse calculations, we utilized the local spatiotemporal values of \(s_w\) directly as observational data for both history matching and the estimation of flow parameters. Additionally, we employ an adaptive fracture importance determination strategy to understand local variations in matrix-fracture interactions, serving as indicators of changes in fracture properties within the rock. A comparison of cases the history matching of the datasets with and without denoised observartional data show no meaningful differences in both saturation distributions as well as the inverse calculated CDC curves. Denosing have been performed via a 3D convolutional kriging approach, as explained in Appendix \ref{sec:PINNsComputationalstrat}. This tells us the potential of PINNs in extracting the main governing properties of the physical systems in presence of of noisy observations \citep{Chen2021Physics-informedData}. 

% In Fig. \ref{fig:insitusat}c, an approach is utilized to automatically detect the inconsistencies between the PINNs predictions (based on the homogeneous fracture properties assumption), and the CT-scan images, in the fractured zones. The approach is explained in ---. In the fracture points with gray color, the PDE solution closely matches the CT images, indicating high agreement. In the blue zones, the CT images show less imbibition than expected by the PINNs solution, suggesting low matrix-fracture interactions. Conversely, in the red regions, the saturation trends in the CT images differ significantly from the PINNs expectations, highlighting discrepancies that were successfully detected in both the original and denoised datasets. The results successfully shows the possible differences between the fracture properties, as well as uncertainties in the zones considered as the fractued areas.



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/insituepinns.jpg}
% \end{center}
% \caption{ The PINNs solution for inverse calculations when the in-situ water saturation data have been used as the observations. A comparison has been made between two cases in which the observations have been pre-processed using a convolutional kriging algorithm. a) A comparison of the inverse calculated flow curves (\(k_r\), \( p_c\) and \(\Lambda\), respectively) for different scenarios of using observational data, b) A comparison of the matched profile of water saturation, c) The results of fracture uncertainty quantification (\textcolor{gray}{gray} indicates minimal uncertainty, \textcolor{blue}{blue} represents medium uncertainty, and \textcolor{red}{red} represents high uncertainty) }
% \label{fig:insitusat}
% \end{figure}







% \subparagraph{Computational Cost:} In this study, we employed two simulation approaches: Finite Difference (FD) and PINNs. The FD numerical simulator were developed in C++ and run on an Intel i9-11950H CPU (2.60 GHz) with 32 GB RAM. Individual forward simulations for a 27,000 cell model ranged from 40 minutes to 2 hours, depending on the complexity of effective parameters (e.g., flow parameter shapes and matrix-fracture property contrasts). We did not try FD for inverse solution of the problem, but it normally requires a large number of iterations (hundreds) to reach to the final solution of the problem. 

% In contrast, PINNs computations were conducted using an NVIDIA RTX A2000 GPU with the PyTorch 1.13.1+cu117 framework. Notably, PINNs simulations exhibited similar runtimes for both forward and inverse problems. Even for complex network architectures with large number collocation points, the inverse computations typically required only 1-2 hours. This highlights a significant advantage of PINNs compared to traditional FD methods for inverse calculations which are normally computationally expensive. However, for the forward solution, both almost methods performed at same time scales. 




% \section{Discussion}

% The results demonstrated the effectiveness of PINNs in capturing the multiscale flow dynamics in fractured porous media systems. In the case of inverse calculations, PINNs could model the coupled matrix-fracture interactions orders of magnitude faster than FD simulation methods. The implemented uncertainty quantification analysis yielded valuable insights into the unique and non-unique characteristics of the obtained solutions. 

% Reaching to time-efficient and accurate solutions by PINNs was not possible without utilizing a variety of techniques, such as pre-training of the PINNs model using simplified assumptions, independent network architecture, resampling of the points during the training, and Fourier transformations in the networks.  This combined strategy facilitated a balance between accuracy and computational efficiency, even when dealing with a problem involving second-order gradients in three dimensions, which is considered a computationally intensive operation. 

% However, while PINNs offer promising solutions, further development is necessary to achieve fully reliable models for a wide range of multiphase flow scenarios. Notably, problems with unfavorable mobility ratios, often encountered in systems like water-CO$_2$ injection, can lead to unbalanced loss terms within the PINNs framework. The significant disparity between residual loss terms of phases can lead to complex convergence behavior during training. This may result in the phase with higher mobility being inaccurately captured by the model.

% Additionally, accurately representing multiphase viscous-dominated flow within porous media, and more importantly fractures, where shock fronts impact the flow regimes, is critical for correct modeling of multiscale processes. However, reliable capturing of shock fronts remains a challenge for PINNs and requires further research. 

% Furthermore, increasingly complex fracture networks likely necessitate even more complex neural network architectures. This highlights the need for developing flexible network architectures capable of handling the significant non-linearities exist in such complex systems. 



% \section{Conclusions}
% In this study, we utilized Physics-Informed Neural Networks (PINNs) as a solver for the simulation and parameter identification of (3D+1) two-phase (water+CO$_2$) flow processes in fractured porous media. We applied the model to interpretation and analysis of a multi-fidelity observational dataset. The problem is characterized by a confluence of complexities: highly unfavorable mobility ratios, significant permeability contrasts, and the presence of shock fronts, and unpatterned distribution of fractures in the system.

% \begin{itemize}

%     \item We applied a series of strategies to solve the complex problem under study, including the sequential training, collocation point resampling, Fourier transformation, and adaptive weight losses. 
%     \item The proposed a training workflow solves the problem using a sequential approach: first, a pre-training strategy with simplified set of equations, followed by fully-coupled training technique. The fully-coupled technique independently solves the flow equations for matrix and fracture media, integrating a transfer term that connects them based on a point-source assumption.     
%     \item We initially validated the capabilities of the deployed model using a benchmark synthetic problem. The obtained results demonstrated the effectiveness of PINNs in both forward and inverse simulations of the problem under study. The inverse calculation results exhibited high accuracy, and the model successfully captured the main physical characteristics of flow, including the matrix-fracture interactions over time. The validation of the obtained results with a finite-difference based numerical simulator revealed the accuracy of the calculated parameters.     
%     \item  The applied model could evaluate the experimental dataset using the different combination of the available observations. The model could successfully extract the multi-phase flow properties of matrix, permeability of fracture system, as well as the uncertainties in the deployed fractures. 
%     \item  Our comparison of inverse calculations with and without fractures demonstrates the critical role of multi-scale effects in interpreting multi-phase flow in porous media.  Neglecting these effects can lead to substantial misinterpretations of the fundamental mechanisms governing the system's behavior.    
%     \item The model performed well in evaluating the (3+1)D noisy observations of water saturation, and achieved results comparable to the denoised dataset.


% \end{itemize}


% . 






% \section*{Acknowledgments}
% Abbasi, Andersen, and Hiorth acknowledge the Research Council of Norway and the industry partners of NCS2030 – RCN project number 331644 – for their support.

% % \bibliographystyle{unsrt}
% \bibliographystyle{apalike}
% \bibliography{mendeley} 

% \newpage
% \appendix

% \section*{Appendices}

% \section{Physics-Informed Neural Networks: Implementation }
% \label{sec:PINNsimplementation}

% Physics-Informed Neural Networks (PINNs) is an approach that is introduced by \cite{Raissi2019Physics-informedEquations} for more efficient solving of differential equations, by combining neural networks with physics-based principles.
% In this study, let NNs \( \mathcal{N}_m \) and \( \mathcal{N}_f \) emulates the funcitonal dependency between the independent and dependent variables:

% \begin{align}
% {s}_{w},{p}_{nw} = {\mathcal{N}^M}(x,y,z,t,\theta,\eta)
% \label{eq:pceq}
% \end{align}
% \begin{align}
% {s}_{w}^{f},{p}_{nw}^{f} = {\mathcal{N}^F}(x_{f},y_{f},z_{f},t,\theta_{f},\eta)
% \label{eq:p1}
% \end{align}

% The goal is to solve an optimization problem in which:
% \begin{align}
% \theta^{m,f},\eta = argmin({{\mathcal{L}}}_{t})
% \label{eq:p2}
% \end{align}

% In this equation, \( \mathcal{L}_t \) represents the weighted summation of all  of the loss terms corresponding to matrix and fracture, as well as the observational data:

% \begin{align}
% \mathcal{L}_{t} = \mathcal{L}_{t}^{M} + \mathcal{L}_{t}^{F} + \mathcal{L}_{t}^{D} 
% \label{eq:p2}
% \end{align}

% where \(\mathcal{L}_{t}^{M}\) and \(\mathcal{L}_{t}^{F}\) are the total loss terms corresponding to the initial/boundary conditions, as well as the PDE residuals for matrix and fracture domains, respectively. Furthermore, \(\mathcal{L}_{t}^{D}\) represents the total loss term corresponding to the errors compared to the observational data values. We will now explore the specific formulations of each loss term in more detail. 

% As the scales of pressure data and water saturation data differ significantly, we needed to ensure they are comparable by bringing them to similar scales. To achieve this, we normalized the pressure loss terms by dividing all related terms by \(\kappa_p\), defined as:

% \begin{align}
% {\kappa}_{p} = ({p}_{in} + {p}_{out} ) /2
% \label{eq:p2}
% \end{align}

% Furthermore, since the scale of loss terms related to PDE residuals also deviates significantly from the [0,1] range, we defined another PDE normalization multiplier as:


% \begin{align}
% {\kappa}_{r} = \frac{ t_{max}}{({\rho}_{w} + {\rho}_{nw} ) /2} 
% \label{eq:p2}
% \end{align}

% where \( t_{max}\) is the time related to the end of experiment, which is almost 1e6 sec (277.78 hrs).


% \subsection{Flow in Matrix Domain}

% The solution for the governing equations within the matrix domain is achieved by minimizing a weighted combination of loss terms, denoted as \(\mathcal{L}_{t}^{M} \). These loss terms account for the residuals of the PDEs, the initial conditions, and the boundary conditions applied at different boundaries.


% \subparagraph{PDE Residuals:} To solve the flow in the matrix, we must simultaneously address the conservation laws for both the wetting and nonwetting phases. Thus, we define different loss terms according to Eq. \ref{eq:e1}:

% \begin{align}
% {{\mathcal{L}}}_{w}^{M} = \frac{1}{\kappa_r} \text{MAE}(\text{ }\phi{\partial }_{t}\left({\rho}_{w}{s}_{w}\right) + \nabla \left({\rho}_{w}{u}_{w}\right )\text{ },\text{ } 0.0),\text{ } \in {\Omega}_{M}
% \label{eq:matrix_loss_w}
% \end{align}
% \begin{align}
% {{\mathcal{L}}}_{nw}^{M} = \frac{1}{\kappa_r} \text{MAE}(\text{ }\phi{\partial }_{t}\left({\rho}_{nw}{s}_{nw}\right) + \nabla \left({\rho}_{w}{u}_{nw}\right)\text{ },\text{ } 0.0),\text{ } \in {\Omega}_{M}
% \label{eq:matrix_loss_w}
% \end{align}

% Here, MAE is the Mean Absolute Error, a metric used to measure the errors. It represents the average absolute difference between the predicted values and the actual values:
% \begin{align}
% {\text{MAE}(\hat{y}_i, y_i) = \frac{1}{n} \sum_{i=1}^{n} \left| \hat{y}_i  - y_i \right|,}
% \label{eq:maeeq}
% \end{align}
% where \( n\) is is the number of observations, \(y_i\) is the actual value, and \( \hat{y}_i\) is the predicted value.
% Then, the total loss corresponding to the residual of equations of flow in matrix is defined as: 

% \begin{align}
% {{\mathcal{L}}}_{PI}^{M} =  ({\mathcal{L}}_{w}^{M}  + {\mathcal{L}}_{nw}^{M}) \cdot e^{\omega^M}, \text{  } \text{  } \in {\Omega}_{M} 
% \label{eq:volbalance}
% \end{align}

% where \( \omega^M\) represents the local weight modifier obtained by self-attention mechanism as outlined in Appendix \ref{sec:PINNsComputationalstrat}.  A loss term is defined to constraint the values of the self-adaptive modifier for :

% \begin{align}
% {{\mathcal{L}}}_{\omega}^{M} = \text{MAE}(\omega^{M} , 0.0),\text{  } \in {\Omega}_{F}
% \label{eq:»LomegaM}
% \end{align}


% \subparagraph{Matrix-Fracture Mass Transfer:} For the matrix collocation points, where mass transfer occurs between the matrix and the superimposed fracture network, we formulate the residual term of the governing partial differential equation as follows:

% \begin{align}
% {{\mathcal{L}}}_{w}^{MF} = \frac{1}{\kappa_r}\text{MAE}(\text{ }\phi{\partial }_{t}\left({\rho}_{w}{s}_{w}\right) + \nabla \left({\rho}_{w}{u}_{w}\right)  - ~\frac{{\rho}_{w}}{{e}_{V}}\left(2{v}_{w}^{\bot }\right)\text{ },\text{ }0.0),\text{  } \in {\Omega}_{MF}
% \label{eq:matrix_loss_w}
% \end{align}
% \begin{align}
% {{\mathcal{L}}}_{nw}^{MF} = \frac{1}{\kappa_r}\text{MAE}(\text{ }\phi{\partial }_{t}\left({\rho}_{nw}{s}_{nw}\right) + \nabla \left({\rho}_{w}{u}_{nw}\right)  - ~\frac{{\rho}_{nw}}{{e}_{V}}\left(2{v}_{nw}^{\bot }\right)\text{ },\text{ }0.0),\text{  } \in {\Omega}_{MF}
% \label{eq:matrix_loss_w}
% \end{align}

% The interaction term is governed by the pressure differential between the matrix and fracture and the local transmissibility of the matrix. In the fully-coupled training stage, we then define:

% \begin{align}
% {{\mathcal{L}}}_{PI}^{MF} =  ({\mathcal{L}}_{w}^{MF}  + {\mathcal{L}}_{nw}^{MF} ) \cdot e^{\omega^{MF}}, \text{  } \text{  } \in {\Omega}_{MF} 
% \label{eq:LMFvolbalance}
% \end{align}



% Here, \( \omega^{MF}\) is defined as a local self-adaptive weight modifier. A loss term is defined to constraint the values of the self-adaptive modifier for :

% \begin{align}
% {{\mathcal{L}}}_{\omega}^{MF} = \text{MAE}(\omega^{MF} , 0.0),\text{  } \in {\Omega}_{MF}
% \label{eq:»LomegaMF}
% \end{align}




% \subparagraph{Pre-training Stage:} 
% In the pre-training stage, we assumed that the matrix collocation points corresponding to the fractured zones are acting as the boundary conditions of the system, following the pressure and saturation trends of the fractures. The matrix and fracture points, however, was calculated via Buckley-Leverett technique. We directly assign the fracture saturation and pressure properties to the collocated matrix points:

% \begin{align}
% {{\mathcal{L}}}_{PT,s_w}^{MF} =  \text{MAE}(\text{ } ({s}_{w} - {s}_{w}^{F}) \xi_f \text{ },\text{ } 0.0 \text{ }), \text{  } \text{  } \in {\Omega}_{MF} 
% \label{eq:LMFPTsw}
% \end{align}

% \begin{align}
% {{\mathcal{L}}}_{PT,p_{nw}}^{MF} =  \frac{1}{\kappa_p}\text{MAE}(\text{ } ({p}_{nw} - {p}_{nw}^{F}) \xi_f\text{ },\text{ } 0.0  \text{ }), \text{  } \text{  } \in {\Omega}_{MF} 
% \label{eq:LMFPTpnw}
% \end{align}

% where, \( {s}_{w}^{F} \) and \( {p}_{nw}^{F}  \) are the fracture state state variables calculated via Buckley-Leverett and linear pressure drop equation, explained in Appendix \ref{sec:BLequation}. Also, \( \xi_f \) is defined as a self-adaptive multiplier acts as the fracture uncertainty identifier. Technically, it adjusts the local matrix-fracture interactions. \( \xi_f \) is a trainable vector defined for all fracture collocation points, and initialized to be equal to one. Then, a restricting loss terms is defined to balance the \( \xi_f \) impacts during the training:

% \begin{align}
% {{\mathcal{L}}}_{\xi_f}^{MF} =  \text{MAE}(\text{ }  \xi_f \text{ },\text{ } 1.0   \text{ }), \text{  } \text{  } \in {\Omega}_{MF} 
% \label{eq:LMFPTxi}
% \end{align}

% In trying to minimize the trade-offs between the loss terms comparing the PINNs predictions vs. CT-scan images, as well as the matrix-fracture physical constraints, the values of \( \xi_f \) is adjusted in a way that the lowest discrepancies was obtained. In scenarios where uncertainty quantification is not a focus, setting \( \xi_f = 1.0 \) for all points simplifies the optimization process.


% \subparagraph{Initial Conditions:}
% With the initial state of the system fully defined, we can now express the corresponding loss terms as:

% \begin{align}
% {{\mathcal{L}}}_{IC,s_w}^{M} = \text{MAE}({s}_{w}(x,y,z,t = 0) , {s}_{wc}) ,\text{  } \in {\Omega}_{M}
% \label{eq:»LeqICmatrix}
% \end{align}
% \begin{align}
% {{\mathcal{L}}}_{IC,p_n_w}^{M} = \frac{1}{\kappa_p}\text{MAE}({p}_{nw}(x,y,z,t = 0) , {p}_{i}) ,\text{  } \in {\Omega}_{M}
% \label{eq:»LeqICmatrix}
% \end{align}

% \subparagraph{Boundary Conditions at Inlet:}
% At the inlet, the core is exposed to water under a constant injection pressure, allowing us to express the loss terms as:


% \begin{align}
% {{\mathcal{L}}}_{BC0,s_w}^{M} = \text{MAE}({s}_{w}(x,y = 0,z,t),{s}_{w,max}),\text{  } \in {\Omega}_{M}
% \label{eq:LBC}
% \end{align}
% \begin{align}
% {{\mathcal{L}}}_{BC0,p_n_w}^{M} = \frac{1}{\kappa_p}\text{MAE}({p}_{nw}(x,y = 0,z,t),{p}_{in}),\text{  } \in {\Omega}_{M}
% \label{eq:LBC}
% \end{align}

% \subparagraph{Boundary Conditions at Outlet:}
% To ensure proper flow characteristics, the outlet should be modeled with a constant pressure boundary condition:

% \begin{align}
% {{\mathcal{L}}}_{BC1,pnw}^{M} = \frac{1}{\kappa_p}\text{MAE}({p}_{nw}(x,y = L,z,t),{p}_{out}), \text{  } \in {\Omega}_{M}
% \label{eq:LpnwBC1}
% \end{align}


% \subparagraph{Boundary Conditions at Radial Surfaces:} 

% The radial \( (r_c)\) boundary condition can be enforced by adding a term to the loss function that penalizes the deviation from zero of the sum of the partial derivatives with respect to \( x \) and \( z \) at \( r = r_c \). The loss function term can be written as:

% \begin{equation}
% \mathcal{L}_{\text{BCr}}^{M} = \frac{1}{\kappa_p}\text{MAE} \left( \frac{\partial p}{\partial x} \Big|_{r = r_c} + \frac{\partial p}{\partial z} \Big|_{r = r_c} \right) , \text{  } \in {\Omega}_{M}
% \label{eq:Lmbcr}
% \end{equation}




% \subparagraph{Pre-training:} 
% In the pretraining stage, we assumed that the matrix collocation points corresponding to the fractured zones are acting as the boundary condiitons of the system, following the pressure and saturation trends of the fractures. The matrix and fracture points, however, was calculated via Buckley-Leverett technique. The 






% \subsection{Flow in Fracture Domain}

% Same as the matrix domain, we define the fracture total loss term, \(\mathcal{L}_{t}^{F} \): 


% \subparagraph{PDE Residuals:} The conservation of mass in fracture media should also be solved in parallel with the matrix equations. By utilizing eq. \ref{eq:massbalF}, we write:

% \begin{align}
% {{\mathcal{L}}}_{w}^{F} = \frac{1}{\kappa_r} \text{MAE}(\text{  }\phi^ \parallel {\partial }_{t}\left({\rho}_{w}{s}_{w}^{F}\right) + \nabla ^ \parallel \left({\rho}_{w}{u}_{w}^{ \parallel }\right)~ + ~\frac{{\rho}_{w}}{{e}_{V}}\left(2{v}_{w}^{\bot }\right)\text{  }),\text{  } \in {\Omega}_{F}
% \label{eq:Lfw}
% \end{align}
% \begin{align}
% {{\mathcal{L}}}_{nw}^{F} = \frac{1}{\kappa_r} \text{MAE}(\text{  }\phi^ \parallel {\partial }_{t}\left({\rho}_{nw}{s}_{nw}^{F}\right) + \nabla ^ \parallel \left({\rho}_{nw}{u}_{nw}^{ \parallel }\right)~ + ~\frac{{\rho}_{w}}{{e}_{V}}\left(2{v}_{nw}^{\bot }\right)\text{  }),\text{  } \in {\Omega}_{F}
% \label{eq:Lfnw}
% \end{align}

% Our approach to address the reported limitations of PINNs in capturing shock fronts for fully-viscous problems \citep{Fuks2020LIMITATIONSMEDIA} involved incorporating a small capillary pressure term. This term introduces a diffusive effect that mitigates the overly sharp transitions typically observed in the displacement front of the replacing fluid. Then, the total loss value for the residual of PDE in the fracture domain is calculated by:

% \begin{align}
% {{\mathcal{L}}}_{PI}^{F} = ( {\mathcal{L}}_{w}^{F}  + {\mathcal{L}}_{nw}^{F} ) \cdot  e^{\omega^F}, \text{  } \text{  } \in {\Omega}_{F} 
% \label{eq:Fvolbalance}
% \end{align}

% Here, \( e^{\omega^F}\) is defined as a local self-adaptive weight modifier (see Appendix \ref{sec:PINNsComputationalstrat}). A loss term is defined to constrain the values of the self-adaptive modifier:

% \begin{align}
% {{\mathcal{L}}}_{\omega}^{F} = \text{MAE}(\omega^F , 0.0),\text{  } \in {\Omega}_{F}
% \label{eq:»LomegaF}
% \end{align}



% \subparagraph{Initial Conditions:}

% A similar initial condition is also applied to the fracture collocation points.

% \begin{align}
% {{\mathcal{L}}}_{IC,s_w}^{F} = \text{MAE}({s}_{w}^{F}(x,y,z,t = 0) , {s}_{wc}),\text{  } \in {\Omega}_{F}
% \label{eq:»LeqICfracture}
% \end{align}
% \begin{align}
% {{\mathcal{L}}}_{IC,p_n_w}^{F} = \frac{1}{\kappa_p}\text{MAE}({p}_{nw}^{F}(x,y,z,t = 0) , {p}_{i}),\text{  } \in {\Omega}_{F}
% \label{eq:»LeqICpfracture}
% \end{align}

% \subparagraph{Boundary Conditions at Inlet:}


% For the fractures with collocation points at the inlet boundary, we may also define a similar set of boundary conditions: 

% \begin{align}
% {{\mathcal{L}}}_{BC0F,s_w}^{F} = \text{MAE}({s}_{w}^{F}(x,y = 0,z,t),{s}_{w,max}),\text{  } \in {\Omega}_{F}
% \label{eq:LBC}
% \end{align}
% \begin{align}
% {{\mathcal{L}}}_{BC0F,p_n_w}^{F} = \frac{1}{\kappa_p}\text{MAE}({p}_{nw}^{F}(x,y = 0,z,t),{p}_{in}),\text{  } \in {\Omega}_{F}
% \label{eq:LBC}
% \end{align}



% \subparagraph{Boundary Conditions at Outlet:}

% Similarly, for fractures with collocation points at the outlet boundary, we define a similar pressure boundary condition to satisfy the downstream pressure of the system in the fracture system.

% \begin{align}
% {{\mathcal{L}}}_{BC1,pnw}^{F} = \frac{1}{\kappa_p}\text{MAE}({p}_{nw}^{F}(x,y = L,z,t),{p}_{out}),\text{  } \in {\Omega}_{F}
% \label{eq:LpnwBC1F}
% \end{align}





% \subsection{Observations}
% During the inverse calculations, ensuring the PINNs predictions closely align with experimental observations is crucial. To achieve this, we define a data loss term, denoted by \(\mathcal{L}_{t}^{D} \) , which represents the sum of one or more individual loss terms detailed below:

% \subparagraph{Recovery Factor (RF):}
% As matching the average recovered fluids at all times is time-consuming and computationally intensive, we matched the RF at one randomly chosen time point during each epoch. This approach helps the network learn from the observation data without imposing a high computational burden on the optimizer. So, consider \( t_r \) as the time corresponding to one of the available CT-scan images, selected randomly, we can define \(  \bar{s_w} \) as:


% \begin{align}
% RF = \frac{1}{N_x N_y N_z} \sum_{i=1}^{N_x} \sum_{j=1}^{N_y} \sum_{k=1}^{N_z} s_w(xi, y_j, z_k, t=t_r), \text{  }  \in {\Omega}_{M}
% \label{eq:LRF}
% \end{align}

% In the above equation, it is assumed that the core is fully-saturated by the non-wetting phase at the beginning of the test. Then, the corresponding loss term will be: 


% \begin{align}
% {{\mathcal{L}}}_{{RF}} = \text{MAE}( RF , \bar{s_w}^{obs}(t=t_r) ), \text{  }  \in {\Omega}_{M}
% \label{eq:LRF}
% \end{align}

% Here, \(  \bar{s_w}^{obs} \) is the observed \bar{s_w} at time \( t_r\), obtained by averaging the water sautration from the CT-scan images.



% \subparagraph{In-situ Water Saturation:} To incorporate the measured in situ saturation data, a loss term is defined that minimises errors in local saturation values:

% \begin{align}
% \mathcal{L}_{s_w} = \text{MAE}( s_w(x,y,z,t), s_{w}^{\text{obs}}(x,y,z,t) ), \quad \text{for} \quad (x,y,z,t) \in \Omega_{M}
% \label{eq:LRF}
% \end{align}

% where \( s_{w}^{\text{obs}} \) is the measured in-situ water saturation data. Given access to approximately one million observation points in the spatiotemporal dimensions, we randomly selected a small fraction of them (25000 points) at each epoch. In this work, the selected points was resampled (randomly) at each epoch.


% \subparagraph{Inflow Rate Constraint:}
% As an observational data, we may have access to the total inflow rate versus time. To match the inflow rate with the observational data, we write it as:



% \begin{align}
% {{\mathcal{L}}}_{{Q}_{inj}} = \text{MAE}( A_m \underset{}{\overset{}{\iint }}{u}_{w}{M}(y = 0)dxdy\text{  } + ... \notag \\
% A_f \underset{}{\overset{}{\iint }}{u}_{w}^{F}(y^{F} = 0)dx^{F}dy^{F}\text{  },\text{  }{Q}_{inj}^{obs}(t)\text{  }) , \text{  }  \in ({\Omega}_{M} \cup {\Omega}_{F})
% \label{eq:Lqwinj}
% \end{align}

% We denote the cross-sectional areas of the matrix and fracture as $A_m$ and $A_f$, respectively. To estimate $A_f$, we sum the areas of all fracture collocation points at the $y = 0$ plane, excluding overlaps. The area of each individual fracture collocation point is calculated using $\pi \left( \frac{e_v}{2} \right)^2$, where $e_v$ represents the fracture aperture. Finally, we determine $A_m$ based on the core radius ($r_c$) and the calculated $A_f$ using the formula $A_m = \pi(r_c)^2 - A_f$.


% \section{Experimental Data/Collocation Points }
% \label{sec:PINNsCollocation Points}

% \subsection{Experimental Data/Collocation Points}

% In this study, we evaluated an experimental dataset corresponding to the injection of water into a fully CO\textsubscript{2}-saturated fractured shale rock, as detailed in \cite{Kurotori2023MixedMedia}. The experiment was conducted using a core-flooding apparatus integrated with an X-ray µCT imaging setup. Fig. \ref{fig:2}d illustrates a map of the porosity distribution. In the test, a cylindrical Wolfcamp shale core with a mean permeability (\(K_{exp}\)) of 1.97e-17 m\textsuperscript{2} (0.02 mD) and an average porosity (\(\phi\)) of 0.102 was used. The reported permeability represents the average permeability of both the matrix and fractures, with the matrix permeability expected to be significantly lower. The viscosities of water \citep{Haynes2016CRCPhysics} and CO$_2$ \citep{Fenghour1998TheDioxide} are assumed to be 0.89 cP and 0.0157 cP, respectively, with their interfacial tension (IFT) assumed to be 0.04 \(N/m\).  \citep{Shiga2023InterfacialTemperature}. Water and  CO$_2$ density also were set to be 998.7 and 78.9 \( kg/m^{3}\), respectively \citep{Houben2021SupercriticalMembranes}.

% The core was initially saturated with CO\textsubscript{2}, and subsequently, water (brine) was injected at room temperature with an injection pressure \((p_{in})\) of 530 psi and a backpressure \((p_{out})\) of 460 psi. Throughout the test, the core was confined at a pressure of 700 psi, ensuring no lateral flow out of the core. The experiment lasted 311 hours, during which dynamic CT images were captured at various intervals. The in-situ saturation data and phase recovery recorded during the injection process have been processed. In addition, the volume of the injected fluid (water) versus time has been recorded and utilised in the computations.

% The collocation points corresponding to the matrix and fractures are extracted from the the core CT and micro-CT images . Each snapshot of the CT-scan had dimensions of [120, 87, 120], with the voxel resolution of 0.024 mm\textsuperscript{3}. We had access to 19 snapshots through the text from 0.1 to 311.405 hrs after starting of the injection. 
% In total, we identified and extracted six fractures from the CT-scan observations, ensuring none of them intersected with each other. The spatial geometry of the fractures is shown in Fig. \ref{fig:coreschematic}b. We neglected the impacts of micro-fractures however, although they were observed in the micro-CT scan images.




% \subparagraph{Collocation Points:} 
% We need to collect collocation points separately for matrix and fracture domains. The spatial coordinates of the collocation points were extracted on the basis of the coordinates of the points in the CT-scan images. The spatial points have been chosen with the resolution of 30 points in  \(x\) and \(z\) (\(dx=dz\)= 0.81 mm) dimensions, and 60 points in  \(y\) dimension (\(dy\)= 0.96 mm). The collocation points close to the fracture collocation points have been removed from the list of spatial points. In total, 73500 spatial points have been used in the cylindrical domain of the core. Refer to Fig. \ref{fig:colls} for a visualization of these collocation points.
% To address the system's boundary conditions, we've also collected the requisite boundary collocation points.
% Fig. \ref{fig:colls} shows the collected collocation points for the boundary conditions at y=0, y=L and r=\(r_{c}\). The radial collocation points have been chosen via  \(x_{r} = r_c.cos(\beta)\) and \(z_{r} = r_c.sin(\beta)\), , where \(\beta\) represents the angular coordinate of the point, randomly generated within the range of \( (0, 2\pi) \). The corresponding y values of the points was extracted from the main collocation points. 

% \subparagraph{Fracture collocation points:} 
% The fracture collocation points were manually extracted from microCT scans, along with porosity and saturation images. Although some of the fractures could be viewed as separate smaller fractures, we merged the fractures that aligned with each other, reflecting their consistent behaviour in passing the fluids during the injection process.


% \subparagraph{Temporal points:} 
% The temporal values assigned to collocation points were selected randomly and subsequently updated during the resampling process. Anticipating spontaneous imbibition as the dominant mechanism, we selected collocation points at equal intervals relative to their square root of time values, ensuring a balanced distribution across the temporal dimension. \cite{Abbasi2023SimulationNetworks} have previously shown that the spontaneous imbibition  occurs with a constant rate at the square root of time coordinate, and it is advantageous to distribute the collocation points accordingly during training of PINNs.



% \section{PINNs Computational Strategies }
% \label{sec:PINNsComputationalstrat}

% \subparagraph*{Adaptive Loss Terms:  }
% In the training of PINNs, especially in complex processes, simultaneous minimization of various terms often requires addressing conflicting objectives. Numerous studies have demonstrated that employing adaptive weights for these loss terms can enhance the performance of PINNs \citep{Xiang2022Self-adaptiveNetworks}. In this study, we applied these techniques by employing self-adaptive weight values for both the loss terms and the calculated PDE residuals at different domains:  matrix \((\Omega_M)\), fracture \((\Omega_F)\),  and matrix-fracture \((\Omega_{MF})\). This adaptive weighting strategy enables more effective training by dynamically adjusting the contribution of different terms, leading to more reliable convergence. 




% In the context of adaptive-weighting of the PDE residuals at domain collocation points, using trainable vectors was impractical due to the high number of collocation points and the random selection of the temporal points. Therefore, we  defined different MLP networks - with spatiotemporal vectors as inputs, and adaptive weights at outputs - to provide self-adaptive weights for PDE residuals at various collocation points, as suggested by \citet{Anagnostopoulos2023Residual-basedPINNs}:
% \begin{align}
% {\omega}^{M} = {\mathcal{N}_{\omega}^{M}}(x,y,z,t,\theta)
% \label{eq:adaptive_loss_matrixM}
% \end{align}
% \begin{align}
% {\omega}^{F} = {\mathcal{N}_{\omega}^{F}}(x_f,y_f,z_f,t_f,\theta)
% \label{eq:adaptive_loss_matrixF}
% \end{align}
% \begin{align}
% {\omega}^{MF} = {\mathcal{N}_{\omega}^{MF}}(x_f,y_f,z_f,t_f,\theta)
% \label{eq:adaptive_loss_matrixMF}
% \end{align}

% The MLP networks had a depth of 4 layers, each with a width of 40 neurons, activated by \( tanh\) activation functions. The weights of these networks were updated during each backpropagation gradient descent step.


% \subparagraph*{Resampling of Collocation Points: }
% The efficient simulation of the processes in 4D spatio-temporal spaces requires a significant number of collocation points to be chosen and computed during the training. These calculations create a significant computational load that makes the computations time-consuming. Various strategies, including resampling, have been proposed to address this challenge \citep{Coulaud2023Physics-InformedTransfer}. 
% In our study, we implemented a resampling strategy for the collocation points, introducing randomness at various unique periods during training. Specifically, resampling for the matrix collocation points occurred every 10 epochs, with approximately 33\% of the spatial points being selected for resampling each time. The uniform sampling strategy inherently leads to a set of collocation points with statistical homogeneity. We have not applied the resampling strategy for the spatial points of the fractures.

% Furthermore, the temporal coordinates corresponding to the points of the matrix and fractures were randomly resampled using a non-uniform square root of time \((\sqrt t) \) distancing approach in the temporal range of [1 - 10$^6$] seconds. For the temporal points also the resampling period was 10 epochs. 


% \subparagraph*{Loss Term (error) Thresholding:  } To enhance the training efficiency and mitigate the risk of overfitting, we have incorporated an error thresholding technique into the PINNs model. This approach involves neglecting the impact of loss terms that fall below certain preset threshold values. By introducing these threshold limits, we effectively disregard the contributions of loss terms that are deemed insignificant or negligible, thereby simplifying the training landscape. 


% \begin{align}
% \text{e} = \max(0, e - \tau) \times w
% \label{eq:threshholding}
% \end{align}

% In this equation, e is the value of the loss term, and \(\tau \) is the threshold value. We applied this technique to modifty the values of boundary and initial conidtions for both saturation and pressure terms. The value of \(\tau =0.003\) for the saturation and pressure of the phases under initial or boundary conditions


% \subparagraph*{Mathematics of the Inverse Calculations: }
% A critical strategy in inverse computations using PINNs is the pre-training stage, at the beginning of the calculations. In the stage, the inverse parameters will be frozen for some epochs - about 2000 epochs in this work. This technique allows the model to learn the basic mathematical features of the system, before looking for the values of the inverse parameters. The length of pre-training stage depends on the complexity of the evaluating process.


% After the freezing step has been ended, the values of the inverse parameters have been updated at the beginning of each epoch.
% The value of the inverse parameter \(\gamma\) have been calculated based on:
% \begin{align}
% \gamma=\gamma_{i}e^{\kappa \theta^*}
% \label{eq:inverse_eq}
% \end{align}

% where \(\gamma_{i}\) is the initial value of the inverse parameter. Also, \( \theta^* \) is the trainable parameter in neural networks, which have been initialised to be zero at the beginning of the training. \( \kappa \) is a regularisation term that is responsible for the training rate of the parameter. We have found that there should be a balance between the model training speed and the inverse parameter. The large values of \( \kappa \) makes the calculations unstable and prone to converge to the wrong values. The exponential form of the equation allows the algorithm to vary in scales of magnitude. Also, it prevents the model to reach to the unphysical negative values. 

% To consider the uncertainties in the calculations, we defined a strategy to initialize the \(\gamma_{i}\) values randomly. It helps us in reaching a wide range of possible solutions for the problem, not only finding same solutions. Considering an initial value for the parameter of interest as \(\gamma_{i}^{*}\), we write:

% \begin{align}
% \gamma_{i} = \gamma_{i}^{*} * 10^{\xi\xi_m}
% \label{eq:inverse_eq}
% \end{align}

% A random number, denoted by $\xi$, is drawn from a uniform distribution between -1 and 1. This randomness is scaled by a model hyperparameter, $\xi_m$, which controls the overall level of randomness injected into the system. In this case, $\xi_m$ was set to 0.6.


% \subparagraph*{Convolutional Kriging: }
% To overcome with the measurement noises in the measured in-situ saturation data, we applied 3D denoising operations on the dataset. We employed a 3D convolutional kriging approach to effectively interpolate between the cell properties and their neighbour property values. Convolutional denoising involves convolving a noisy data with a weighting kernel that performs smoothing to reduce the noises in the observations, while preserving the main features of the data. The kernel is an important part of the denoising. In this work, we utilized a semi-Gaussian weighted kernel that is shown in Fig. \ref{fig:convkrig}a. The algorithm of the computations is shown in Algorithm \ref{alg:convkrig}. We have used similar kernels for all three dimensions. Finally, a comparison of the saturation distribution in the rock after some time is shown at two different experiment times is shown in \ref{fig:convkrig}b. We can see that the approach could effectively capture the main features of the data while removing unnecessary noise.

 
% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.9\textwidth]%
%     {graphics/kongkrig.jpg}
% \end{center}
% \caption{The impact of 3D convolutional kriging on the in-situ water saturation data. a) The applied weighting kernel, b) A comparisons of the saturation distribution before and after kriging at two different times}
% \label{fig:convkrig}
% \end{figure}



% \begin{algorithm}
% \caption{3D Convolutional Kriging}
% \begin{algorithmic}[1]
% \REQUIRE $inp$: 3D array of input data
% \STATE $k1, k2, k3 \leftarrow \begin{pmatrix} 1 & 1 & 1 & 1 & 2 & 1 & 1 & 1 & 1 \end{pmatrix}$ \COMMENT{the kernel along the dimensions}
% % \STATE $k2 \leftarrow k1$, $k3 \leftarrow k1$ \COMMENT{the kernels along the 2nd and 3rd dimensions}
% \STATE $k1, k2, k3 \leftarrow \text{normalize}(k1, k2, k3)$ \COMMENT{Normalize the kernels to ensure the mass balance is attained.}
% \STATE $out \leftarrow inp$ \COMMENT{Initialize output array as input}
% \FOR{$i$ in range($0$, $3$)}
%     \STATE $out \leftarrow \text{convolve}(out, k_i, \text{axis}=i)$ \COMMENT{Convolve over dimension $i$ }
% \ENDFOR
% \RETURN $out$
% \end{algorithmic}
% \label{alg:convkrig}
% \end{algorithm}

% \subparagraph*{Normalization and Denormalization: }
% An essential pre/post processing step in training of PINNs is normalization and then denormalization of the inlet and outlet variables. By standardizing the input/output data into a common scale and distribution, it can greatly enhance the model's stability and performance. In this work, we have utilized a Z-score normalization shceme. We normalized the PINNa inlets as:


% \begin{align}
% x_n = \frac{{x - \bar{x}}}{{\sigma}}
% \label{eq:norm}
% \end{align}

% And then the outlets denormalized via:

% \begin{align}
% x = x_n \cdot \sigma + \bar{x}
% \label{eq:norm}
% \end{align}

% In above equations  \bar{x} \(\sigma\) are the mean and standard deviation of the variable \(x\) in the domain under study. 



% \subparagraph*{Fourier Transformation: } Table \ref{table:fft}

% \input{tables/fft}


% \section{Buckley-Leverett equation}
% \label{sec:BLequation}

% At the first stage of the PINNs calculations, we have assumed the flow in fractures is governed by the Buckley-Leverett assumptions, meaning that flow is assumed to be a sole function of viscous forces, while capillary and gravity forces are neglected.  

% As a basic solution to this problem, we may follow the solution recommended by \citet{buckley1942mechanism}, called the Buckley-Leverett (BL) equation. The solution assumes that two fluids are incompressible and that the flow occurs unidirectionally.  Rock properties (e.g., porosity and permeability) is considered homogeneous and constant. 
% Also, the problem is considered isothermal with no interphase mass transfer between fluids. The mass conservation equation may be written as  \citep{Lake1989EnhancedRecovery}: 
% \begin{equation}
% \twoPflow
% \end{equation}

% Rewriting the equation for a 1D problem, and assuming incompressibility of rock and fluids, leads to a further simplification as: 
% \begin{equation}
% \oneDtwoP
% \end{equation}

% where, \(u_i\) is the Darcy flow velocity of each phase and is determined by Darcy's law:


% \begin{equation}
% \darcy
% \label{darcy}
% \end{equation}


% Eq. \ref{darcy} may be rewritten by eliminating pressure in the equation and summing the phase equations of two phases:

% \begin{equation}\label{oneDfractionalform}
% \oneDfractionalform
% \end{equation}

% In this equation, \(f_i\) is the fractional flow of phase water, and is written as:
% \begin{equation}\label{oneDfractionalform}
% \fractionalflow
% \end{equation}

% We then employ the Welge tangent method \citep{Welge1952ADrive} to calculate the local water saturation at each time step, as shown in the following equation:

% \begin{align}
% x = \frac{u_t}{\phi} \frac{\partial f_w}{\partial s_w} t 
% \label{eq:norm}
% \end{align}

% Here, \( q_t\) is the total velocity of the fluids, which we can calculate it via:

% \begin{align}
% u_t = \frac{k {k}_{rw}^{max}}{\mu_w}  \frac{(p_{in}-p_{out})}{l}  
% \label{eq:norm}
% \end{align}




% \section*{Appendix: Sensitivity analysis [to be added...]}




% \subparagraph*{Training Dynamics. }
% The dynamics of training of PINNs is visualized in Fig. \ref{fig:b_trdyna}. It’s evident that the precision of PINNs computations is enhanced as the training advances. Initially, the PINNs predictions adeptly encapsulate the high-dimensional attributes of the flow within the matrix. Following this, the interactions between matrix and fracture flows have been learnt.

 
% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/trdyna.jpg}
% \end{center}
% \caption{The dynamics of training PINNs at different epochs (200-8000) compared to the FD simulation result at same time (t=47.2 hrs).}
% \label{fig:b_trdyna}
% \end{figure}



% \subparagraph*{Sensitivity analysis on the model parameters. } To make sure a reliable model properties have been utilized for the calculations, the two most critical properties of the PINNs model - the model size, and the number of collocation points - have been analyzed here. A comparison of the prediction history of the model at the different network sizes is shown in Table \ref{table:netsize}. In this table, the network width and depth of the latent MLP is gradually increased. We can see that ...

% In Table \ref{table:collpoints}, the impact of the number of collocation points have been compared...






% \input{tables/table_bench_netsize}




% \subparagraph*{Resampling of Collocation Points. }  As it is demonstrated in Fig. ~\ref{fig:reselectioncoll}, utilizing resampling techniques significantly reduces errors while accelrating the computations. Resampling, applicable for both spatial and temporal domains, helps the network avoid getting stuck on local regions and steers it towards the optimal general solution of the system in the domain. This is particularly advantageous for large-scale problems requiring a substantial number of collocation points. 

% As Figure~\ref{fig:reselectioncoll}b illustrates, the effectiveness of the resampling strategy depends on the frequency of resampling, or how often it's applied during training epochs. Resampling with very low frequency can not significantly help the optimization. Conversely, excessively frequent resampling prevents the system from learning the selected points effectively. In this context, a frequency between 0.03 and 0.1 (corresponding to resampling every 10-30 epochs) appears to be the optimal choice.



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/sens_collpoints.jpg}
% \end{center}
% \caption{The sensitivity analysis on the number of collocation points in the matrix. All the models were trained for 20000 epochs. a) A comparison of the impact of the number of collocation points on the MAE in the predicted RF curve, b) The impact of resampling period on the accuracy of the predictions.}
% \label{fig:reselectioncoll}
% \end{figure}





% \end{document}

% % \section*{Appendix: Numerical simulations }
% % We have utilized a finite-difference simulation approach to simulate the 








==> changes/main2.tex <==
% \documentclass[12pt]{article}
% \usepackage{graphicx}
% \usepackage{titlesec}
% \usepackage[hyperfootnotes=true]{hyperref}
% \hypersetup{colorlinks, citecolor=blue, linkcolor=blue, urlcolor=blue}
% \usepackage{makecell}
% \renewcommand{\cellalign}{vh}
% \usepackage{hyperref}%
% \usepackage{color,soul}
% \usepackage{amsmath}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{changes}
% \providecommand{\keywords}[1]
% {\small	
% \textbf{\textit{Keywords---}} #1}
% \usepackage{geometry}
% \geometry{ a4paper, total={170mm,257mm}, left=30mm, right=30mm, top=25mm, bottom=25mm, }
% \graphicspath{{figs/}}
% \usepackage{caption}
% % \ucharacterisationinputenc
% \usepackage{authblk}
% \renewcommand\Authfont{\small}
% \renewcommand\Affilfont{\small}

% \usepackage[numbers]{natbib}

% % \usepackage{natbib} 
% % \bibliographystyle{apalike}
% % \bibliographystyle{naturemag} % Nature bibliography style
% % \bibliographystyle{nature} % Nature bibliography style
% \bibliographystyle{IEEEtranN} % Nature bibliography style

% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{eqns}  % Use the equations
% % \captionsetup{font=small}
% \usepackage{xcolor}




% \title{\textbf{History-Matching of Imbibition Flow in Multiscale Fractured Porous Media Using Physics-Informed Neural Networks (PINNs)}}
% % \title{\textbf{Physics-Informed Neural Networks (PINNs) Solver for History Matching of Multiphase Flow in Multiscale Fractured Porous Media}}


% \author[1]{Jassem Abbasi\thanks{Corresponding author: Jassem Abbasi (jassem.abbasi@uis.no)}}
% \author[2]{Ben Moseley}
% \author[3]{Takeshi Kurotori}
% \author[4]{Ameya D. Jagtap}
% \author[3]{Anthony R. Kovscek}
% % \author[2]{Siddhartha Mishra}
% \author[1]{Aksel Hiorth}
% \author[1]{Pål Østebø Andersen}

% \affil[1]{\textit{Department of Energy Resources, University of Stavanger, Stavanger, Norway}}
% \affil[2]{\textit{Seminar for Applied Mathematics, ETH Zürich, Zürich, Switzerland}}
% \affil[3]{\textit{Department of Energy Science and Engineering, Stanford University, Stanford, USA}}
% \affil[4]{\textit{Aerospace Engineering Department, Worcester Polytechnic Institute, Worcester, MA 01609, USA}}

% \begin{document}
% \maketitle

% \begin{abstract}
% In this work, we propose a workflow based on physics-informed neural networks (PINNs) to model multiphase flow in fractured porous media. After validating the workflow in forward and inverse modeling of a synthetic problem of flow in fractured porous media, we applied it to a real experimental imbibition dataset in which brine is injected at a constant pressure drop into a CO$_2$ saturated naturally fractured shale core plug. The exact spatial position of fractures and dynamic in-situ distribution of fluids were imaged using a CT-scan setup. 
% To model the targeted system, we followed a domain decomposition approach for matrix and fractures; and a multi-network architecture for the separate calculation of water saturation and pressure. The flow equations in matrix, fractures, and interplay between them were solved during the training. Prior to fully-coupled simulations, we suggested pre-training the model to aid in the capturing of physical attributes more effectively.
% Both for the synthetic and experimental problems, we determined flow parameters within the matrix and the fractures. Multiple random initializations were performed to assess the uncertainty and uniqueness of the calculations, and the results confirmed the precision of the workflow in retrieving the main flow characteristics of the system. The consideration of multiscale matrix-fracture impacts, while commonly overlooked in existing workflows, has led to several orders of magnitude variations in the calculated flow properties. To the best of our knowledge, the proposed workflow is the first to offer a reliable and computationally efficient solution for inverse modeling of multiphase flow in fractured porous media, achieved through history-matching noisy and multifidelity experimental measurements.




% \end{abstract}


% \keywords{keywords: Physics-Informed Neural Networks (PINNs), \and multiphase flow, \and inverse calculations, \and multiscale fractured porous media}



% \section{Introduction}


% Interpretation of multiphase flow phenomena in fractured porous media is challenging, because of their intrinsic multiscale nature \cite{Fung1991SimulationReservoirs}. In multiscale systems, there is not a clear separation of scales, meaning that traditional homogenization techniques does not apply. The physical processes at the micro scale have to be explicitly modeled and solved in order to get a consistent coarse scale solution of the overall behavior of the system  \citep{Mehmani2021StrivingLearned}. Almost all natural porous media are to some degree fractured; however, an inaccurate mathematical description or modeling of their influence on flow phenomena can lead to substantial errors  \citep{Berre2019FlowApproaches}. These errors are a result of an inaccurate handling of microscale force balances. For applications such as geological carbon storage, fluid flow in aquifers, and recovery of hydrocarbons  \citep{Rangel-German2006Multiphase-flowMedia} an inaccurate description of multiscale systems this can lead to incorrect predictions,  and suboptimal or even wrong decisions. Still, the most common approaches for modeling estimating multiphase flow properties in porous media are developed for homogeneous systems with simplified frontal behavior \cite{McPhee2015CoreGuide}, but these methods are inapplicable for complex multiscale problems \cite{Yang2021RecentMedia}.  Experimentally, multiphase flow properties are characterized via parameter inversion, through history matching of the experimental measurements \cite{Finsterle1998MultiphaseOverview, Schembre2006EstimationExperiments}. In many cases, the multiscale problem is bypassed by selecting rock samples that are relatively homogeneous or making different simplifying assumptions \citep{Berre2019FlowApproaches}. However, when boundary conditions change, experimental simplifications can lead to unreliable parameter estimations, particularly for formations such as shale, where complex fracture networks significantly influence fluid flow behaviour \citep{Salem2022ImpactShale}.


% Furthermore, recent advancements in measurement and imaging technologies have revolutionized our ability to characterize complex, multiphase, flow patterns in porous media. These improvements significantly enhances our capacity to investigate multiphase flow dynamics \citep{Tekseth20244DTomography}. The coupled matrix and fracture multiphase flow systems requires a multiscale description and must be treated carefully when solved numerically \citep{Odster2019AMedia}. Fractures introduce discontinuities in the flow field, which can lead to numerical instabilities and reduced accuracy \cite{Su2015MultiphaseFractures}. Additionally, a multiscale method requires a fine discretization of the domain to capture both multiphase discontinuities and fine scale behavior, which results in high computational costs \citep{Bastian2000NumericalMedia}. Typically, one use numerical methods based on finite-element and finite-volume to solve the problem more efficiently, due to the capability of these methods in handling complex fracture geometries and incorporating discontinuities \citep{Komijani2023AnCoupling, Myner2016AGrids}. However, the implementation of the algorithms is complex, and the numerical schemes typically faces challenges such as high computational requirements and in some cases low convergence reliability \citep{Yang2021RecentMedia}, which could make them impractical and time-consuming for inverse calculation purposes. Given these limitations and opportunities, there is a persistent demand to develop more precise and computationally reliable mathematical tools, especially for the inverse interpretation of multi-fidelity datasets.


% In recent years, Physics-Informed Neural Networks (PINNs) have emerged as a mathematical technique, seamlessly integrating high-fidelity and noisy datasets and domain expertise to solve differential equations governing various engineering and scientific problems \citep{Raissi2019Physics-informedEquations}. More specifically, it has shown potential to solve problems of multiphase flow in porous media in forward or inverse modes \citep{Latrach2024ASystems}, e.g., modelling of countercurrent spontaneous imbibition \citep{Abbasi2023SimulationNetworks}, solving multiphysics coupled flow problems\citep{Amini2023InverseNetworks} and modelling density-driven flow in porous media for CO$_2$ storage \citep{Du2023ModelingSequestration}. However, current studies are primarily focused on systems with homogeneous properties, often overlooking systems with multiscale features. The application of PINNs to multiscale problems is an emerging area of research, with some studies proposing various techniques in recent years \citep{Alber2019IntegratingSciences}. 
% For instance, \citet{Wang2021OnNetworks}, in the case of wave propagation and the Poisson equation, proposed to use Fourier feature embedding to capture the behavior of the system at various spatial scales and at the same time avoiding the potential spectral biases in the PINNs predictions. Spectral bias is defined as the tendency of networks to learn solutions with the lowest possible frequencies. \citet{Weng2022MultiscaleKinetics} proposed multiscale PINNs to model chemical kinetics that happens at very different time scales. They utilized different NNs with similar architectures for the different  reaction rates. \citet{Riganti2023AuxiliaryProblems} applied multi-output PINNs with multiple auxiliary variables associated and the Legendre terms to solve the Boltzmann equation efficiently. \citet{Moseley2023FiniteEquations} introduced Finite-Basis PINNs, by decomposing the domains of the problems, e.g., (2+1)-dimensional (D) wave propagation equations, using a finite set of basis functions, inspired by finite element methods. However, the literature shows significant gaps in applying PINNs for solving the multiphase flow in naturally fractured porous media, as a strategy for forward modeling and inverse parameter identification. 

% In this work, we have implemented a workflow based on the multiscale PINNs architecture for the forward and inverse simulation of (3+1)D multiphase flow in fractured porous media. To the best of our knowledge, the proposed workflow is the first to offer a PINNs-based approach for reliable and computationally efficient inverse modeling of multiphase flow in fractured porous media, suitable for history-matching noisy and multifidelity experimental measurements. The proposed workflow utilizes a multi-network architecture combined with various regularization techniques, such as data resampling during training, along with a step-wise training strategy to efficiently achieve the desired solutions. The robustness of the computational framework was first demonstrated through validation using a synthetic benchmark problem, and the performance compared against a finite-difference (FD) based numerical simulator, as a common approach in the community. Then we investigated a complex experimental scenario of water imbibition in CO$_2$ saturated fractured shale rock \citep{Kurotori2023MixedMedia}. We incorporated a large multi-fidelity observational dataset, including 3D in situ saturation data measured using a high-resolution computed tomography (CT) scan setup, in the process of inverse calculations. In this case, we applied the workflow for the simultaneous extraction of flow properties of the matrix and fracture system.


% % {\color{red}Ameya: To enhance clarity and highlight the novelty of this manuscript, it is a good idea to integrate a point-wise discussion on the contributions alongside the discussion on the experimental dataset. This approach will distinctly showcase the unique aspects and innovations of the study.}



% \section{Results}

% We investigate a (3+1)D problem of two-phase flow in fractured porous media. It is assumed the flow is controlled by Darcy's law in both fracture (Ω$_F$ ) and matrix (Ω$_M$ ) domains, where we refer to the low-permeability non-fractured zone as matrix, and the high-permeability fractured zone as fracture. The matrix domain occupies the majority of the pore volume while the fracture domain has a much higher permeability than the matrix. A schematic of the geometry of the core and the fractures is visualized in Fig. \ref{fig:2}a. The Darcy velocity (\(u_i\)) of each phase is determined by Darcy's law \citep{Das2005UpscalingBeyond}

% \begin{equation}
% u_i =-\lambda_i \nabla p_i,\ \ \lambda_i=\frac{Kk_{ri}}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy}
% \end{equation}
% where \(\lambda_i\) is mobility, \(p_i\) is the phase pressure, \(K\) and \(k_{ri}\) are absolute permeability and relative permeability, respectively, and \(\mu_i\) is the phase viscosity. The index \(i\) determines wetting \((w)\), and non-wetting \((nw)\) phases. The effects of gravity have been ignored due to low value of Bond number (ratio of gravity to capillary forces), i.e., $Bo << 1$ \cite{Li2018DynamicsMedia}. The capillary pressure, \(p_c = p_{nw}-p_{w}\), relates the phase pressures.  The conservation law for the spatiotemporal mass transport of phases in a matrix zone is defined as
% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right)+q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_frac_cont}
% \end{align}
% A similar mass conservation equation can be defined in the fracture domain 
% \begin{align}
% \phi^F\partial_t\left(\rho_is_{i}^{F}\right)=-\nabla^\parallel\left(\rho_iu_i^\parallel\right)\ -q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_F \label{eq:massbalF}
% \end{align}
% where \(q_i^\bot\) is matrix-fracture mass flux term and is a function of the local pressure difference between two mediums, and the matrix flow properties \citep{Berre2019FlowApproaches}. To solve the above coupled equations, we defined PINNs-based workflow based on a multiscale neural networks architecture. See \hyperref[sec:methods]{Methods} for detailed information on the mathematics of the problem, the NNs architecture, the collocation points applied, the observational data used, and the training procedure.



% \begin{figure}[htbp]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=.999\textwidth]%
%     {graphics/Fig2.jpg}% picture filename
% \end{center}
% \caption{\textbf{A schematic of the problem under study and the proposed PINNs-based computational workflow.} \textbf{a)} The simplified geometry of the matrix-fracture system and the impacting boundary conditions, \textbf{b)} The spatial distribution of the matrix and fracture collocation points, \textbf{c)} Separate networks for the state variables of matrix and fracture systems, \textbf{d)} The architecture of each NN, and \textbf{e)} the cross-sectional view of the porosity distribution in the experimental data, \textbf{f)} the proposed step-wise learning strategy.}
% \label{fig:2}
% \end{figure}



% \subsection{Synthetic Benchmark Problem}
% \label{sec:benchmarksection}
% This section focuses on validating the proposed PINNs-based workflow against forward and inverse modeling of a fully-characterized synthetic problem. We introduce a coupled matrix-fracture flow problem to validate the solutions obtained using PINNs and to compare different strategies. Fig. \ref{fig:benchprof}a1 provides a 3D visualization of the matrix-fracture system. Specifically, we define a cylindrical core featuring a significant vertical fracture (located at \(x=12.5\) mm) in the flow direction (\(y\)). The properties of both the matrix and the fracture are detailed in Table \ref{tab:benchprops}. Additionally, Fig. \ref{fig:benchprof}a2 illustrates the static geometry of the matrix and fracture system, along with a 3D visualization of the discretized model used for the FD simulations. The applied simulator were developed by \citet{Lohne2017ARegimes}, and provided us with the true solution of the defined benchmark problem. The advantage of the used simulator compared to other available simulators was its ability to solve seamlessly the experimental boundary conditions. The specifications of the utilized PINNs model is provided in Table \ref{tab:benchPINNsprops}. In this section, the network architecture is the same as in Fig. \ref{fig:2}. Also, the pre-training strategy was applied in both forward and inverse problems.


% \input{tables/t_bl}


% \subparagraph*{Forward simulation. } The flow saturation profile within the matrix, after forward solution of the problem based on the true parameter values, is visualized in Fig.~\ref{fig:benchprof}. The visualisation of the 3D profile of \(s_w\) and \(p_{w}\) as well as cross-sectional lateral invasion of water demonstrate the ability of the PINNs model to capture key 3D flow characteristics. The small errors in the predictions - i.e., the mean absolute error (MAE) of 0.028 for \(s_w\) and 0.42 bar for \(p_w\) - is accumulated mainly around the imbibition fronts. The computational times for the numerical solver and the PINNs solver were comparable for this specific forward problem. Fig.~\ref{fig:benchprof} clearly shows a sharp change in saturation at the flow fronts. This observation is primarily due to the low viscosity of CO$_2$ compared to the water phase (viscosity ratio of \(\mu_{\text{CO}_2}/\mu_{\text{water}} = 0.017\)). This difference in mobility of fluids creates a sharp saturation gradients in the system. Furthermore, the viscous flow in porous media creates shock fronts that are reported to be challenging to solve by many mathematical methods, including PINNs \cite{Fuks2020LIMITATIONSMEDIA}. In the matrix domain, the problem is manageable as the frontal shock is mainly cancelled out by capillary spreading effects. However, in the fracture domain, flow is governed primarily by viscous forces, which require specialised techniques. In this work, we assumed an insignificant value of capillary pressure in the fracture domain to mitigate the issue described, without compromising the accuracy and speed of the computations.
 

% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.95\textwidth]%
%     {graphics/fdbench.jpg}
% \end{center}
% \caption{\textbf{The geometry, and a comparative analysis of the frontal behavior of fluids as simulated by PINNs and FD for the benchmark problem forward simulation.} \textbf{a)} The map of the fracture in the synthetic matrix-fracture problem: 1) the geometry, 2) the equivalent static model for the FD simulations, \textbf{b)} a 3D visualization of  \(s_w\), and \(p_w\) profiles, and their point-wise absolute errors at t=57.7 hrs. \textbf{c)} the 2D cross-sectional view of \(s_w\) at y=29 mm for various time points: t=33.2, 57.7, and 81.2 hrs.}
% \label{fig:benchprof}
% \end{figure}


% \subparagraph{Inverse calculations based on history matching of recovery factor.}
%  Here, we utilise PINNs for the purpose of obtaining the flow parameters of the system, i.e., \(k_r\), \(p_c\) and \(\Lambda\) of matrix, by history matching of the observational data. \(\Lambda\) refers to a normalized Capillary Diffusion Coefficient (CDC), that controls the rate of capillary flow within porous media and is a function of the \(k_r\) and \(p_c\) curves. At this stage, we consider only the recovery factor (RF) curve as the observation data - which represents the volumetric fraction of the CO$_2$ phase expelled from the porous media over time. In this benchmark example, the porosity and permeability of the matrix, as well as all the properties of the fracture (including locations, porosity, permeability, and relative permeability curves), are assumed to be known prior to calculations. After random sampling of the inverse parameters, the calculations continued for 22000 epochs, until the error in RF was minimized (Fig. \ref{fig:benchinvres}a), the loss terms are stabilized (Fig. \ref{fig:benchinvres}f1), and the trend of changes in inverse parameters plateaued (Fig. \ref{fig:benchinvres}f2). The matching of the matrix RF curve (Fig. \ref{fig:benchinvres}b) could lead to the accurate estimation of the \(\Lambda\) curve with normalized mean absolute error (NMAE) of 0.098 (see Fig. \ref{fig:benchinvres}c1). PINNs calculations could also predict accurately the volumetric rate of the injected water, as shown in Fig. \ref{fig:benchinvres}d. The main determining factor on the brine injected rate is $K_F$, as the fracture shows orders of magnitude higher permeability compared to the matrix. 

% However, as expected, the model did not accurately retrieve the \(k_r\) and \(p_c\) curves (Figs. \ref{fig:benchinvres}c2 and \ref{fig:benchinvres}c3) due to the system's high degrees of freedom and the insufficient information on the wetting phase pressure. This limitation is evident in Fig. \ref{fig:benchinvres}e, where the workflow could predict the saturation profile in the system but failed to accurately predict the pressure distributions. The error is higher in zones with lower \(s_w\) values, due to the significance of \(p_c\).
% As the flow in matrix is mainly controlled by imbibition mechanism, we expect that there are infinite sets of \(k_r\) and \(p_c\) curves that can lead to the observed dataset  \cite{Abbasi2024ApplicationTests}. Actually, all possible combinations of \(k_r\) and \(p_c\) curves that lead to similar \(\Lambda\) curves are expected to lead to similar imbibition trends and frontal behavior. 


% Fig. \ref{fig:MFflow} provides a comparison of the matrix-fracture exchanges. Positive values indicate flow out of the fracture (into the matrix). In contrast, negative values indicate flow into the fracture (from the matrix). Initially, we observe a strong wetting phase flow from the fracture to the matrix, that stabilizes over time. This behavior results in an almost straight cumulative flow line versus \(\sqrt{t}\) at the beginning of the flow (\(t<20\) hr), highlighting the significant influence of capillary forces. The trend of cumulative imbibed volume then stabilizes at $\sqrt{t}>4.5 $ hr$^{0.5}$ ($t>20$ hr). However, the non-wetting phase experienced a matrix to fracture flow at the early times of the simulation, and which then stopped after \(t\approx 4\) hr. This behavior is expected in combined co-current/counter-current spontaneous imbibition processes \cite{Haugen2014CapillaryTest}. Fig. \ref{fig:MFflow}c compares the vector field of velocity for both phases. Although the wetting phase continuously imbibes into the matrix, the non-wetting phase follows viscous forces within the matrix towards the outlet of the system, indicating \textit{the governance of the co-current spontaneous imbibition mechanism in the matrix in a large fraction of the injection period}. 





% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/benchres.jpg}
% \end{center}
% \caption{\textbf{The results of inverse calculation for the synthetic benchmark model, based on history matching of the RF curve vs. time.} \textbf{a)} The trend of minimizing error compared to the RF data, \textbf{b)} The RF curves for matrix and fracture, \textbf{c)} The estimated flow curves compared to the true and the randomly initialized values: \(\Lambda\), \( p_c\) and \(k_r\) curves, respectively, \textbf{d)} The comparison of water injection rate for FD and PINNs models,  \textbf{e)} The flow profile along the injection direction for (1) \(s_w\)  and (2) \(p_w\), at t= 23.22, 57.7, 98.2, 167.9 hrs, \textbf{f)} the training trend, 1) The total loss term, ${\mathcal{L}}_{t}$, and loss terms corresponding to the PDE residuals for matrix, i.e.,  ${\mathcal{L}}_{PI}^{M}$, ${\mathcal{L}}_{PIw}^{M}$, and ${\mathcal{L}}_{PInw}^{M}$ , 2) the trend of changes in $\bar{\Lambda}$, representing the area under $\Lambda$ curve, \textbf{g)} A comparison of the run-time and accuracy of two history-matching approaches in the estimation of the \(\Lambda\) curve: PINNs, and FD + Nelder-Mead (NM) optimizer. }
% \label{fig:benchinvres}
% \end{figure}




% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/MFflow.jpg}
% \end{center}
% \caption{ \textbf{The matrix-fracture interaction rates for the benchmark problem.} In all the figures the right axis shows the cumulative values. The scatter points represent values at various spatiotemporal collocation points; \textbf{a1,2)} The mass rate of flow between two media for both phases; the right axis shows the cumulative mass flow (equation (\ref{eq:massratecum})). \textbf{b1,2)} the volumetric rate of flow; the right axis show the cumulative fraction of pore-volume (equation (\ref{eq:dimenlessPVMF})), \textbf{c)} 2D vector field plot at z=0.0125 m. Here, \( u_w \) and \( u_{nw} \) are not directly comparable, as they are scaled to the same range for visualization purposes.}
% \label{fig:MFflow}
% \end{figure}



% \subparagraph{Uncertainty quantification.} To validate the reported results, we employed an ensemble-based uncertainty quantification approach, performing multiple iterations with random initializations of the inverse parameters (refer to Appendix \ref{sec:PINNsComputationalstrat} for detailed methodology). As demonstrated in Fig. \ref{fig:benchinvens}a, the \(\Lambda\) curves consistently converged to similar values in different cases, all with low errors compared to the true \(\Lambda\) curve (Fig. \ref{fig:benchinvens} b shows how the solutions plateaued during training). It shows that \textit{ the system is well defined  with respect to the \(\Lambda\) curve}, meaning that there is only one set of \(\Lambda\) that can produce the observed measurements. In contrast, the \(k_r \) and \(p_c\) curves converged to distinct values, exhibiting the high degree of freedom in the system of equations. Similar results have been discussed in \citet{Abbasi2024ApplicationTests} for a 1D spontaneous imbibition system. 
% In this problem, due to the significantly higher permeability of the fracture compared to the matrix, the fracture is quickly saturated by water, and fracture-matrix contact faces behave similar to imbibition boundary conditions, resulting in capillary-dominated matrix-fracture flow. The imbibition boundary is treated as a Dirichlet condition, where \( s_w = 1-s_{nwr} \), \( p_{nw} = p_{nw}^F \) and \( p_{c} = 0 \) \cite{Meng2017AWettability}. Meaning that the system is primarily governed by imbibition, and is controlled by the shape and value of $\Lambda (s_w)$ curve  \cite{Abbasi2024ApplicationTests}.




% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.991\textwidth]%
%     {graphics/bench_ens.jpg}
% \end{center}
% \caption{ \textbf{The inverse calculation results for an ensemble with different initialization of the inverse parameters.} The initialization has been performed randomly.  \textbf{a)} the initial guess \textcolor{gray}{(gray)} and the final estimations after inverse calculations have been compared for \textcolor{magenta}{(magenta)} of \( \Lambda\), \( p_c\), \( k_{rw}\) and \( k_{rnw}\)  curves, respectively. The \textcolor{blue}{blue} curves show the true values. The shaded areas represent the mean $\pm$ standard deviations (STD).  \textbf{b)} the optimization landscape of different terms during optimization during the training: \( \mathcal{L}_t\), RF (MAE), and \( \bar{\Lambda}\), respectively.}
% \label{fig:benchinvens}
% \end{figure}



% \subparagraph{Computational cost.} The PINNs calculations were performed on a single A2000 GPU, which took around 1.5-2.5 hours depending on the size of the network and collocation points. The computational time was in the same range for both the forward and inverse problems, and regardless of the different sets of observational data used during history-matching, such as the in-situ $s_w$ dataset. For comparison, we also attempted to history-match the problem using a coupled FD and Nelder-Mead (NM) optimizer (see Appendices \ref{sec:compres} and \ref{sec:historymatching} for more info). Individual forward simulations for a 27,000 cell FD model ranged from 40 minutes to 2 hours, depending on the complexity of effective parameters (e.g., flow parameter shapes and matrix-fracture property contrasts). In the case of history matching the RF curve, the computational time of FD-NM optimisation was around 20 hours, with the NMAE of 0.81 (compared to the NMAE of 0.098 for PINN) in the estimated $\Lambda$ curve (see Fig. \ref{fig:benchinvres}g). When we added the in-situ $s_w$ dataset, the FD-NM optimizer failed to operate efficiently. The results highlight \textit{the significant advantage of proposed PINNs-based workflow compared to FD-based history-matching approach for inverse evaluation of experiments of multiphase flow in fractured porous media}.






% \subsection{Experimental Problem}
% This section employs PINNs for the interpretation and parameter identification of a real experiment of multiphase water-CO$_2$ flow in a naturally fractured shale rock sample, presented in \ref{sec:experimentaldata}. The known properties of the system are shown in Table \ref{table:shalerockprops}. In this experiment, the core is saturated by CO$_2$, and brine is injected at a fixed pressure drop. As an initial estimation, \(K\) and \(K_F\)  are assumed as 0.01 and 100 multipliers of the experimentally measured mean permeability of the rock  (\( K = 0.01 K_{exp} \) and \( K_F = 100 K_{exp} \)). The impact of \( K \) can be indirectly adjusted based on the calculated \(\Lambda\) curve, and \( K_F \) can be accurately calculated through history-matching the injection rate of water. Among all properties of the system, \(k_r(s_w)\), \(p_c(s_w)\), and their combined alternative, \(\Lambda(s_w)\), as well as \(K_F\) are unknown and are required to be estimated based on the experimental observations.



% \input{tables/table_experimental_props}



% \subparagraph{History matching of the recovery curve and the total injection rate.} 
% The volume of recovered fluids, the volume of the injected fluids, and the pressure drop along the core, all over time, are the most commonly utilized observational data for studying multiphase flow processes in porous media. We calculated the RF curve by averaging the in-situ water saturation data obtained from CT-scan measurements. In addition to the matrix multiphase flow parameters,  $K_F$ was assumed unknown, and allowed to be estimated during the inverse calculations. Inverse computations were started by randomly generated initial guess values for each parameter. To perform history matching of the RF curve, we employed the step-wise calculation process, as introduced in section \ref{sec:SolutionMethod}. The training process was stopped after 17000 epochs, when the trainable parameters reached a plateau. The validity of the inverse-calculated parameters then was validated by running a fine-grid FD numerical simulation based on these parameters, and comparing the obtained results with the experimental data. The results of inverse computation of matrix flow parameters, i.e., \(k_r\), \(p_c\), and \(\Lambda\) curves  are shown in Fig. \ref{fig:expres1}a. The validation of these curves by the forward FD simulations showed a reasonable match to the RF of the experimental data (Fig. \ref{fig:expres1}c). Fig. \ref{fig:3DprofileExp} compares the saturation and pressure profiles between PINNs and FD simulations. The profiles obtained from the inverse calculations using PINNs show reliable accuracy, closely matching those from the FD simulations. Also, despite not using in-situ saturation data during training, the PINNs were able to effectively capture the overall trend of water saturation in the CT images. Simultaneously, we matched the total injected fluids versus time, as shown in Fig. \ref{fig:expres1}d. The total volume of injected fluids is predominantly influenced by \(K_F\), as a significant portion $(>99\%)$ of the injected fluid enters the core through the fracture system and then flows toward the outlet face by bypassing the matrix. A small fraction of the fluid imbibes into the matrix (Fig. \ref{fig:expres1}d2), enabling the depletion of the non-wetting phase. The high injection rate at the beginning of the flow is due to the low resistance of the CO$_2$ phase, that initially saturated the fracture domain. The rate quickly drops to the level of $\approx$ 1.0 $mm/hr$ after breakthrough of the water phase at the outlet. A comparison of the RF curve, and the breakthrough time of water shows the injection rate of water is much higher than the critical rate of water advance. The critical rate is defined as the rate of water advance at which the positions of the water fronts in both the matrix and the fracture are equal \citep{Mattax1962ImbibitionReservoir}. It is concluded that \textit{the frontal behavior of fluids in matrix is not significantly influenced by the total injection rate in the system}, due to the permeability dominance of the fracture domain \cite{Berkowitz2002CharacterizingReview}.


% \subparagraph{ The calculated $k_r$ and $p_c$ curves are not unique.} 
% As it is also previously discussed in \ref{sec:benchmarksection}, \textit{the \(k_r\) and \(p_c\) curves exhibit non-uniqueness due to the degrees of freedom within the system} (unlike the \(\Lambda\) curve that can be uniquely estimated). 
% This conclusion is further supported by the results of ensemble-based uncertainty quantification shown in Fig. \ref{fig:expres1}e. The accurate estimation of \(k_r\) is easier when the effects of viscous forces dominate the matrix flow. However, in this system, the matrix is primarily influenced by capillary forces.



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.999\textwidth]%
%     {graphics/expres1.jpg}
% \end{center}
% \caption{ \textbf{The results for inverse calculation of matrix flow parameters by history matching of the RF experimental data.} \textbf{a)} The initial guess and final inverse calculated flow curves, i.e., \(k_r\), \(p_c\) and \( \Lambda\) curves, respectively. \textbf{b)} The trend of converging to the final values vs. epoch for different inverse parameters, \textbf{c)} The matched \( \bar{s_w}\) curve by PINNs (1) and the validation results from FD simulations (2), \textbf{d)} Matching the fracture permeability (\(K_f\)) and the history matching of volumetric injection rate: 1) the trend of changes in \(K_f\) versus the matrix permeability and experimentally measured permeability, \(K_{exp}\), 2) The contribution of matrix and fracture in the inlet face, 3) The total velocity of fluids compared to the experimental observational data. \textbf{e)} The results of inverse calculations for an ensemble of models with different initialization values. e1 and e2 show the convergence trends, and later show the saturation function curves. The grey curves are the initial guesses. }
% \label{fig:expres1}
% \end{figure}




% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/profile3dexp.jpg}
% \end{center}
% \caption{ \textbf{A visualization compares water saturation ($s_w$) and wetting phase pressure ($p_w$) distributions in the porous media (matrix) at different times}. The figure compares the PINNs solution after inverse computations, FD solution after forward validation simulation, and experimental CT-scan images. It is important to note that the local saturation data was not utilized during the inverse calculations for the PINNs. Also, the FD simulation shows the forward analysis using the PINNs-based inverse calculated flow parameters. }
% \label{fig:3DprofileExp}
% \end{figure}

% \subparagraph{The importance of multiscale simulations.} We investigate the significance of multiscale simulations in understanding multiphase flow in porous media in complex geometries, and their impacts on parameter identification calculations. In two separate cases, we conducted inverse calculations using PINNs while ignoring fractures and their interaction with the matrix: 1) matching only RF data, 2) matching RF data as well as water injection rate (Q$_{inj}$). Then, we compared the results to the cases with included fractures (see Fig.~\ref{fig:fracimpact}). The results clearly show the differences between the inverse calculated flow parameters (Fig.~\ref{fig:fracimpact}a). In the case of matching only RF data, ignoring the impacts of fractures could lead to about two orders of magnitude difference in the magnitude of the capillary forces in matrix ( \( \bar{\Lambda}= 8e-3 \) for the non-fractured scenario, compared to \( \bar{\Lambda}= 9e-5 \) for the fractured scenario). When Q$_{inj}$ was used as observational data, the results, specifically the relative importance of viscous and capillary forces, significantly changed. This led to high relative permeability and low capillary pressure values, that are unexpected for shale rock. It resulted in the misidentification of viscous flow as the dominant mechanism, underestimating the influence of capillary forces. 
% The obtained results highlights the \textit{critical need for multiscale matrix-fracture simulations when dealing with porous media exhibiting multiscale features like fractures}. However, these multiscale impacts are normally bypassed or overlooked in existing workflows due to computational inefficiencies and instability issues in numerical methods .


% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/fracimpact.jpg}
% \end{center}
% \caption{ \textbf{The impact of multiscale simulations on the inverse calculated flow parameters of porous media.} \textbf{a)} The calculated flow parameters, i.e.,  \( \Lambda\) ,\( p_c\), and \( k_r\) vs. saturation, respectively. \textbf{b)} The validation of the obtained results with FD simulations, in matching with the experimental RF data, \textbf{c)} The trend of changes in \( \mathcal{L}_t\), \( \bar{\Lambda}\), \({k}_{rw}^{max}\), and MAE in RF  vs. epochs, respectively. }
% \label{fig:fracimpact}
% \end{figure}




% \subparagraph{History matching of in-situ water saturation data.}

% History matching of high-fidelity datasets, in this case (3+1)D in-situ water saturation data from CT scans, presents a significant challenge but also offers exciting opportunities to gain deeper insights into porous media properties. In Fig. \ref{fig:insitusat}, rather than relying on RF data for the inverse calculations, we utilized the local spatiotemporal values of \(s_w\) directly as observational data for both history matching and the estimation of flow parameters. Additionally, we employ an adaptive fracture importance determination strategy to understand local variations in matrix-fracture interactions, serving as indicators of changes in fracture properties within the rock. A comparison of cases between the history matching of the datasets with and without denoised observational data show no meaningful differences in both saturation distributions as well as the inverse calculated \(\Lambda\) curves. Denoising has been performed via a 3D convolutional kriging approach, as explained in Appendix \ref{sec:PINNsComputationalstrat}. These results exhibit \textit{the capabilities of PINNs in extracting the governing physical properties of systems even in the presence of noisy observations} \citep{Chen2021Physics-informedData}. 

% In Fig. \ref{fig:insitusat}c, an approach is utilized to  detect automatically the inconsistencies between the PINNs predictions (based on the homogeneous fracture properties assumption), and the CT-scan images, in the fractured zone. The approach is explained in Appendix \ref{sec:PINNsimplementation}. In the points with gray color, the PDE solution closely matches the CT images, indicating high certainty in the defined fracture system. In the blue zones, the CT images show less imbibition than expected values by the PINNs solution, suggesting lower matrix-fracture interactions. Conversely, in the red regions, the saturation trends in the CT images differ significantly from the PINNs expectations, highlighting discrepancies that were successfully detected in both the original and denoised datasets. The results successfully showed the differences between the fracture properties, as well as uncertainties in the zones considered as the fractured areas. The results demonstrate that while we assumed a connected fracture network with uniform properties, the observations may not confirm these assumptions.



% \begin{figure}[htbp]
% \begin{center}
% \includegraphics[width=.99\textwidth]%
%     {graphics/insituepinns.jpg}
% \end{center}
% \caption{\textbf{ The PINNs solution for inverse calculations when the in-situ water saturation data have been used as the observations.} A comparison has been made between two cases in which the observations have been pre-processed using a convolutional kriging algorithm. \textbf{a)} A comparison of the inverse calculated flow curves (\(k_r\), \( p_c\) and \(\Lambda\), respectively) for different scenarios of using observational data, \textbf{b)} A comparison of the 3D water saturation ($s_w$) profiles at $t=23.4$ hrs, \textbf{c)} The results of fracture uncertainty quantification; $\xi_f=1$ (\textcolor{gray}{gray}) indicates minimal uncertainty, $\xi_f=0.6$ (\textcolor{blue}{blue}) represents medium uncertainty, and $\xi_f=0.2$ (\textcolor{red}{red}) represents high uncertainty) }
% \label{fig:insitusat}
% \end{figure}






% \section{Discussion}

% In this study, we have proposed a computational workflow based on Physics-Informed Neural Networks (PINNs) as a solver for the simulation and parameter identification of (3+1)D two-phase flow processes in naturally fractured porous materials. 
% The workflow is quite general, and can be applied to interpret a wide range of experimental datasets involving multiphase flow in porous media with complex geometries. The PINNs model employed a multi-scale network architecture, along with pre-training strategies and various regularization techniques (e.g., adaptive weighting, collocation point resampling, and Fourier transforms) to solve the PDEs under investigation.
% After validation of the model against a synthetic scenario, we applied the framework to interpret and analyse a multi-fidelity experimental dataset for water injection in a CO$_2$ saturated fractured shale rock. The studied experimental problem is characterized by a confluence of complexities: significant permeability contrasts, unpatterned distribution of fractures, highly unfavorable mobility ratios, and the presence of shock fronts in the fractures. 

% The results demonstrated the effectiveness of the workflow in capturing the multiscale flow dynamics, as well as the phase and pressure distributions in the system. In the case of inverse calculations, the workflow performed the calculations order(s) of magnitude faster and more accurately than FD-based simulation methods. The implemented uncertainty quantification analysis yielded valuable insights into the unique and non-unique characteristics of the obtained solutions. As the flow in matrix was mainly governed by capillary forces (imbibition), the problem could be uniquely characterized with a unique \(\Lambda\) curve, which  combines different flow properties of the system, confirming the relative dominance of capillarity forces as the flow mechanism in the matrix. However, reaching reliable information on individual \(k_r\) or \(p_c\) curves was not possible due to the unfavorable degree of freedom of the system, as demonstrated by the applied uncertainty quantification analysis. 
% It can potentially be overcome if separate measurements of both phase pressures are conducted \cite{Abbasi2024ApplicationTests, ShakerShiran2023ContinuousReservoir}. Additionally, simultaneous history-matching of RF curve, and brine injection rate depicts that the fractures served as primary flow conduits in the system. So, we could reach to the unique values for the fracture permeability. 

% Our comparison of inverse calculations with and without fractures demonstrates the pivotal role of multiscale phenomena in interpreting the experiments of imbibition in fractured porous media, as the presence of fractures introduces a hierarchy of scales in the system. These multiscale effects, while commonly overlooked in practical procedures, can significantly change the overall system behavior, influencing the inverse calculated parameters such as effective permeability, capillary pressure, and relative permeability relationships, as well as the interplay between different flow mechanisms in the system. For instance, the role of capillary forces may be significantly mischaracterized, as the harmony between capillary forces in the matrix and viscous forces in the fractures creates a complex, scale-dependent flow regime. This oversight can result in misleading parameter estimations, misattribution of flow behaviors, and ultimately, the development of incorrect conceptual or large-scale geological models, potentially leading to poor predictions and decision-making in practical applications. The proposed workflow with the applied strategies also performed well in evaluating the (3+1)D noisy high-fidelity observations of water saturation, and achieved results comparable to the denoised dataset. However, while the workflow offers more accurate and and order(s) of magnitude quicker solutions in comparison to a standard approach, further development is necessary to achieve fully reliable models for a wider range of multiphase flow scenarios. Increasingly complex fracture distributions likely require even more complex neural network architectures. This highlights the need for developing more flexible network architectures capable of handling the significant non-linearities exist in such complex systems.


% % {\color{red} Ameya: We should emphasize the detailed discussion of the in-situ experimental data set, as this is a key expectation of top journals like NMI. Without this, the paper may be perceived as another application-based PINN study.}




% \section{Methods}
% \label{sec:methods}


% \subsection{Mathematics of Flow in Fractured Porous Media}
% \label{sec:mathematicsofphysics}

% We approach a problem of 3D multiphase flow in a fractured porous media at core scale. 
% Our focus is specifically on interpreting data from a cylindrical core-plug (a shale rock taken from the Wolfcamp formation) \citep{Kurotori2023MixedMedia}. We refer to the low-permeability non-fractured zone as a matrix, and the high-permeability fractured zone as a fracture. The model is inferred from the definition that the matrix domain \((\Omega_M)\) occupies the majority of the pore volume and that fractures domain \((\Omega_F)\) have a much higher permeability than the matrix.
% The geometric structures of the core and the fractures are given in \citet{Kurotori2023MixedMedia}. A simplified schematic of the sample set-up is visualized in Fig. \ref{fig:2}a.
% The core is placed horizontally, and the fractures are distributed in the core with different orientations. The radial surface of the core at \(r_c\) is closed (no-flow boundary). The inlet and outlet faces are at \(y=0\)  and \(y=L\), respectively.  Water and CO\textsubscript{2} are considered to be the wetting \((w)\) and non-wetting \((nw)\) phases, respectively. In line with the experimental conditions, we neglected both the compressibility and the solubility of the phases. The system is initially saturated with the \(nw\) phase. The definition of the system implies that the flow phenomena are governed by mixed-imbibition mechanisms, where the fracture flow is driven by forced imbibition, and the matrix flow is governed by spontaneous imbibition between the fracture(s) and the matrix. Forced imbibition happens when an external force drives the wetting phase fluid through the porous media, overcoming any resistance from the medium and the non-wetting phase. Spontaneous imbibition, on the other hand, is the process in which the wetting phase fluid flows into a porous media via capillary forces without the need for external pressure \citep{Anderson1987WettabilityPressure}. In the following, the mathematics of flow in matrix and fracture domains are discussed.

% \subparagraph{Matrix flow. }
% The Darcy flow velocity (\(u_i\)) of each phase in the matrix is determined by Darcy's law
% \begin{equation}
% u_i =-\lambda_i \nabla p_i,\ \ \lambda_i=\frac{Kk_{ri}}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy}
% \end{equation}
% where \(\lambda_i\) is mobility, \(p_i\) is the phase pressure, \(K\) and \(k_{ri}\) are absolute permeability and relative permeability, respectively, and \(\mu_i\) is the phase viscosity. The index \(i\) determines\((w)\), and \((nw)\) phases. The effects of gravity have been ignored. The conservation law for the spatiotemporal mass transportation of phases in a matrix zone is defined as
% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right),\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_cont}
% \end{align}
% Given that \({s}_{wc}=0\), we define the initial conditions as
% \begin{align}
% \left\{\begin{array}{left} {s}_{w}(x,y,z,t = 0) = 0\\ {p}_{nw}(x,y,z,t = 0) = {p}_{i} \\  \end{array}\right \ \ \ {, \in\Omega}_M
% \label{eq:eqICmatrix}
% \end{align}

% At the inlet face ($y=0$), the wetting phase is injected under a constant pressure ${p}_{in}$ over time. At this face, it is assumed the wetting phase takes the highest possible mobility
% \begin{align}
% \left\{\begin{array}{left} {s}_{w}(x,y = 0,z,t) = 1 - {s}_{nwr} \\ {p}_{w}(x,y = 0,z,t) = {p}_{in} \\  \end{array} 
% \label{eq:eqBC0matrix}
% \end{align}
% The production from the outlet face \((y=l)\) occurs at a constant pressure, \({p}_{out}\)
% \begin{align}
% {p}_{nw}(x,y = L,z,t) = {p}_{out} 
% \label{eq:eqBC1matrix}
% \end{align}
% At the outlet face of the core, no explicit constraints are imposed on the saturation of the fluid phases. The radial faces \((r = r_c)\) are sealed from flow in radial directions
% \begin{align}
%  \frac{\partial p}{\partial r} |_{r = r_c} \approx |\frac{\partial p}{\partial x} |_{r = r_c} + |\frac{\partial p}{\partial z} |_{r = r_c} |= 0 
% \label{eq:eqBC1matrix}
% \end{align}

%  The assumed matrix properties state that the flow in the matrix is governed by viscous and capillary forces (gravity effects are assumed to be negligible). 


% \subparagraph{Fracture flow. }
%  A fracture is typically characterized as a narrow, and high permeability zone enclosed by a less permeability matrix zone. This contrast in properties leads to highly heterogeneous flow behavior across the scales. The aperture between the fracture surfaces is generally small and is normally occupied by filling materials, that affects its effective porosity and permeability values \citep{Wu2016MultiphaseMedia}. 

% Although fractures are discontinuities in the porous medium, they are considered as a separate porous medium domain \((\Omega_F)\). This assumption enables us to apply Darcy's law. 
% Consequently, we assume fractures to be high permeability porous zones. This makes the equations in the two media consistent, eliminating the need for unnecessary complexities in the calculations \citep{Martin2005ModelingMedia}. So, the average flux of each flowing phase in a fracture is written by modification of Darcy's law in equation (\ref{eq:darcy}) as
% \begin{equation}
% v_i^{\parallel}=-\lambda_i^{\parallel} \nabla^\parallel p_i ,\ \ \lambda_i^\parallel=\frac{K^F k_{ri}^\parallel}{\mu_i},\ \ \left(i=w,nw\right)\label{eq:darcy_frac}.
% \end{equation}
% In this equation, \(K_F\) is the fracture permeability, and \(k_{ri}^\parallel\) is the relative permeability of the fluids in the fracture. The value of the \(K_F\) is dependant on the fracture aperture, and also the extent of the filling materials in the fracture. 


% \subparagraph{Matrix-fracture interactions. }

% The accurate treatment of multiphase flow in a fractured porous media depends on the modeling of the dynamic matrix-fracture coupled interactions. Utilizing Darcy's law \cite{Berre2019FlowApproaches}, the matrix-fracture flux is approximated by 
% \begin{align}
% v_i^\bot=-2K^\bot\lambda_i^\bot\left[\frac{ p_{M,i}-p_{F,i} }{e_V}\right],\ \ \lambda_i^\bot \simeq \frac{k_{ri}}{\mu_i},\ \ \left(i=w,nw\right), \label{eq:e8}
% \end{align}
% where \(K^\bot\) refers to the matrix-fracture permeability normal to the fracture surface, and \(e_V\) is the fracture average aperture. As an ideal case, if one assumes a fracture as an open space between two parallel surfaces, then the aperture is called the hydraulic aperture, \(e_h\). In practice, the value of \(e_v\) is much larger than  \(e_h\), i.e., \(e_v>>e_h\), as the fractures are normally filled with materials. The value of \(K_F\) is theoretically correlated to \(e_v\). In this study, the fracture aperture, \(e_v\), is assumed to be 0.001 m for all the fractures, and kept constant in all the evaluations. The cumulative value \( V_i^\bot(t)  \) of a rate \( v_i^\bot(t)  \) over time is given by the following integral
% \begin{align}
% V_i^\bot(t) = \int_0^t v_i^\bot(\tau) \, d\tau
%  ,\ \ \left(i=w,nw\right). \label{eq:cumv}
% \end{align}
% We can rewrite equation (\ref{eq:e8}) to obtain the mass transfer rate [kg/m\(^3\)/s] between the two media as
% \begin{align}
% q_i^\bot=\frac{2\rho_i}{e_V} v_i^\bot ,\ \ \left(i=w,nw\right). \label{eq:massrate}
% \end{align}
% The factor 2 denotes the flow across both sides of fracture to matrix, assuming the equal flow characteristics across the two surfaces of the fracture. Then, the cumulative injected mass [kg/m\(^3\)] is
% \begin{align}
% Q_i^\bot(t) = \int_0^t q_i^\bot(\tau) \, d\tau
%  ,\ \ \left(i=w,nw\right). \label{eq:massratecum}
% \end{align}
% The equation of mass conservation in the fracture is the same as in the matrix, with an additional term representing the mass from the fracture to the matrix \( q_i^\bot \). So, by modifying the matrix mass balance equation (equation (\ref{eq:matrix_cont})), we define the mass balance in the fracture system as follows
% \begin{align}
% \phi^F\partial_t\left(\rho_is_{i}^{F}\right)=-\nabla^\parallel\left(\rho_iu_i^\parallel\right)\ -q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_F \label{eq:massbalF}
% \end{align}
% At the contact point of the matrix and fractures, the continuity equation should also be solved in the matrix domain. So, we may rewrite equation (\ref{eq:matrix_cont}) as 
% \begin{align}
% \phi\partial_t\left(\rho_is_i\right)=-\nabla\left(\rho_iu_i\right)+q_i^\bot,\ \ \left(i=w,nw\right),\ \ {\in\Omega}_M \label{eq:matrix_frac_cont}
% \end{align}
% The fraction of the pore volume of the matrix [dimensionless] that has been transferred between the matrix and fracture can also be calculated using the following equation
% \begin{align}
% V_i^\bot(t) = \frac{Q_i^\bot(t)}{\phi \rho_i},\ \ \left(i=w,nw\right), \label{eq:dimenlessPVMF}
% \end{align}




% \subparagraph{Closure equations. }
% Capillary pressure and relative permeability curves are crucial input to model multiphase flow in porous media, e.g., in equations (\ref{eq:matrix_cont}), (\ref{eq:massbalF}) and (\ref{eq:matrix_frac_cont}). These curves are normally defined using theoretical correlations, with a few matching parameters. In this work, we apply an extended version of the Corey function \citep{Corey1954ThePermeabilities} to model relative permeability curves
% \begin{align}
% {k}_{rw}({S}_{w}) = {k}_{rw}^{max}({S}_{w})^{{n}_{w}};\ \ \ \ \ \ {n}_{w} = {n}_{w1}{S}_{w} + {n}_{w2}(1 - {S}_{w}) \label{eq:krw_eq}
% \end{align}
% \begin{align}
% {k}_{rnw}({S}_{w}) = {k}_{rnw}^{max}(1 - {S}_{w})^{{n}_{nw}};\ \ \ \ \ \ {n}_{nw} = {n}_{nw1}{S}_{w} + {n}_{nw2}(1 - {S}_{w})
% \label{eq:krnw_eq}
% \end{align}

% In the extended version, \(n_w\) and \(n_{nw}\) are defined as saturation exponents that are weighted linearly with saturation \(S_w\). \(S_w\) is the normalized water saturation and is calculated as
% \begin{align}
% {S}_{w} = \frac{{s}_{w} - {s}_{wc}}{1 - {s}_{nwr} - {s}_{wc}};
% \label{eq:Sweq}
% \end{align}
% The capillary pressure curve \(P_c(S_w)\) [pa] is calculated via Leverett scaling \citep{Leverett1942Dimensional-modelBehavior}

% \begin{align}
% P_c = \sigma \sqrt{\frac{\phi}{K}} J
% \label{eq:pceq}
% \end{align}
% In this context, J(S$_w$) represents the Leverett J-function, a dimensionless function that describes the shape of the capillary pressure curve. We define J-function via the modified \citet{Bentsen1977UsingCurve} correlation
% \begin{align}
% J(S_w) =  - {J}_{1}\mathrm{\ln}(\frac{{S}_{w}}{{S}_{eq}}) + {J}_{2}\mathrm{\ln}(\frac{1 - {S}_{w}}{1 - {S}_{eq}})
% \label{eq:Jeq}
% \end{align}

% The equation is hard constrained in a way that that \(J(S_{eq})=0\) and that \(dJ/dS_w\)   becomes infinite at endpoints. 

% However, previous research by \cite{Andersen2023Early-andCoefficient} demonstrated that capillary-dominated two-phase flow in porous media (spontaneous imbibition) can be uniquely characterized by the capillary diffusion coefficient (CDC) curve. This curve represents a mixed combination of flow properties of both phases
% \begin{align}
% \Lambda = \mu_m \lambda_{nw} f_w \left( -\frac{dJ}{dS_w} \right)
% \label{eq:Lambda}
% \end{align}
% In this equation, \(\mu_m\) is the geometric mean of the phase viscosities \((\sqrt{\mu_w \mu_{nw}}\)). The CDC curve, as well as the dynamics of multiphase flow in porous media is mainly controlled by the relative permeability of the phases and the capillary pressure curves. Measurement of these curves is challenging and typically requires indirect methods, such as history matching using numerical simulations \citep{Krause2015AccurateCurves}. However, history matching in complex geometries, such as fractured porous media, is a challenging task that involves significant computational complexities. The challenge becomes more serious when high-fidelity datasets, such as CT-scan images, must be matched. In this work, we propose the application of PINNs as a reliable framework for history matching and characterisation of such problems. 


% \subparagraph{Known and unknown parameters. }
% To characterize fully the discussed system of equations, it is crucial to determine and understand the properties of both the matrix and the fractures. The determination of fluids properties, or average porosity and permeability of rock can be done using simpler methods. However, determination of the multiphase flow properties of the system - i.e., the relative permeability (\( k_r\)) and capillary pressure (\( p_c\)) of the matrix - is essential for accurately understanding the governing mechanisms, and this primarily requires multiphase experimental core flooding tests, in which the cylindrical rock is first saturated by a phase, then injected by the second phase at controlled pressures and flow rates. 
% The \( k_r\) curve can be fully addressed via six parameters related to the Corey model (equations (\ref{eq:krw_eq}) and (\ref{eq:krnw_eq})): \({k}_{rw}^{max}\), \({k}_{rnw}^{max}\), \(n_{w1}\) and \(n_{w2}\), \(n_{nw1}\) and \(n_{nw2}\). Also, the \( p_c\) curve can be characterized via \(J_{1}\) and \(J_{2}\) parameters, based on equation (\ref{eq:Jeq}). 

% Due to the small pore volume of the fractures, we can reasonably assume a constant fracture porosity. The fracture permeability (\(K_{F}\)), which significantly impacts the overall flow rate during the experiments, needs to be calculated. Additionally, for simplicity, we assumed linear relative permeability curves for fractures \citep{DeLaPorte2005TheReservoirs}. 




% \subsection{Methodology}

% Physics-Informed Neural Networks (PINNs) were introduced by \citet{Raissi2019Physics-informedEquations} as an efficient method for solving differential equations by combining neural networks with physics-based principles. In this study, we defined neural networks (separately for matrix (\( \mathcal{N}_m \)) and fracture (\( \mathcal{N}_f \)) domains), to emulate the functional dependency between the independent and dependent variables
% \begin{align}
% {s}_{w},{p}_{nw} = \mathcal{N}^{M}(x,y,z,t,\theta,\eta)
% \label{eq:pceq}
% \end{align}
% \begin{align}
% {s}_{w}^{f},{p}_{nw}^{f} = \mathcal{N}^{F}(x_{f},y_{f},z_{f},t,\theta_{f},\eta)
% \label{eq:p1}
% \end{align}
% where, [\(x, y, z\)] and [\(x_f, y_f, z_f\)]   are the spatial coordinates corresponding to the collocation points of matrix and fracture, respectively. \( \theta\) and \( \theta_f\) are the network trainable parameters.
% The goal is to solve an optimization problem where
% \begin{align}
% \theta^{m,f},\eta = \arg\min(\mathcal{L}_{t})
% \label{eq:p2}
% \end{align}
% where \( \eta\) is a set of inverse parameters calculated during the inverse calculations. Also, \( \mathcal{L}_{t} \) is the total loss term, defined to minimize the errors in both the physical flow equations in the matrix and fracture, as well as the available observation data. The outlet of networks are the state variables of the system, that are the \(s_w\), and \(p_{nw}\). The total loss term is a weighted combination of matrix and fracture losses, as well as losses corresponding to observational data
% \begin{align}
% \mathcal{L}_{t} = \mathcal{L}_{t}^{M} + \mathcal{L}_{t}^{F} + \mathcal{L}_{t}^{D} 
% \label{eq:p2}
% \end{align}
% where \(\mathcal{L}_{t}^{M}\) and \(\mathcal{L}_{t}^{F}\) are the total loss terms corresponding to the initial/boundary conditions, as well as the PDE residuals for matrix and fracture domains, respectively. Minimizing these terms ensures the PINNs solution respects the physical constraints within their domain.
% Furthermore, \(\mathcal{L}_{t}^{D}\) represents the total loss term corresponding to the errors in the predictions of PINNs compared to the observational data. The complete explanation of the PINNs implementation and the underlying loss terms is provided in Appendix \ref{sec:PINNsimplementation}.

% To address the inverse problem, we adopted an ansatz approach for representing the relative permeability and capillary pressure curves. This means a trainable vector was defined, where each element corresponded to a parameter within the chosen correlations for these curves (equations (\ref{eq:krw_eq}), (\ref{eq:krnw_eq}) and (\ref{eq:pceq})). More information regarding the initialization and definition of the inverse variables is provided in Appendix \ref{sec:PINNsComputationalstrat}. 



% \subsection{Model Architecture}
% The architecture of the applied PINNs model is shown in Fig. \ref{fig:2}.
% Due to the complexities in the geometry, and non-linearities in flow profiles, we considered the matrix and fracture systems as decomposed domains. Then, separate networks were allocated to each domain, to increase the flexibility of the networks in capturing the high-frequency trends in the solution of equations. Also, for each domain, the system state variables, i.e., pressure (\(p_{nw}\))  and water saturation (\(s_w\)) had separate networks (Fig. \ref{fig:2}b). Before passing the data to the network, the input data was normalised to the approximate range of (-1,1). The (de)normalization technique is discussed in Appendix \ref{sec:PINNsComputationalstrat}. 
% In the NNs corresponding to the \(S_w\) values (for both matrix and fracture), we used the following sequence of operators: an encoder, a Fourier transformer, a latent multilayer perceptron (MLP) network, an inverse Fourier transformer, and a decoder network (as shown in Fig. \ref{fig:2}c). The outlet of the NNs is then denormalized to the range of actual values. The Fourier transformers were used to make the networks able to capture the high-frequency or multiscale behavior \citep{Wang2021OnNetworks} in the frontal regions of the saturation profiles. The NNs for the calculation of \(p_{nw}\) were similar, except that the Fourier and inverse Fourier transformations were not applied. The MLP network, which had a depth of five and a width of 80 neurons, was activated by an adaptive \(tanh\) activation function. 
% The model was initialized using the Glorot initialization scheme \citep{Glorot2010UnderstandingNetworks}. Separate MLP networks were used to address the self-adaptive local weighting of the errors in PDE residuals for matrix and fracture domains. See Appendices \ref{sec:PINNsimplementation} and \ref{sec:PINNsComputationalstrat} for more details.

% \subparagraph{Training:} 
% The network was trained utilizing an Adam optimizer employing a full-batch approach and incorporating a gradually decreasing learning rate, from 0.0003, to 0.0001. We have applied a weight decay value of 0.0001. The number of gradient descent training steps (epochs) depended on the problem's complexity. Typically, 15,000 to 25,000 epochs were needed for stable error values. 



% \input{tables/table_app2}


% \subsection{The Solution Approach} 
% \label{sec:SolutionMethod}
% The investigated system of equations governing the matrix and fracture domains exhibits a complex interdependency.  In this context, training the model using a fully-coupled approach generates chaotic computational behavior as the interaction terms between the matrix and fracture domains are highly sensitive to the accuracy of the calculations performed in each domain individually. On the other hand, the invasion of fluids from the fracture into the matrix domain is a strong function of the values of the interaction terms. Crucially, the differing loss landscapes of the matrix and fracture PINNs models result in distinct convergence behaviors. To mitigate these issues, alternative preconditioning techniques are necessary \citep{Krishnapriyan2021CharacterizingNetworks}. In this work, we suggested to apply a sequence of pre-training training steps before performing the fully-coupled simulations. The details of the applied approach is visualized in Fig. \ref{fig:2}e. In this process, at first, the matrix and fracture networks are trained individually, without utilizing any coupled inter dependencies. Then, we shift to the fully-coupled training technique. 

% However, the utilisation of the pre-training technique, although considers many of the possible flow mechanisms, neglects the impact of mechanisms such as viscous flow interactions between the matrix and fracture. The difference gets more critical when the permeability and capillary variation in matrix and fracture media is less significant. The mentioned mechanisms are naturally considered in the fully coupled approach. So, after pre-training of the networks, and reaching an equilibrium in the training process, we switch to the fully coupled technique. The mathematics behind coupling the matrix and fracture is previously explained in section \ref{sec:mathematicsofphysics}. 


% \subparagraph{Pre-training:} This stage leverages the model reduction technique \citep{Chung2017CouplingApproaches} as a means to tackle multiscale problems. To do so, we applied an independent training strategy for matrix and fracture at the beginning of training, before shifting to the fully-coupled training strategy. In this approach, instead of defining the matrix-fracture transfer to modify the PDEs of flow, we explicitly applied their impacts as the boundary conditions in the matrix as follows. 

% \begin{itemize}
% \item Matrix: The multiphase flow in the matrix is analyzed by assuming that the \(s_w\)  and the \(p_{nw}\) in the matrix at points of intersection with fractures are equal to the corresponding values in the fractures
% \begin{align}
% s_w = s_{w}^{F,BL},\ \ \ \ {\in\Omega}_{MF} \label{eq:pretrsw}
% \end{align}
% \begin{align}
% p_{nw} = p_{nw}^{F,BL},\ \ \ \ {\in\Omega}_{MF} \label{eq:pretrpnw}
% \end{align}
% \(s_{w}^{F,BL}\) is calculated using the 1D Buckley-Leverett (BL) theory, and \(p_{nw}^{F,BL}\)  is calculated using linear pressure distribution assumption. The Buckley-Leverett theory offers a fundamental analytical approach for forecasting the saturation profile and front velocity of the displacing fluid in two-phase flow in porous media. The BL theory is explained in Appendix  \ref{sec:BLequation}. 
% \item Fracture: The PINNs model corresponding to the PDE of multiphase flow in fractures is solved by ignoring the interactions with matrix. 
% \end{itemize}

% In the case of inverse calculations, before starting the optimization of inverse variables, it is essential to partially train the networks so that they can learn the main characteristics of the problem. This approach has been successfully applied in previous studies, such as those by \citet{Zhang2022AnalysesNetworks} and \citet{Abbasi2024ApplicationTests}. At this step, the trainable inverse parameters are kept frozen for some limited epochs. 


% \input{tables/table_dlnetwork}






% \subsection{Experimental Data}
% \label{sec:experimentaldata}
% The study evaluated experimental data from injecting brine into a  CO\textsubscript{2}-saturated fractured shale rock core, as detailed in \cite{Kurotori2023MixedMedia}. The cylindrical Wolfcamp shale core had a length of 5.8 cm, diameters of 2.5 cm, an average permeability of \(1.97e-17\) m$^2$ (0.020 mD) and porosity of 0.102. The core was initially saturated with CO\textsubscript{2}, then brine was injected at 530 psi injection pressure and 460 psi backpressure for 311 hours while confined at 700 psi. Dynamic CT images were captured at intervals, recording in-situ saturation, phase recovery, and injected fluid volume over time. Different fractures were identified from the CT scan images \cite{Murugesu2024CoupledCaprocks}. History matching and inverse calculations in this study relied on several key experimental measurements (also see Fig. \ref{fig:colls}e)

% \begin{itemize}
% \item\textbf{Recovery Factor (RF)}: the volume fraction of the pore space displaced by the injected fluid over time. We calculated the RF curve by averaging the saturation of the wetting phase fluid obtained from CT scan images.
% \item\textbf{Boundary Conditions}: The constant pressure at the inlet and outlet boundaries were known based on the experimental setup.
% \item\textbf{Injection Volume}: The total volume of water injected into the system as a function of time was directly measured.
% \item\textbf{Spatial Saturation Data}: Spatial distribution of fluid saturation within the sample at different times, obtained through CT scans.
% \end{itemize}

% More details on the data sets used in this study and their use within the PINNs framework can be found in Appendix \ref{sec:PINNsimplementation}2.



% \subsection{Collocation Points}
% As it is visualized in Fig. \ref{fig:colls}, collocation points were extracted separately for the matrix and fracture domains based on the CT/micro-CT scan coordinates. 23500 matrix spatial collocation points were used in the core cylinder domain at specified x, y, z resolutions, excluding points in superposition with fractures. Boundary collocation points were collected for the cylinder ends and radius. Fracture collocation points were manually extracted from micro-CT scans. Temporal collocation points were randomly selected based on the \(\sqrt{t}\) distribution intervals, as it is expected that the system is mainly controlled by spontaneous imbibition mechanism. \cite{Abbasi2023SimulationNetworks} have shown how the selection of temporal points based on \(\sqrt{t}\) distribution intervals helps in improving PINNs solutions. More detailed information about the experimental data and the collocation points are provided in Appendix \ref{sec:PINNsCollocation Points}.





% \begin{figure}[htbp]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=.99\textwidth]%
%     {graphics/colls.jpg}% picture filename
% \end{center}
% \caption{ \textbf{The collocation points have been used for solving the problem under study.} The color of the points demonstrate the corresponding time for each point in the range \(t=1-10^6 \) sec. \textbf{a)} The collocation points at the boundary conditions of inlet (y=0) and outlet (y=L) faces (940 spatial points), \textbf{b)} The collocation points corresponding to the non-flowing boundary condition at \(r=r_{c}\) (8630 spatial points), \textbf{c)} The collocation points corresponding to the fracture (4103 spatial points), \textbf{d)} The collocation points corresponding to the matrix (23500 spatial points). The matrix collocation points with distance less than 0.0006 m from the fracture collocation points have been removed. \textbf{e)} the observational data points used in the data loss: 1) RF points, 2) points with the measured injected volume, and 3) spatiotemporal points of the in-situ \( s_w\) measured using CT-scan. }
% \label{fig:colls}
% \end{figure}






% \section*{Acknowledgments}
% Abbasi, Andersen, and Hiorth acknowledge the Research Council of Norway and the industry partners of NCS2030 – RCN project number 331644 – for their support.


% \bibliography{mendeley} 
% \printbibliography

% \input{suppl}

% \end{document}

% % \section*{Appendix: Numerical simulations }
% % We have utilized a finite-difference simulation approach to simulate the 








==> diffmain.tex <==
% \RequirePackage{shellesc}
% \usepackage[dvipsnames]{xcolor}
% %DIF PREAMBLE
% \providecommand{\DIFadd}[1]{{\protect\color{green}\uwave{#1}}} %DIF PREAMBLE
% \providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
% \ShellEscape{latexdiff changes/main0.tex main.tex  > main-d.tex}
% \input{main-d}
% \documentclass{dummy}
% \title{Demonstrating latexdiff}

==> tables/table_bench_netsize.tex <==

\begin{table}[ht]

\caption{The impact of network size (length and width) on the accuracy of the forward calculations. The simlations continued upto 18000 epochs for all of the cases.}
\begin{center}
    \label{tab:2}
    \begin{tabular}[t]{llll}
    \hline
    Length & Width & Model Size & RF (MAE)  \\ \hline
    4  &  40 & 1154 & 0.093  \\ \hline
    5  &  50 & 1781 & 0.037  \\ \hline
    6  &  60 & 2544 & 0.035  \\ \hline
    7  &  70 & 3246 & 0.037  \\ \hline
    8  &  80 & 3876 & 0.024 \\ \hline
  
    \end{tabular}
\end{center}
\label{table:netsize}

\end{table}



==> tables/table_collpoints.tex <==

\begin{table}[ht]

\caption{The impact of the number of collocation points on the accuracy of the training. In all of the cases, the same training strategy has been used.}
\begin{center}
    \label{tab:2}
    \begin{tabular}[t]{llll}
    \hline
    \# of Collocation Points & RF (MAE) & \(P_{nw}\) (MAE)   \\ \hline
    4010  &  0.023 & 53.69 (1.62 \%)  \\ \hline
    13226  &  0.025 & 51.63 (1.56 \%)  \\ \hline
    22970  &  0.028 & 52.43 (1.58 \%)  \\ \hline
    54880  &  0.028 & 51.45 (1.55 \%)  \\ \hline
    76500  &  0.030 & 54.95 (1.69 \%)  \\ \hline
  
    \end{tabular}
\end{center}
\label{table:collpoints}
\end{table}
